A Probabilistic Angle on One Loop Scalar Integrals

Recasting the $N$-point one loop scalar integral as a probabilistic problem, allows the derivation of integral recurrence relations as well as exact analytical expressions in the most common cases. $\epsilon$ expansions are derived by writing a formula that relates an $N$-point function in decimal dimension to an $N$-point function in integer dimension. As an example, we give relations for the massive 5-point function in dimension $n=4-2\epsilon$, $n=6-2\epsilon$. The reduction of tensor integrals of rank 2 with $N=5$ is achieved showing the method's potential. Hypergeometric functions are not needed but only integration of arcsine function whose analytical continuation is well known.

==> bibliography.tex <==

@PROCEEDINGS{1998WinterSimulationConference,
  title = {{Proceedings of the 1998 Winter Simulation Conference}},
  year = {1998},
  editor = {D. J. Medeiros and E. F. Watson and J. S. Carson and M. S. Manivannan},
  note = {D.J. Medeiros, E.F. Watson, J.S. Carson and M.S. Manivannan, eds.},
}

@PROCEEDINGS{2000Bachelier,
  title = {{Mathematical Finance - Bachelier Congress 2000}},
  year = {2002},
  editor = {H. Geman and D. Madan and S. R. Pliska and T. Vorst},
}

@PROCEEDINGS{2001WinterSimulationConference,
  title = {{Proceedings of the 2001 Winter Simulation Conference}},
  year = {2001},
  editor = {B. A. Peters and J. S. Smithand D. J. Medeiros and M. W. Rohrer},
  month = {Dec},
}

@INPROCEEDINGS{ABOwen,
  author = {A. B. Owen},
  title = {{Monte Carlo extension of quasi-Monte Carlo}},
  booktitle = {{Proceedings of the 1998 Winter Simulation Conference}},
  year = {1998},
  address = {Department of Statistics Stanford University Stanford, CA 94305,
	USA},
  note = {\url{www.informs-cs.org/wsc98papers/076.PDF}},
  crossref = {1998WinterSimulationConference},
}

@ARTICLE{ACM-659,
  author = {P. Bratley and B. L. Fox},
  title = {{Algorithm 659: Implementing Sobol's Quasirandom Sequence Generator}},
  journal = {ACM Transactions of Mathematical Software},
  year = {1988},
  volume = {14},
  pages = {88--100},
}

@ARTICLE{ACM-738,
  author = {P. Bratley and B. L. Fox and H. Niederreiter},
  title = {{Algorithm 738: Programs to generate Niederreiter's low-discrepancy
	sequences}},
  journal = {ACM Transactions of Mathematical Software},
  year = {1994},
  volume = {20},
  pages = {494--495},
  number = {4},
  month = {December},
}

@TECHREPORT{Abe2004,
  author = {K.E.S. Abe},
  title = {{Strong Taylor Schemes for Stochastic Volatility}},
  year = {2004},
  type = {Working paper},
  note = {\url{www.maths.ox.ac.uk/\~schmitz/project2.htm}},
  owner = {gbjaep},
}

@BOOK{AbramowitzStegun,
  title = {{Pocketbook of Mathematical Functions}},
  publisher = {Harri Deutsch},
  note = {ISBN 3-87144-818-4},
  year = {1984},
  author = {M. Abramowitz and I. A. Stegun},
}

@MISC{Acklam,
  author = {P. J. Acklam},
  title = {{An algorithm for computing the inverse normal cumulative distribution
	function}},
  howpublished = {\url{home.online.no/~pjacklam/notes/invnorm/index.html}},
  month = {June},
  year = {2000},
  note = {University of Oslo, Statistics Division},
}

@INCOLLECTION{AcworthBroadieGlasserman,
  author = {P. Acworth and M. Broadie and P. Glasserman},
  title = {{A comparison of some Monte Carlo and Quasi Monte Carlo techniques
	for option pricing}},
  booktitle = {{Monte Carlo and Quasi-Monte Carlo Methods}},
  publisher = {Springer},
  year = {1997},
  pages = {1--18},
  crossref = {NiederreiterHellekalekLarcherZinterhof},
}

@MISC{AdaptiveGaussLobatto,
  author = {W. Gander and W. Gautschi},
  title = {{Adaptive Gauss-Lobatto Quadrature}},
  howpublished = {\url{www.inf.ethz.ch/personal/gander/adaptlob.m}},
  year = {2000},
  institution = {Institut f{\"u}r Wissenschaftliches Rechnen, ETH Zentrum, 8092 Z{\"u}rich,
	Switzerland},
}

@ARTICLE{AdaptiveGaussLobattoArticle,
  author = {W. Gander and W. Gautschi},
  title = {{Adaptive Quadrature --- Revisited}},
  journal = {BIT},
  year = {2000},
  volume = {40},
  pages = {84--101},
  number = {1},
  month = {March},
  note = {CS technical report: \url{ftp.inf.ethz.ch/pub/publications/tech-reports/3xx/306.ps.gz}},
}

@ARTICLE{AfflerbachWenzel,
  author = {L. Afflerbach and K. Wenzel},
  title = {{Normal Random Numbers Lying on Spirals and Clubs}},
  journal = {Statistische Hefte},
  year = {1988},
  volume = {29},
  pages = {237--244},
}

@TECHREPORT{Akgun,
  author = {A. Akgun},
  title = {{Defaultable Security Valuation and Model Risk}},
  institution = {HEC, University of Lausanne, and FAME (International Centre for Financial
	Asset Management and Engineering), Geneva, Switzerland},
  year = {2001},
  type = {Working paper},
  note = {\url{www.risklab.ch/ftp/papers/DefaultSecurityValuation.pdf}},
}

@BOOK{Albert,
  title = {{Regression and the Moore-Penrose Pseudo-Inverse}},
  publisher = {Academic Press},
  year = {1972},
  author = {A. Albert},
}

@ARTICLE{AliMikhailHaq,
  author = {M. M. Ali and N. N. Mikhail and M. S. Haq},
  title = {{A class of bivariate distributions including the bivariate logistic}},
  journal = {Journal of Multivariate Analysis},
  year = {1978},
  volume = {8},
  pages = {405--412},
}

@ARTICLE{AllanMacLead,
  author = {A. MacLead},
  title = {{ACM Algorithm 757}},
  journal = {ACM Transactions of Mathematical Software},
  year = {1996},
  volume = {22},
  pages = {288--301},
  number = {3},
  month = {September},
  note = {\url{www.netlib.org/toms/757}},
}

@INPROCEEDINGS{Amdahl,
  author = {G. M. Amdahl},
  title = {{Validity of the Single Processor Approach to Achieving Large Scale
	Computing Capabilities}},
  booktitle = {{AFIPS Conference Proceedings}},
  year = {1967},
  pages = {483--485},
  address = {Reston, VA},
}

@ARTICLE{AndersenAndreasen,
  author = {L. Andersen and J. Andreasen},
  title = {{Volatility Skews and Extensions of the Libor Market Model}},
  journal = {Applied Mathematical Finance},
  year = {2000},
  volume = {7},
  pages = {1--32},
  number = {1},
  month = {March},
}

@ARTICLE{AndersenAndreasenEliezer,
  author = {L. B. G. Andersen and J. Andreasen and D. Eliezer},
  title = {{Static replication of barrier options: some general results}},
  journal = {Journal of Computational Finance},
  year = {2002},
  volume = {5},
  pages = {1--25},
  number = {4},
}

@ARTICLE{AndersenBermudan,
  author = {L. Andersen},
  title = {{A simple approach to the pricing of Bermudan swaptions in the multifactor
	LIBOR market model}},
  journal = {Journal of Computational Finance},
  year = {1999/2000},
  volume = {3},
  pages = {5--32},
  number = {2},
  month = {Winter},
}

@TECHREPORT{AndersenBrothertonRatcliffe,
  author = {L. Andersen and R. Brotherton-Ratcliffe},
  title = {{Extended Libor Market Models with Stochastic Volatility}},
  institution = {Gen Re Securities},
  year = {2001},
  type = {Working paper},
}

@ARTICLE{AndersenBrothertonRatcliffeSmile,
  author = {L. Andersen and R. Brotherton-Ratcliffe},
  title = {{The equity option volatility smile: An implicit finite-difference
	approach}},
  journal = {Journal of Computational Finance},
  year = {1997},
  volume = {1},
  pages = {5--38},
}

@ARTICLE{AndersenBuffum,
  author = {L. Andersen and D. Buffum},
  title = {{Calibration and implementation of convertible bond models}},
  journal = {Journal of Computational Finance},
  year = {2004},
  volume = {7},
  pages = {1--34},
  number = {2},
}

@TECHREPORT{AndersenPiterbarg2004,
  author = {L. Andersen and V. Piterbarg},
  title = {{Moment Explosions in Stochastic Volatilty Models}},
  institution = {Bank of America},
  year = {2004},
  note = {\url{ssrn.com/abstract=559481}},
  owner = {gbjaep},
}

@TECHREPORT{AndersenSidenius,
  author = {L. Andersen and J. Sidenius},
  title = {{Extensions to the Gaussian Copula: Random Recovery and Random Factor
	Loadings}},
  institution = {Bank of America},
  year = {2004},
  month = {June},
  note = {\url{www.ebusinessdesign.com/gaussextensions.pdf}},
}

@ARTICLE{AndersenSideniusBasu,
  author = {L. Andersen and J. Sidenius and S. Basu},
  title = {{All your hedges in one basket}},
  journal = {Risk},
  year = {2003},
  volume = {November},
  pages = {67--72},
}

@TECHREPORT{AndreasenDefaultSwaps,
  author = {Andreasen, J.},
  title = {{Credit Default Swap Pricing in the Par Recovery Model}},
  institution = {Gen Re Securities},
  year = {1998},
  type = {Working paper},
}

@ARTICLE{AntonovSaleev,
  author = {I. A. Antonov and V. M. Saleev},
  title = {{An economic method of computing lp-sequences}},
  journal = {USSR Computational Mathematics and Mathematical Physics},
  year = {1979},
  volume = {19},
  pages = {252--256},
  number = {1},
  key = {low-discrepancy numbers, Sobol' numbers, Gray code},
}

@ARTICLE{Avellaneda98,
  author = {M. Avellaneda},
  title = {{Minimum-relative-entropy calibration of asset pricing models}},
  journal = {International Journal of Theoretical and Applied Finance},
  year = {1998},
  volume = {1},
  pages = {442--472},
  number = {4},
}

@ARTICLE{AvellanedaBuffFriedmanGrandchampKrukNewman,
  author = {M. Avellaneda and R. Buff and C. Friedman and N. Grandchamp and L.
	Kruk and J. Newman},
  title = {{Weighted Monte Carlo: a new approach for calibrating asset-pricing
	models}},
  journal = {International Journal of Theoretical and Applied Finance},
  year = {2001},
  volume = {4},
  pages = {91--119},
  number = {1},
}

@INPROCEEDINGS{AvellanedaGamba,
  author = {M. Avellaneda and R. Gamba},
  title = {{Conquering the Greeks in Monte Carlo: Efficient Calculation of the
	Market Sensitivities and Hedge-Ratios of Financial Assets by Direct
	Numerical Simulation}},
  booktitle = {{Mathematical Finance - Bachelier Congress 2000}},
  year = {2000/2002},
  pages = {93--109},
  note = {\url{www.math.nyu.edu/faculty/avellane/ConqueringTheGreeks.pdf}},
  crossref = {2000Bachelier},
}

@ARTICLE{BDT,
  author = {F. Black and E. Derman and W. Toy},
  title = {{A one-factor model of interest rates and its apllication to treasury
	bond options}},
  journal = {Financial Analysts Journal},
  year = {1990},
  pages = {33--39},
  month = {Jan.--Feb.},
}

@BOOK{BFGLMOI,
  title = {{Modelling and Hedging Equity Derivatives}},
  publisher = {Risk Books},
  year = {1999},
  author = {O. Brockhaus and A. Ferraris and C. Gallus and D. Long and R. Martin
	and M. Overhaus},
  month = {June},
}

@BOOK{BFGLMOII,
  title = {{Equity Derivatives and Market Risk Models}},
  publisher = {Risk Books},
  year = {2000},
  author = {O. Brockhaus and M. Farkas and A. Ferraris and D. Long and M. Overhaus},
  month = {February},
}

@ARTICLE{BGK1,
  author = {M. Broadie and P. Glasserman and S. Kou},
  title = {{A continuity correction for discrete barrier options}},
  journal = {Mathematical Finance},
  year = {1997},
  volume = {7},
  pages = {325--349},
}

@ARTICLE{BGM,
  author = {A. Brace and D. Gatarek and M. Musiela},
  title = {{The Market Model of Interest Rate Dynamics}},
  journal = {Mathematical Finance},
  year = {1997},
  volume = {7},
  pages = {127--155},
  number = {2},
}

@MISC{BRODA,
  author = {S. Kucherenko and I. M. Sobol'},
  title = {{BRODA : British-Russian Offshore Development Agency}},
  howpublished = {\url{www.broda.co.uk}},
}

@ARTICLE{Baaquie1,
  author = {B. E. Baaquie},
  title = {{A Path Integral Approach to Option Pricing with Stochastic Volatility
	: Some Exact Results}},
  journal = {Journal de Physique},
  year = {1997},
  volume = {1},
  pages = {1733--1753},
  number = {7},
}

@PHDTHESIS{Bachelier,
  author = {Bachelier},
  title = {{Th{\'e}orie de la Sp{\'e}culation}},
  school = {Universit{\'e} de Paris},
  year = {1900},
}

@ARTICLE{BallandHughston,
  author = {P. Balland and L. Hughston},
  title = {{Markov Market Model consistent with Cap Smile}},
  journal = {International Journal of Theoretical and Applied Finance},
  year = {2000},
  volume = {3},
  pages = {161-181},
  number = {2},
}

@TECHREPORT{BallandImpliedVolatility,
  author = {P. Balland},
  title = {{Deterministic Implied Volatility Models}},
  institution = {Merrill Lynch International},
  year = {2001},
  type = {Working paper},
  note = {\url{www.eurandom.nl/workshops/abstracts\%20levy/ImpliedVolatilityLevyProcess.pdf}},
}

@TECHREPORT{BarkerJointCalibrationWithGenericBGM,
  author = {R. Barker},
  title = {{Joint Calibration with Generic BGM}},
  institution = {ABN AMRO},
  year = {2005},
  month = {September},
}

@TECHREPORT{BarraquandMartineau,
  author = {J. Barraquand and D. Martineau},
  title = {{Numerical Valuation of High Dimensional Multivariate American Securities}},
  institution = {Digital Equipment Corporation Research Laboratory},
  year = {1994},
  type = {Working paper},
  number = {Report 38},
  month = {April},
  note = {\url{www.smartquant.com/references/OptionPricing/option9.pdf}},
}

@ARTICLE{BarrettMooreWilmott,
  author = {J. W. Barrett and G. Moore and P. Wilmott},
  title = {{Inelegant efficiency}},
  journal = {Risk},
  year = {1992},
  volume = {5},
  pages = {82--84},
  number = {9},
}

@TECHREPORT{BassoNardonPianca,
  author = {A. Basso and M. Nardon and P. Pianca},
  title = {{Discrete monitoring corrections of American options exercise}},
  institution = {Department of Applied Mathematics, University Ca' Foscari of Venice},
  year = {2002},
  type = {Working paper},
  month = {December},
  note = {\url{www.icer.it/workshop/Basso_Nardon_Pianca.pdf}},
}

@BOOK{BaxterRennie,
  title = {{Financial Calculus}},
  publisher = {Cambridge University Press},
  year = {1996},
  author = {M. Baxter and A. Rennie},
}

@ARTICLE{BeagleholeChebanier,
  author = {D. Beaglehole and A. Chebanier},
  title = {{A two-factor mean-reverting model}},
  journal = {Risk},
  year = {2002},
  volume = {15},
  pages = {65--69},
  number = {7},
  month = {July},
}

@ARTICLE{Beckers,
  author = {S. Beckers},
  title = {{The constant elasticity of variance model and its implications for
	option pricing}},
  journal = {Journal of Finance},
  year = {1980},
  volume = {XXXV},
  pages = {661--673},
  number = {3},
  month = {June},
  key = {CEV},
}

@TECHREPORT{BenhamouMarketModelInflation,
  author = {N. Belgrade and E. Benhamou and E. Koehler},
  title = {{A Market Model For Inflation}},
  institution = {CDC Ixis Capital Markets and CNCE},
  year = {2004},
  month = {January},
  note = {\url{ssrn.com/abstract=576081}},
}

@TECHREPORT{BennaniFLM,
  author = {N. Bennani},
  title = {{The Forward Loss Model: A Dynamic Term Structure Approach 
           For The Pricing Of Portfolio Credit Derivatives}},
  institution = {The Royal Bank Of Scotland},
  year = {2005},
  month = {November},
  note = {\url{http://uk.geocities.com/nbennani@btinternet.com/_private/FLM.pdf}},
}

@ARTICLE{BerestyckiBuscaFlorent,
  author = {H. Berestycki and J. Busca and I. Florent},
  title = {{Asymptotics and calibration of local volatility models}},
  journal = {Quantitative Finance},
  year = {2002},
  volume = {2},
  pages = {61-69},
  note = {\url{www.iop.org/EJ/article/1469-7688/2/1/305/qf2105.pdf}},
}

@ARTICLE{BinomialAsDiffusion,
  author = {D. B. Nelson and K. Ramaswamy},
  title = {{Simple binomial processes as diffusion approximations in financial
	models}},
  journal = {Review of Financial Studies},
  year = {1990},
  volume = {3},
  number = {3},
}

@ARTICLE{Black76,
  author = {F. Black},
  title = {{The pricing of commodity contracts}},
  journal = {Journal of Financial Economics},
  year = {1976},
  volume = {3},
  pages = {167--179},
}

@ARTICLE{BlackCox,
  author = {F. Black and J.C.C ox},
  title = {{Valuing Corporate Securities: Some Effects of Bond Indenture Provisions}},
  journal = {Journal of Finance},
  year = {2004},
  volume = {31},
  number = {2},
}

@ARTICLE{BlackKarasinski,
  author = {F. Black and P. Karasinski},
  title = {{Bond and option pricing when short rates are lognormal}},
  journal = {Financial Analysts Journal},
  year = {1991},
  pages = {52--59},
  month = {July/August},
}

@ARTICLE{BlackScholes,
  author = {F. Black and M. Scholes},
  title = {{The Pricing of Options and Corporate Liabilities}},
  journal = {Journal of Political Economy},
  year = {1973},
  pages = {637--654},
}

@ARTICLE{Boness,
  author = {J. Boness},
  title = {{Elements of a theory of stock-option value}},
  journal = {Journal of Political Economy},
  year = {1964},
  volume = {72},
  pages = {163--175},
}

@BOOK{BorodinSalminen,
  title = {{Handbook of Brownian Motion --- Facts and Formulae}},
  publisher = {Birkh{\"a}user},
  year = {1996},
  author = {A. N. Borodin and P. Salminen},
  note = {ISBN 3-7643-5463-1},
}

@BOOK{BouchaudPotters,
  title = {{Theory of Financial Risks}},
  publisher = {Cambridge University Press},
  year = {2000},
  author = {J. P. Bouchaud and M. Potters},
}

@TECHREPORT{Bouye,
  author = {E. Bouy{\'e}},
  title = {{Copulas for Finance - A Reading Guide and Some Applications}},
  institution = {City University Business School London},
  year = {2000},
  type = {Working paper},
  note = {\url{gro.creditlyonnais.fr/content/wp/copula-survey.pdf}},
}

@ARTICLE{BoxMuller,
  author = {G. E. P. Box and M. E. Muller},
  title = {{A note on the generation of random normal deviates}},
  journal = {Annals Math. Statist.},
  year = {1958},
  volume = {29},
  pages = {610--611},
}

@MISC{Boyeretal,
  author = {B. H. Boyer and M. S. Gibson and M. Loretan},
  title = {{Pitfalls in Tests for Changes in Correlations}},
  howpublished = {International Finance Discussion paper \#597},
  month = {December},
  year = {1997},
  publisher = {The board of Governors of the Federal Reserve System},
}

@ARTICLE{Boyle1977,
  author = {P. Boyle},
  title = {{Options: a Monte Carlo approach}},
  journal = {Journal of Financial Economics},
  year = {1977},
  volume = {4},
  pages = {323--338},
  month = {May},
}

@ARTICLE{BoyleAndVorst,
  author = {P. Boyle and T. Vorst},
  title = {{Option replication in discrete time with transaction costs}},
  journal = {Journal of Finance},
  year = {1992},
  volume = {47},
  pages = {271},
}

@ARTICLE{BoyleBroadieGlasserman,
  author = {P. Boyle and M. Broadie and P. Glasserman},
  title = {{Monte Carlo Methods for Security Pricing}},
  journal = {Journal of Economic Dynamics and Control},
  year = {1997},
  volume = {21},
  pages = {1267--1322},
  number = {8--9},
}

@TECHREPORT{BoyleEvnineGibbs,
  author = {P. P. Boyle and Evnine and S. Gibbs},
  title = {{Valuation of Options on Several Underlying Assets}},
  institution = {University of Waterloo},
  year = {1988},
  type = {Working paper},
  address = {Waterloo, Ontario, Canada},
}

@TECHREPORT{BraceGoldysKlebanerWomersley,
  author = {A. Brace and B. Goldys and F. Klebaner and R. Womersley},
  title = {{Market Model of Stochastic Implied Volatility with Application to
	the Bgm Model}},
  institution = {Departmen of Statistics, University of New South Wales},
  year = {2001},
  note = {\url{www.maths.unsw.edu.au/~rsw/Finance/svol.pdf}},
}

@TECHREPORT{BraceGoldysKlebanerWomersly,
  author = {A. Brace and B. Goldys and F. Klebaner and R. Womersly},
  title = {{Market Model of Stochastic Implied Volatility with Application to
	the BGM model}},
  institution = {University of New South Wales},
  year = {2001},
  type = {Preprint},
  month = {May},
  note = {\url{www.maths.unsw.edu.au/~rsw/Finance/svol.pdf}},
}

@TECHREPORT{BraceWomersly,
  author = {A. Brace and R. Womersly},
  title = {{Exact fit to the swaption volatility matrix using semi-definite
	programming}},
  institution = {University of New South Wales},
  year = {2000},
  type = {Working paper, presented at the ICBI 2000 Global Derivatives conference},
  month = {April},
}

@BOOK{BratleyFoxSchrage,
  title = {{A Guide to Simulation}},
  publisher = {Springer},
  year = {1983},
  author = {P. Bratley and B. L. Fox and E. L. Schrage},
}

@TECHREPORT{Bray,
  author = {T. Bray and J. Paoli and C. M. Sperberg-McQueen and E. Maler and
	F Yergeau},
  title = {{Extensible Markup Language (XML) 1.0}},
  institution = {W3C},
  year = {2004},
  month = {February},
  note = {\url{www.w3.org/TR/REC-xml}},
}

@ARTICLE{BreedenLitzenberger,
  author = {D. T. Breeden and R. H. Litzenberger},
  title = {{Prices of state-contingent claims implicit in option prices}},
  journal = {Journal of Business},
  year = {1978},
  volume = {51},
  pages = {621--651},
  number = {4},
}

@ARTICLE{BrennanSchwartz,
  author = {M.J. Brennan and E.S. Schwartz},
  title = {{Analyzing convertible bonds}},
  journal = {Journal of Financial and Quantitative Analysis},
  year = {1980},
  volume = {15},
  pages = {907--929},
}

@ARTICLE{BrennanSchwartz1977,
  author = {M. Brennan and E. S. Schwartz},
  title = {{The Valuation of American Put Options}},
  journal = {Journal of Finance},
  year = {1977},
  volume = {32},
  pages = {449--462},
  month = {May},
}

@BOOK{BrigoMercurioInterestRateModels,
  title = {{Interest Rate Models: Theory and Practice}},
  publisher = {Springer},
  year = {2001},
  author = {D. Brigo and F. Mercurio},
}

@INPROCEEDINGS{BroadieAndGlassermanMilstein,
  author = {M. Broadie and P. Glasserman},
  title = {{Simulating Interest Rates to Price Term Structure Derivatives}},
  booktitle = {{Monte Carlo Seminar at Global Derivatives Conference 1997}},
  year = {1997},
}

@INPROCEEDINGS{BroadieAndGlassermanVarianceReductionReview,
  author = {M. Broadie and P. Glasserman},
  title = {{Variance Reduction Techniques}},
  booktitle = {{Global Derivatives 97}},
  year = {1997},
}

@ARTICLE{BroadieDetemple,
  author = {M. Broadie and J. Detemple},
  title = {{American Option Valuation: New Bounds, Approximations, and a Comparison
	of Existing Methods}},
  journal = {Review of Financial Studies},
  year = {1996},
  volume = {9},
  pages = {1211--1250},
  number = {4},
}

@INCOLLECTION{BroadieGlasserman2,
  author = {M. Broadie and P. Glasserman},
  title = {{Monte Carlo Methods in Option Pricing and Risk Management}},
  booktitle = {{Risk Management and Analysis: Volume 1: Measuring and Modeling Financial
	Risk}},
  pages = {173--208},
  crossref = {RiskManagementAndAnalysisI},
}

@ARTICLE{BroadieGlassermanAmerican,
  author = {M. Broadie and P. Glasserman},
  title = {{Pricing American-Style Securities Using Simulation}},
  journal = {Journal of Economic Dynamics and Control},
  year = {1997},
  volume = {21},
  pages = {1323--1352},
  number = {8--9},
}

@ARTICLE{BroadieGlassermanGreeks,
  author = {M. Broadie and P. Glasserman},
  title = {{Estimating Security Price Derivatives Using Simulation}},
  journal = {Management Science},
  year = {1996},
  volume = {42},
  pages = {269--285},
  number = {2},
}

@ARTICLE{BroadieGlassermanMC,
  author = {M. Broadie and P. Glasserman},
  title = {{Monte Carlo methods for pricing high-dimensional American options:
	An overview}},
  journal = {Net Exposure: The Electronic Journal of Financial Risk},
  year = {1997},
  volume = {1},
  pages = {15--37},
  number = {3},
  month = {December},
}

@TECHREPORT{BroadieKaya2004,
  author = {M. Broadie and {\"O}. Kaya},
  title = {{Exact Simulation of Stochastic Volatility and other Affine Jump
	Diffusion Processes}},
  institution = {Columbia University, New York},
  year = {2004},
  type = {Working paper},
  note = {\url{www.orie.cornell.edu/~aberndt/FEseminar/papers04/exact_sim_200409.pdf}},
}

@TECHREPORT{BrodyHughston,
  author = {L. Hughston and D. Brody},
  title = {{Entropic Calibration Revisited}},
  institution = {Imperial College London},
  year = {2004},
  note = {\url{www.imperial.ac.uk/research/theory/people/brody/DCB/sa10.pdf}},
}

@MISC{Brooksetal,
  author = {C. Brooks and B. Scott-Quinn and J. Whalmsey},
  title = {{Adjusting VaR Models for the impact of the Euro}},
  howpublished = {Working paper of the ISMA Centre},
  year = {1998},
  publisher = {The ACI Foundation},
}

@INCOLLECTION{BrownOnRand,
  author = {G. Brown},
  title = {{History of RAND's Random Digits --- Summary}},
  booktitle = {{Monte Carlo Method}},
  year = {1951},
  chapter = {13},
  pages = {31--32},
  month = {June},
  crossref = {NBSMonteCarloMethod},
}

@TECHREPORT{BrunnerHafner,
  author = {B. Brunner and R. Hafner},
  title = {{Arbitrage-Free Estimation of the Risk-Neutral Density from the Implied
	Volatility Smile}},
  institution = {Department of Finance and Banking, University of Augsburg, Germany},
  year = {2002/2003},
  note = {\url{www.wiwi.uni-augsburg.de/bwl/steiner/download/forschung}},
}

@ARTICLE{BuchenKelly,
  author = {P. W. Buchen and M. Kelly},
  title = {{The maximum entropy distribution of an asset inferred from option
	prices}},
  journal = {Journal of Financial and Quantitative Analysis},
  year = {1996},
  pages = {143--159},
  number = {31},
}

@TECHREPORT{CALCodingStandards,
  author = {G. Ceuppens},
  title = {{Common Analytics Library C++ Coding Standards}},
  institution = {ABN AMRO},
  year = {2003},
  month = {December},
  optannote = {https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BE4002BEE1E.nsf/h_Toc/E9839A5570CB297FC1256BF2002891D0/?OpenDocument},
}

@TECHREPORT{CALDirect,
  author = {Stephen Channell},
  title = {{Common Analytics Library Direct Design}},
  institution = {ABN AMRO},
  year = {2004},
  month = {August},
  optannote = {https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BE4002BEE1E.nsf/h_Toc/E9839A5570CB297FC1256BF2002891D0/?OpenDocument},
}

@ARTICLE{CEV,
  author = {J. C. Cox and S. A. Ross},
  title = {{The valuation of options for alternative stochastic processes}},
  journal = {Journal of Financial Economics},
  year = {1976},
  volume = {3},
  pages = {145--166},
  month = {March},
}

@MISC{CGMY,
  author = {P. Carr and H. Geman and D. Madan and M. Yor},
  title = {{The fine structure of asset returns : an empirical investigation}},
  howpublished = {\url{www.pims.math.ca/industrial/2001/financial/madan-3-9/cgmy3.pdf}},
  year = {2000},
}

@ARTICLE{CIR,
  author = {J. C. Cox and J. E. Ingersoll and S. A. Ross},
  title = {{A theory of the term structure of interest rates}},
  journal = {Econometrica},
  year = {1985},
  volume = {53},
  pages = {385--408},
}

@ARTICLE{CIR81,
  author = {J. C. Cox and J. E. Ingersoll and S. A. Ross},
  title = {{The relation between forward prices and futures prices}},
  journal = {Journal of Financial Economics},
  year = {1981},
  volume = {9},
  pages = {321--346},
  number = {4},
  month = {December},
}

@ARTICLE{CKLS,
  author = {C.K. Chan and G.A. Karolyi and F.A. Longstaff and A.B. Sanders},
  title = {{An empirical comparison of alternate models of the short-term interest
	rate}},
  journal = {Journal of Finance},
  year = {1992},
  pages = {1209--1227},
  note = {\url{www.cob.ohio-state.edu/~sanders/ckls.pdf}},
  tvolume = {57},
}

@ARTICLE{CRR,
  author = {J. C. Cox and S. A. Ross and M. Rubinstein},
  title = {{Option Pricing: A Simplified Approach}},
  journal = {Journal of Financial Economics},
  year = {1979},
  volume = {7},
  pages = {229--263},
  month = {September},
}

@ARTICLE{CaflischMorokoffOwen,
  author = {R. E. Caflisch and W. Morokoff and A. Owen},
  title = {{Valuation of Mortgage Backed Securities using Brownian Bridges to
	Reduce Effective Dimension}},
  journal = {Journal of Computational Finance},
  year = {1997},
  volume = {1},
  pages = {27--46},
  number = {1},
  month = {Fall},
}

@TECHREPORT{CalamaroNassaroFolkertslandau,
  author = {J-P. Calamaro and T. Nassar and D. Folkerts-Landau},
  title = {{CMCDS: The path to floating credit spread products}},
  institution = {Deutsche Bank},
  year = {2004},
  month = {March},
}

@ARTICLE{CambanisHuangSimons,
  author = {S. Cambanis and S. Huang and G. Simons},
  title = {{On the theory of elliptically contoured distributions}},
  journal = {Journal of Multivariate Analysis},
  year = {1981},
  volume = {11},
  pages = {368--385},
}

@BOOK{CarolAlexanderMarketModels,
  title = {{Market Models}},
  publisher = {John Wiley and Sons},
  year = {2001},
  author = {C. Alexander},
}

@ARTICLE{CarrBowie,
  author = {P. Carr and A. Bowie},
  title = {{Static Simplicity}},
  journal = {Risk},
  year = {1994},
  pages = {44--50},
  note = {\url{www.math.nyu.edu/research/carrp/papers/pdf/staticsimp.pdf}},
}

@TECHREPORT{CarrChou,
  author = {P. Carr and A. Chou},
  title = {{Hedging Complex Barrier Options}},
  institution = {Courant Institute, New York University},
  year = {1997},
  note = {\url{www.math.nyu.edu/research/carrp/papers/pdf/multipl3.pdf}},
  optannote = {Abstract: We show how several complex barrier options can be hedged
	using a portfolio of standard European options. These hedging strategies
	only involve trading at a few times during the option's life. Since
	rolling, ratchet, and lookback options can be decomposed into a portfolio
	of barrier options, our hedging results also apply to them.},
}

@ARTICLE{CarrFAQ,
  author = {P. Carr},
  title = {{Frequently Asked Questions in Option Pricing Theory}},
  journal = {Journal of Derivatives},
  year = {2004},
  note = {\url{www.math.nyu.edu/research/carrp/papers/pdf/faq2.pdf}},
}

@ARTICLE{CarrLewis,
  author = {P. Carr and K. Lewis},
  title = {{Corridor Variance Swaps}},
  journal = {Risk},
  year = {2004},
  volume = {17},
  pages = {67--72},
  number = {2},
  month = {February},
  note = {\url{www.math.nyu.edu/research/carrp/papers/pdf/RiskCVSpaper.pdf}},
}

@ARTICLE{CarrPicron,
  author = {P. Carr and J. Picron},
  title = {{Static Hedging of Timing Risk}},
  journal = {Journal of Derivatives},
  year = {1999},
  volume = {6},
  number = {3},
  month = {Spring},
  note = {\url{www.math.nyu.edu/research/carrp/papers/pdf/jodstatichedgepaper.pdf}},
  optannote = {Abstract: Many exotic options involve a payoff which occurs at the
	first passage time to a constant barrier. Although the amount to
	be paid is known, the time at which it is paid is not. This paper
	shows how a static position in vanilla European options can be used
	to hedge against this timing risk. We also show how the results can
	be used to price any barrier options.},
}

@TECHREPORT{CarrTariZariphopoulou,
  author = {P. Carr and M. Tari and T. Zariphopoulou},
  title = {{Closed Form Option Valuation with Smiles}},
  institution = {Courant Institute, New York University},
  year = {1999},
  note = {\url{www.math.nyu.edu/research/carrp/papers/pdf/closed4.pdf}},
  optannote = {Abstract: Assuming that the underlying local volatility is a function
	of stock price and time, we develop an approach for generating closed
	form solutions for option values for a certain class of volatility
	functions. The class is the set of volatility functions which solve
	the same partial differential equation as derivative security values
	in the Black Scholes model. We illustrate our results with three
	examples.},
}

@TECHREPORT{CastellaciSiclari,
  author = {G. Castellaci and M. Siclari},
  title = {{Asian basket spreads and other exotic averaging options}},
  institution = {OpenLink},
  year = {2003},
  month = {March},
  note = {\url{66.77.50.156/news/articles/exotic_options.pdf}},
}

@ARTICLE{ChebanierBeaglehole,
  author = {A. Chebanier and D. Beaglehole},
  title = {{Mean-reverting smiles}},
  journal = {Risk},
  year = {2002},
  volume = {15},
  pages = {95--98},
  number = {4},
  month = {April},
}


@BOOK{CheneyKincaid,
  title = {{Numerical Mathematics and Computing, 2nd edition}},
  publisher = {Pace Grove, California: Brooks/Cole Publishing Company, page 354},
  year = {1985},
  author = {W. Cheney and D. Kincaid},
}

@ARTICLE{ChesneyScott,
  author = {M. Chesney and L. Scott},
  title = {{Pricing European Currency Options: A comparison of the modified
	Black-Scholes model and a random variance model}},
  journal = {Journal of Financial and Quantitative Analysis},
  year = {1989},
  volume = {24},
  pages = {267--284},
  month = {September},
}

@ARTICLE{Cheyette,
  author = {O. Cheyette},
  title = {{Term Structure Dynamics and Mortgage Valuation}},
  journal = {Journal of Fixed Income},
  year = {1992},
  volume = {1},
  pages = {28--41},
}

@BOOK{Childs,
  title = {{A concrete introduction to Higher Algebra}},
  publisher = {Springer},
  year = {2000},
  author = {L. N. Childs},
  edition = {2},
  note = {ISBN 0387989994},
}

@TECHREPORT{ChryssochoosAdaptiveMonotoneCubic,
  author = {Ioannis Chryssochoos},
  title = {{Adaptive Monotone Cubic Quadrature of Integrals Involving the Gaussian Density}},
  institution = {ABN AMRO},
  year = {2005},
  month = {September},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@TECHREPORT{ChryssochoosCDOValuationModifications,
  author = {Ioannis Chryssochoos},
  title = {{CDO Valuation Modifications}},
  institution = {ABN AMRO},
  year = {2005},
  month = {August},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@TECHREPORT{ChryssochoosPhillipsRoggeFDO,
  author = {I. Chryssochoos and S. Phillips and E. Rogge},
  title = {{FDOs using the SpaceTime Copula}},
  institution = {ABN AMRO},
  year = {2005},
  month = {June},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@ARTICLE{ClarificationHittingTimesOrsteinHulenbeck,
  author = {Anja Going-Jaeschke and Marc Yor},
  title = {{A Clarification about Hitting Times Densities for Orstein-Uhlenbeck Processes}},
  note = {\url{file://nlas-00033.emea.abnamro-net.com/source/Product%20Development%20Group/Documentation/Public/AClarificationAboutHittingTimesDensitiesForOrsteinUhlenbeckProcesses.pdf}},
  year = {2002},
}

@ARTICLE{Cody,
  author = {W. J. Cody},
  title = {{Rational Chebyshev approximations for the error function}},
  journal = {Mathematics of Computation},
  year = {1969},
  pages = {631--638},
}

@TECHREPORT{CompositeBasketModel,
  author = {P. A. C. Tavares and T.-U. Nguyen and A. Chapovsky and I. Vaysburd},
  title = {{Composite Basket Model}},
  institution = {Merrill Lynch Credit Derivatives},
  year = {2004},
  type = {Working paper},
  month = {July},
  note = {\url{pedro_t.tripod.com/finance/articles/CompositeBasketModel.pdf}},
}

@ARTICLE{ContDaFonsecaDurrleman,
  author = {R. Cont and J. Da Fonseca and V. Durrleman},
  title = {{Stochastic models of implied volatility surfaces}},
  journal = {Economic notes by Banca Monte dei Paschi di Siena SpA},
  year = {2002},
  volume = {31},
  pages = {361--377},
  number = {2},
  note = {\url{www.princeton.edu/~vdurrlem/papers/ContDaFonseca.pdf}},
}

@BOOK{ContTankov,
  title = {{Financial modelling with jump processes}},
  publisher = {Chapman \& Hall / CRC},
  year = {2004},
  author = {R. Cont and P. Tankov},
}

@TECHREPORT{CorrelationRadhakrishnan,
  author = {A. R. Radhakrishnan},
  title = {{Does Correlation Matter in Pricing Caps and Swaptions?}},
  institution = {Department of Finance, Stern School of Business, New York University},
  year = {1998},
  type = {Working paper},
  address = {9-190 P, 44 West 4th Street, New York, NY 10012-1126},
  month = {September},
  note = {\url{www.stern.nyu.edu/~aradhakr}},
}

@TECHREPORT{CoxCEV,
  author = {J. C. Cox},
  title = {{Notes on option pricing I: Constant elasticity of variance diffusions}},
  institution = {{Stanford University}},
  year = {1975},
  type = {{Working paper}},
}

@ARTICLE{CozzolinoZahner,
  author = {J. M. Cozzolino and M. J. Zahner},
  title = {{The maximum entropy distribution of the future market price of a
	stock}},
  journal = {Operations Research},
  year = {1973},
  pages = {1200--1211},
}

@ARTICLE{CrankNicolson,
  author = {J. Crank and P. Nicolson},
  title = {{A practical method for numerical evaluation of solutions of partial
	differential equations of the heat-conduction type}},
  journal = {Proc. Camb. Philos. Soc.},
  year = {1947},
  volume = {43},
  pages = {50--67},
}


@MISC{CreditGrades,
  title = {{Credit Grades}},
  year = {2002},
  note = {\url{www.creditgrades.com/resources/pdf/CGtechdoc.pdf}},
  key = {CreditGrades},
}

@MISC{CygWinWebSite,
  author = {Cygnus},
  title = {{GNU utilities for Windows}},
  howpublished = {\url{www.cygwin.com}},
}

@ARTICLE{DateyGauthierSimonato,
  author = {J. Datey and G. Gauthier and J. Simonato},
  title = {{The Performance of Analytical Approximations for the Computation
	of Asian Quanto-Basket Option Prices}},
  journal = {Multinational Finance Journal},
  year = {2003},
  volume = {7},
  pages = {55--82},
  number = {1\&2},
  note = {\url{mfs.rutgers.edu/journal/post\&pdf/v7n12p3.pdf}},
}

@ARTICLE{Davis99,
  author = {M. Davis and F. Lischka},
  title = {{Convertible Bonds with Market Risk and Credit Risk}},
  journal = {Working Paper, Tokyo-Mitsubishi International.},
  year = {1999},
}

@TECHREPORT{DemertefiDermanKamalZou,
  author = {Kresimir Demeterfi and Emanuel Derman and Michael Kamal and Joseph
	Zou},
  title = {{More than you ever wanted to know about volatility swaps}},
  institution = {Goldman Sachs},
  year = {1999},
  type = {Quantitative Strategies Research Notes},
}

@TECHREPORT{DermanErgenerKani,
  author = {E. Derman and D. Ergener and I. Kani},
  title = {{Static Options Replication}},
  institution = {Goldman Sachs},
  year = {1994},
  type = {Quantitative Strategies Research Notes},
  month = {May},
}

@ARTICLE{DermanKani,
  author = {E. Derman and I. Kani},
  title = {{Stochastic Implied Trees: Arbitrage Pricing with Stochastic Term
	and Strike Structure of Volatility}},
  journal = {International Journal of Theoretical and Applied Finance},
  year = {1998},
  volume = {1},
  pages = {61--110},
  number = {1},
  month = {January},
}

@ARTICLE{DermanKaniRisk,
  author = {E. Derman and I. Kani},
  title = {{Riding on a Smile}},
  journal = {Risk},
  year = {1994},
  volume = {7},
  pages = {32--39},
  number = {2},
}

@ARTICLE{DermanKaniZou,
  author = {E. Derman and I. Kani and J. Zou},
  title = {{The Local Volatility Surface: Unlocking the Information in Option
	Prices}},
  journal = {Financial Analysts Journal},
  year = {1996},
  pages = {25--36},
  month = {July/August},
}

@BOOK{DesignPatterns,
  title = {{Design patterns : elements of reusable object-oriented software}},
  publisher = {Addison Wesley},
  year = {1995},
  author = {E. Gamma and R. Helm and R. Johnson and J. Vissides},
  note = {ISBN 0201633612},
}

@BOOK{Devroye,
  title = {{Non-Uniform Random Variate Generation}},
  publisher = {Springer},
  year = {1986},
  author = {L. Devroye},
}

@ARTICLE{DiscreteBarriers,
  author = {M. Broadie and P. Glasserman and S. Kou},
  title = {{Connecting Discrete and Continuous Path-Dependent Options}},
  journal = {Finance and Stochastics},
  year = {1999},
  volume = {3},
  pages = {55--82},
}

@ARTICLE{DisplacedDiffusion,
  author = {M. Rubinstein},
  title = {{Displaced diffusion option pricing}},
  journal = {Journal of Finance},
  year = {1983},
  volume = {38},
  pages = {213--217},
  month = {March},
}

@TECHREPORT{DisplacedDiffusionBlackKarasinskiLattice,
  author = {L. Wild and P. J{\"a}ckel},
  title = {{A Displaced-Diffusion Black-Karasinski Model for the Valuation of Credit and Interest Rate Contingent Claims}},
  institution = {ABN AMRO},
  year = {2005},
  month = {November},
  note = {\url{file://nlas-00033.emea.abnamro-net.com/source/Product%20Development%20Group/Documentation/TeX/HybridDerivatives/DisplacedBlackKarasinskiHybrid/DisplacedBlackKarasinskiHybrid.pdf}},  
}

@ARTICLE{Doob1942,
  author = {J. L. Doob},
  title = {{The Brownian Movement and Stochastic Equations}},
  journal = {The Annals of Mathematics},
  year = {1942},
  volume = {43},
  pages = {351--369},
  month = {April},
  owner = {gbjaep},
}

@ARTICLE{Doss,
  author = {H. Doss},
  title = {{Liens entre {\'e}quations diff{\'e}rentielles stochastiques ordinaires}},
  journal = {Annales de l'Institut Henrie Poincar{\'e}. Probabilit{\'e}s et Statistiques},
  year = {1977},
  volume = {13},
  pages = {99--125},
}

@ARTICLE{DouadyBarriers,
  author = {R. Douady},
  title = {{Closed Form Formulas for Exotic Options and their Lifetime Distribution}},
  journal = {International Journal of Theoretical and Applied Finance},
  year = {1998},
  volume = {2},
  pages = {17--42},
  number = {1},
  optpublisher = {World Scientific Publishing Company},
}

@TECHREPORT{DoubleCheckedLockingBroken,
  author = {D. Bacon and J. Bloch and J. Bogda and C. Click and P. Haahr and
	D. Lea and T. May and J. Maessen and J. Mitchell and K. Nilsen and
	B. Pugh and E. Sirer},
  title = {{The ``Double-Checked Locking is Broken'' Declaration}},
  institution = {IBM Research, Javasoft},
  year = {2000},
  note = {\url{www.cs.umd.edu/~pugh/java/memoryModel/DoubleCheckedLocking.html}},
}

@ARTICLE{DouglasRachford,
  author = {J. Douglas and H. H. Rachford},
  title = {{On the numerical solution of heat conduction problems in two and
	three space variables}},
  journal = {Transactions of the American Mathematical Society},
  year = {1956},
  volume = {82},
  pages = {421--439},
}

@ARTICLE{Duffee,
  author = {G.R. Duffee},
  title = {{Estimating the price of default risk}},
  journal = {Review of Financial Studies},
  year = {1999},
  volume = {12},
  pages = {197--226},
  number = {1},
  note = {\url{faculty.haas.berkeley.edu/duffee/rfs.pdf}},
}

@ARTICLE{Duffie99,
  author = {D. Duffie and K. Singleton},
  title = {{Modeling Term Structure of Defaultable Bonds}},
  journal = {Review of Financial Studies},
  year = {1999},
  volume = {12},
  pages = {687--720},
}

@TECHREPORT{DuffieCorrelatedDefaults,
  author = {D. Duffie},
  title = {{Simulating correlated defaults}},
  institution = {Graduate School of Business},
  year = {1998},
  type = {Working paper},
  month = {September},
  note = {\url{www.stanford.edu/~duffie/cor_def.pdf}},
}

@TECHREPORT{DuffieFirstToDefault,
  author = {D. Duffie},
  title = {{First-to-Default Valuation}},
  institution = {Graduate School of Business, Stanford University and Universit{\'e}
	de Paris, Dauphine},
  year = {1998},
  month = {May},
  note = {\url{www.stanford.edu/~duffie/first.pdf}},
}

@ARTICLE{DuffiePanSingleton,
  author = {D. Duffie and J. Pan and K. Singleton},
  title = {{Transform Analysis and Asset Pricing for Affine Jump Diffusions}},
  journal = {Econometrica},
  year = {2000},
  volume = {68},
  pages = {1343--1376},
}

@ARTICLE{Dupire,
  author = {B. Dupire},
  title = {{Pricing with a Smile}},
  journal = {Risk},
  year = {1994},
  volume = {7},
  pages = {18--20},
  number = {1},
}

@BOOK{DupireMC,
  title = {{Monte Carlo: Methodologies and Applications for Pricing and Risk
	Management}},
  publisher = {Risk Publications},
  year = {1998},
  editor = {B. Dupire},
}

@ARTICLE{EJWatson,
  author = {E. J. Watson},
  title = {{Primitive polynomials (mod 2)}},
  journal = {Mathematics of Computation},
  year = {1962},
  volume = {16},
  pages = {368--369},
  number = {79},
  month = {July},
}

@ARTICLE{EMBrownianBridge,
  author = {W. Morokoff},
  title = {{The {{Brownian}} bridge {{E-M}} algorithm for covariance estimation
	with missing data}},
  journal = {Journal of Computational Finance},
  year = {1998/1999},
  volume = {2},
  pages = {75--100},
  number = {2},
  month = {Winter},
}

@article{Einstein1905,
		 author={Einstein, A.},
		 title={{{\"U}ber die von der molekularkinetischen Theorie der W{\"a}rme geforderte Bewegung von in ruhenden Fl{\"u}ssigkeiten suspendierten Teilchen}},
		 journal={{Annalen der Physik}},
		 volume={17},
		 year= 1905,
		 pages={549--560}
}

@ARTICLE{EmanuelMacBeth,
  author = {D. C. Emanuel and J. D. MacBeth},
  title = {{Further results on the constant elasticity of variance call option
	pricing model}},
  journal = {Journal of Financial and Quantitative Analysis},
  year = {1982},
  pages = {533--554},
  optkey = {CEV},
}

@TECHREPORT{EmbrechtsLindskogMcNeil,
  author = {P. Embrechts and F. Lindskog and A. McNeil},
  title = {{Modelling Dependence with Copulas and Applications to Risk Management}},
  institution = {Department of Mathematics, ETHZ CH-8092, Z{\"u}rich, Switzerland},
  year = {2001},
  type = {Working paper},
  note = {\url{www.risklab.ch/ftp/papers/DependenceWithCopulas.pdf}},
  optmonth = {April 6},
}

@BOOK{Erdelyi,
  title = {{Asymptotic Expansions}},
  publisher = {Dover},
  year = {1987},
  author = {A. Erd{\'e}lyi},
}

@BOOK{Euler1768,
  title = {{Theoria motuum lunae nova methodo pertractata}},
  year = {1768},
  author = {L. Euler},
  owner = {gbjaep},
}

@BOOK{Euler1768a,
  title = {{Institutiones Calculi Integralis}},
  year = {1768},
  author = {L. Euler},
  owner = {gbjaep},
}

@TECHREPORT{Expat,
  author = {James Clark},
  title = {{Expat -- an XML Parser Toolkit}},
  institution = {Thai Open Source Software},
  year = {2000},
  note = {\url{www.jclark.com/xml/expat.html}},
}

@ARTICLE{FFTOptionValuation,
  author = {P. Carr and D.B. Madan},
  title = {{Option valuation using the fast {{Fourier}} transform}},
  journal = {Journal of Computational Finance},
  year = {1999},
  volume = {2},
  pages = {61--73},
  number = {4},
}

@ARTICLE{FLLLT,
  author = {E. Fourni{\'e} and J. M. Lasry and J. Lebuchoux and P. L. Lions and
	N. Touzi},
  title = {{Applications of {{M}}alliavin Calculus to {{M}}onte {{C}}arlo Methods
	in Finance}},
  journal = {Finance \& Stochastics},
  year = {1999},
  volume = {3},
  pages = {391--412},
  number = {4},
  abstract = {This paper presents an original probabilistic method for the numerical
	computations of Greeks (i.e. price sensitivities) in finance. Our
	approach is based on the \emph{integration-by-parts} formula, which
	lies at the core of the theory of variational stochastic calculus,
	as developed in the Malliavin calculus. The Greeks formulae, both
	with respect to initial conditions and for smooth perturbations of
	the local volatility, are provided for general discontinuous path-dependent
	payoff functionals of multidimensional diffusion processes. We illustrate
	the results by applying the formula to exotic European options in
	the framework of the Black and Scholes model. Our method is compared
	to the Monte Carlo finite difference approach and turns out to be
	very efficient in the case of discontinuous payoff functionals.},
}

@ARTICLE{FLLLT2,
  author = {E. Fourni{\'e} and J. M. Lasry and J. Lebuchoux and P. L. Lions},
  title = {{Applications of {{M}}alliavin Calculus to {{M}}onte {{C}}arlo Methods
	in Finance II}},
  journal = {Finance \& Stochastics},
  year = {2001},
  volume = {5},
  pages = {201--236},
  number = {2},
}

@ARTICLE{FangFangRosen,
  author = {K. Fang and H. Fang and D. von Rosen},
  title = {{A family of bivariate distributions with non-elliptical contours}},
  journal = {Communications in Statistics - Theory and Methods},
  year = {2000},
  volume = {29},
  pages = {1885--1898},
}

@ARTICLE{Feller51,
  author = {W. Feller},
  title = {{Two Singular Diffusion Problems}},
  journal = {Annals of Mathematics},
  year = {1951},
  volume = {54},
  pages = {173--182},
}

@ARTICLE{Feynman,
  author = {R. Feynman},
  title = {{Space-time approach to non-relativistic quantum mechanics}},
  journal = {Rev. Mod. Phys.},
  year = {1948},
  volume = {20},
  pages = {367--387},
}

@ARTICLE{Finger,
  author = {C. Finger},
  title = {{A Methodology for Stress Correlation}},
  journal = {RiskMetrics Monitor},
  year = {1997},
  pages = {3--11},
  month = {Fourth Quarter},
}

@ARTICLE{FingerComparison,
  author = {Christopher C. Finger},
  title = {{A Comparison of Stochastic Default Rate Models}},
  journal = {RiskMetrics Journal},
  year = {2000},
  pages = {49--73},
  month = {November},
  note = {\url{www.riskmetrics.com/pdf/journals/rmj4q00.pdf}},
  abstract = {Collateralized Debt Obligations have sparked interest in portfolio
	default models over multiple horizons. For these, in contrast to
	single period models, there is little understanding of the impact
	of model assumptions. We investigate four multiple horizon models,
	each calibrated to the same set of input data. Our results show a
	significant disparity, showing that the issue of model choice is
	more consequential here than in the single period case.},
}

@ARTICLE{FisherCorrelation,
  author = {R. A. Fisher},
  title = {{Frequency distribution of the values of the correlation coefficient
	in samples from an indefinitely large population}},
  journal = {Biometrika},
  year = {1915},
  volume = {10},
  pages = {507--521},
}

@BOOK{Fishman96,
  title = {{Monte Carlo: Concepts, Algorithms, and Applications}},
  publisher = {Springer},
  year = {1996},
  author = {G. Fishman},
  note = {ISBN 038794527X},
  description = {This volume presents a comprehensive first course in the Monte Carlo
	method, suitable for graduate and undergraduate students in the mathematical
	sciences and engineering, principally operations research, statistics,
	mathematics and computer science. The reader is assumed to have a
	sound understanding of calculus, introductory matrix analysis and
	intermediate statistics, but otherwise the book is self-contained.
	As well as an exploration of all the important concepts of the Monte
	Carlo method, the volume includes over 75 algorithms which allow
	the reader to move rapidly from the concepts to putting them into
	practice. The book also contains numerous exercises, many of which
	employ hands-on implementation of selected algorithms to demonstrate
	the application of these ideas in realistic settings.},
}

@BOOK{ForsytheMalcolm,
  title = {{Computer Methods for Mathematical Computations}},
  publisher = {Prentice-Hall},
  year = {1977},
  author = {G. E. Forsythe and M. A. Malcolm and C. B. Moler},
  address = {Englewood Cliffs, NJ},
}

@INCOLLECTION{ForsytheOnNumberTesting,
  author = {G. E. Forsythe},
  title = {{Generation and Testing of Random Digits at the National Bureau of
	Standards, Los Angeles}},
  booktitle = {{Monte Carlo Method}},
  year = {1951},
  chapter = {12},
  pages = {34--35},
  month = {June},
  crossref = {NBSMonteCarloMethod},
}

@BOOK{Fouque,
  title = {{Derivatives in Financial Markets with Stochastic Volatility}},
  publisher = {Cambridge University Press},
  year = {2000},
  author = {J.-P. Fouque and G. Papanicolaou and K. R. Sircar},
  month = {September},
  note = {ISBN 0521791634},
}

@TECHREPORT{Fox96generating,
  author = {B. L. Fox},
  title = {{Generating Poisson processes by quasi-Monte Carlo}},
  institution = {SIM-OPT Consulting, 872 Timber Lane, Boulder, CO 80304},
  year = {1996},
  type = {Technical report},
  note = {\url{citeseer.nj.nec.com/cache/papers/cs/4246/http:zSzzSzwww.math.hkbu.edu.hkzSzqmczSzgpp.pdf/fox96generating.pdf}},
}

@INPROCEEDINGS{FreesValdez,
  author = {E. W. Frees and E. A. Valdez},
  title = {{Understanding Relationships using Copulas}},
  booktitle = {{32nd Actuarial Research Conference}},
  year = {1997},
  address = {Calgary, Alberta, Canada},
  month = {August 6--8},
  organization = {School of Business, University of Wisconsin, Madison, 975 University
	Avenue, Madison, Wisconsin 53706},
  note = {\url{www.soa.org/library/naaj/1997-09/naaj9801_1.pdf}},
}

@MISC{FrizMalliavin,
  author = {P. Friz},
  title = {{Malliavin Calculus in Finance}},
  howpublished = {Courant Institute, New York University},
  year = {2002},
  note = {\url{www.math.nyu.edu/fellows_fin_math/gatheral/malliavin2003.pdf}},
}

@TECHREPORT{FultonJacobsRainbow,
  author = {Nic Fulton and Andrew Jacobs and Marcus Rainbow et al.},
  title = {{Financial products Markup Language (FpML) Architecture version 1.0}},
  institution = {Reuters, IBM et al.},
  year = {2001},
  month = {March},
  note = {\url{xml.coverpages.org/FpMLrec-arch-1-0-2001-03-16-1.pdf}},
}

@ARTICLE{GB2,
  author = {R. M. Bookstaber and J. B. McDonald},
  title = {{A General Distribution for Describing Security Price Returns}},
  journal = {Journal of Business},
  year = {1987},
  volume = {60},
  pages = {401--424},
  number = {3},
  month = {July},
  note = {University of Chicago Press},
  abstract = {This paper introduces a generalized distribution, called the GB2 distribution,
	for describing security returns. The distribution is extremely flexible,
	containing a large number of well-known distributions, such as the
	lognormal, log-t, and log-Cauchy distribu tions, as special or limiting
	cases and allowing large, even infinite, higher moments. This flexibility
	allows a direct representation of different degrees of fat tails
	in the distribution. The properties of the GB2 make it useful in
	empirical estimation of security returns and in facilitating the
	development of option-pricing models and other models that depend
	on the specification and mathematical manipulation of distributions.},
}

@ARTICLE{GB2Cummins,
  author = {J. D. Cummins and G. Dionne and J. B. McDonald},
  title = {{Application of the GB2 family of distributions in modeling insurance
	loss processes}},
  journal = {Insurance: Mathematics and Economics},
  year = {1990},
  volume = {9},
  pages = {257--272},
}

@ARTICLE{GainesLyons1994,
  author = {J.G. Gaines and T.J. Lyons },
  title = {{Random Generation of Stochastic Area Integrals}},
  journal = {SIAM Journal on Applied Mathematics},
  year = {1994},
  volume = {54},
  pages = {1132--1146},
  number = {4},
  owner = {gbjaep},
}

@BOOK{Gander,
  title = {{Computermathematik}},
  publisher = {Birkh{\"a}user},
  year = {1992},
  author = {W. Gander},
  note = {ISBN 3764327650},
}

@ARTICLE{GarmanKohlhagen,
  author = {M. B. Garman and S. W. Kohlhagen},
  title = {{Foreign Currency Option Values}},
  journal = {Journal of International Money and Finance},
  year = {1983},
  volume = {2},
  pages = {231--237},
  month = {December},
}

@MISC{GatheralLectureNotes,
  author = {J. Gatheral},
  title = {{Case Studies in Financial Modelling}},
  howpublished = {Courant Institute, New York University},
  year = {2002},
  note = {\url{www.math.nyu.edu/fellows_fin_math/gatheral/case_studies.html}},
}

@ARTICLE{GemanYor1993,
  author = {H. Geman and M. Yor},
  title = {{Bessel Processes, Asian Options, and Perpetuities}},
  journal = {Mathematical Finance},
  year = {1993},
  volume = {3},
  pages = {349--375},
  owner = {gbjaep},
}

@ARTICLE{GeneralOneFactorClass,
  author = {W. M. Schmidt},
  title = {{On a general class of one factor models for the term structure of
	interest rates}},
  journal = {Finance and Stochastics},
  year = {1997},
  volume = {1},
  number = {1},
}

@ARTICLE{GeneralisedLambda,
  author = {J. S. Ramberg and B. W. Schmeiser},
  title = {{An approximate method for generating asymmetric random variables}},
  journal = {Communications of the ACM},
  year = {1974},
  volume = {17},
  pages = {78--82},
}

@ARTICLE{GeneralisedLambda2,
  author = {J. S. Ramberg and E. J. Dudewicz and P. R. Tadikamalla and E. F.
	Mykytka},
  title = {{A Probability Distribution and Its Uses in Fitting Data}},
  journal = {Technometrics},
  year = {1979},
  volume = {21},
  pages = {201--214},
  number = {2},
  month = {May},
}

@ARTICLE{GeneralisedLambda3,
  author = {M. Freimer and G. S. Mudholkar and G. Kollia and C. T. Lin},
  title = {{A study of the generalized Tukey lambda family}},
  journal = {Communications in Statistics --- Theory and Methods},
  year = {1988},
  volume = {17},
  pages = {3547--3567},
  note = {A web applet showing the distribution for different parameters can
	be found at \url{www.ens.gu.edu.au/robertk/gld/}},
}

@ARTICLE{GeneralisedLambda4,
  author = {Z. E. Karian and E. J. Dudewicz and P. McDonald},
  title = {{The extended generalized lambda distribution system for fitting
	distributions to data: history, completion of theory, tables, applications,
	the ``Final Word'' on Moment fits}},
  journal = {Communications in Statistics --- Simulation and Computation},
  year = {1996},
  volume = {25},
  pages = {611--642},
}

@TECHREPORT{GenestRivest,
  author = {C. Genest and L. Rivest},
  title = {{On the multivariate probability integral transformation}},
  institution = {D{\'e}partement de math{\'e}matiques et de statistique, Universit{\'e}
	Laval, Que{\'e}bec, Canada, G1K 7P4},
  year = {2000},
  type = {Working paper},
  month = {July},
  note = {\url{www.mat.ulaval.ca/pages/genest/k.pdf}},
}

@ARTICLE{Geske,
  author = {R. Geske},
  title = {{The Valuation of Compound Options}},
  journal = {Journal of Financial Economics},
  year = {1979},
  volume = {7},
  pages = {63--81},
}

@ARTICLE{GeskeJohnsonAmerican,
  author = {R. Geske and H. E. Johnson},
  title = {{The American put option valued analytically}},
  journal = {Journal of Finance},
  year = {1984},
  volume = {39},
  pages = {1511--1524},
  number = {5},
}

@ARTICLE{GeskeJohnsonLeverage,
  author = {R. Geske and H. E. Johnson},
  title = {{The Valuation of Corporate Liabilities as Compound Options: A Correction}},
  journal = {Journal of Financial and Quantitative Analysis},
  year = {1984},
  volume = {19},
  pages = {231--232},
}

@ARTICLE{GeskeLeverage,
  author = {R. Geske},
  title = {{The Valuation of Corporate Liabilities as Compound Options}},
  journal = {Journal of Financial and Quantitative Analysis},
  year = {1977},
  volume = {12},
  pages = {541--552},
}

@TECHREPORT{GincbergMurexInflation,
  author = {E. Gincberg},
  title = {{CPI Seasonality Configuration in Murex}},
  institution = {ABN AMRO},
  year = {2005},
  month = {July},
  }

@TECHREPORT{GincbergNotesOnDailyQuantoOptionsWithVolatilitySkew,
  author = {E. Gincberg},
  title = {{Notes On the Valuation of Daily Quanto Options in presence of Volatility Skew}},
  institution = {ABN AMRO},
  year = {2005},
  month = {December},
  note = {\url{file://nlas-00033.emea.abnamro-net.com/source/Product%20Development%20Group/Documentation/TeX/NotesOnDailyQuantoOptionsWithVolatilitySkew/NotesOnDailyQuantoOptionsWithVolatilitySkew.pdf}},
}

@TECHREPORT{GincbergRatioOrOrProductsOfAsianBaskets,
  author = {E. Gincberg},
  title = {{Options on Ratios or Products of Asian Baskets}},
  institution = {ABN AMRO},
  year = {2005},
  month = {July},
  note = {\url{file://nlas-00033.emea.abnamro-net.com/source/Product%20Development%20Group/Documentation/TeX/OptionsOnRatiosOrProductsOfAsianBaskets/OptionsOnRatiosOrProductsOfAsianBaskets.pdf}},	
}

@BOOK{Glasserman,
  title = {{Monte Carlo Methods in Financial Engineering}},
  publisher = {Springer},
  year = {2003},
  author = {P. Glasserman},
}

@TECHREPORT{GlassermanMerener2002,
  author = {P. Glasserman and N. Merener},
  title = {{Cap and swaption approximations in LIBOR Market Models with Jumps}},
  institution = {Columbia University},
  year = {2002},
  type = {Working paper},
  note = {\url{www-1.gsb.columbia.edu/faculty/pglasserman/Other/swaption.pdf}},
}

@ARTICLE{GlassermanMerener2003,
  author = {P. Glasserman and N. Merener},
  title = {{Numerical solution of jump-diffusion LIBOR market models}},
  journal = {Finance and Stochastics},
  year = {2003},
  volume = {7},
  pages = {1--27},
  number = {1},
}

@ARTICLE{GlassermanZhao,
  author = {P. Glasserman and X. Zhao},
  title = {{Fast greeks by simulation in forward Libor models}},
  journal = {Journal of Computational Finance},
  year = {1999},
  volume = {3},
  pages = {5--39},
  number = {1},
  month = {Fall},
}

@ARTICLE{Golub,
  author = {G. H. Golub and W. Kahan},
  title = {{Calculating The Singular Values and Pseudo-Inverse of a Matrix}},
  journal = {SIAM. Numer. Anal. ser B 2},
  year = {1965},
  pages = {205--224},
}

@BOOK{GolubVanLoan,
  title = {{Matrix Computations}},
  publisher = {The John Hopkins University Press},
  year = {1983,1989,1996},
  author = {G. H. Golub and C. F. Van Loan},
}

@BOOK{GoverBarnett,
  title = {{Applications of Matrix Theory}},
  publisher = {Oxford University Press},
  year = {1989},
  editor = {M. J. C. Gover and S. Barnett},
}

@ARTICLE{GreeksWithMonteCarloPJ,
  author = {P. J{\"a}ckel},
  title = {{Greeks with Monte Carlo}},
  journal = {Wilmott},
  year = {2001},
  month = {May},
  pages = {55--63}
}

@ARTICLE{GregoryLaurentOctober2004,
  author = {J. Gregory and J.-P. Laurent},
  title = {{In the core of correlation}},
  journal = {Risk},
  year = {2004},
  pages = {87--91},
  month = {October},
}

@BOOK{GuHo,
  title = {{Nonlinear Oscillations, Dynamical Systems, and Bifurcations of Vector
	Fields}},
  publisher = {Springer},
  year = {1983},
  author = {J. Guckenheimer and P. Holmes},
  volume = {42},
  series = {Applied Mathematical Sciences},
}

@ARTICLE{GuptaSubrahmanyam,
  author = {A. Gupta and M.G. Subrahmanyam},
  title = {{An Empirical Examination of the Convexity Bias in the Pricing of
	Interest Rate Swaps}},
  journal = {Journal of Financial Economics},
  year = {2000},
  volume = {55},
  pages = {239--279},
  number = {2},
  month = {February},
  note = {\url{www.stern.nyu.edu/fin/workpapers/papers99/wpa99001.pdf}},
}

@ARTICLE{Gustafson,
  author = {J. L. Gustafson},
  title = {{Re-evaluating Amdahl's Law}},
  journal = {Communications of the ACM},
  year = {1988},
  volume = {31},
  pages = {532--533},
  number = {5},
  month = {May},
}

@ARTICLE{HJM,
  author = {D. Heath and R. Jarrow and A. Morton},
  title = {{Bond pricing and the term structure of interest rates}},
  journal = {Econometrica},
  year = {1992},
  volume = {61},
  pages = {77--105},
  number = {1},
}

@ARTICLE{HJM0,
  author = {D. Heath and R. Jarrow and A. Morton},
  title = {{Bond pricing and the term structure of interest rates: a discrete
	time approximation}},
  journal = {Journal of Financial and Quantitative Analysis},
  year = {1990},
  volume = {25},
  pages = {419--440},
  number = {4},
  month = {December},
}

@ARTICLE{HN1,
  author = {H. Niederreiter},
  title = {{Low-Discrepancy and Low-Dispersion Sequences}},
  journal = {Journal of Number Theory},
  year = {1988},
  volume = {30},
  pages = {51--70},
}

@ARTICLE{HN2,
  author = {H. Niederreiter},
  title = {{Low-Discrepancy Sequences and Global Function Fields with Many Rational
	Places}},
  journal = {Finite Fields and their Applications},
  year = {1996},
  volume = {2},
  pages = {241--273},
}

@BOOK{HNBook,
  title = {{Random Number Generation and Quasi-Monte Carlo Methods}},
  publisher = {Society for Industrial and Applied Mathematics (SIAM)},
  year = {1992},
  author = {H. Niederreiter},
}

@TECHREPORT{HaganCredit,
  author = {P.S. Hagan},
  title = {{Summary of standard credit derivatives -- working draft}},
  institution = {Bloomberg LLP},
  year = {2005},
}

@INCOLLECTION{HammerOnMidSquare,
  author = {P. C. Hammer},
  title = {{The Mid-Square Method of Generating Digits}},
  booktitle = {{Monte Carlo Method}},
  year = {1951},
  chapter = {11},
  pages = {33},
  month = {June},
  crossref = {NBSMonteCarloMethod},
}

@TECHREPORT{HarrisHahn,
  author = {M. Harris and P. Hahn},
  title = {{Credit Option Pricing Model}},
  institution = {JPMorgan},
  year = {2004},
  month = {October},
}

@BOOK{Harrison,
  title = {{Brownian motion and stochastic flow systems}},
  publisher = {Wiley, Krieger},
  year = {1985, 1990},
  author = {J. Michael Harrison},
  note = {ISBN 0-89464-455-6},
}

@ARTICLE{HarrisonPliska,
  author = {J. M. Harrison and S. Pliska},
  title = {{Martingales and stochastic integrals in the theory of continuous
	trading}},
  journal = {Stochastic processes and their applications},
  year = {1981},
  volume = {11},
  pages = {215--260},
}

@BOOK{Haug,
  title = {{The Complete Guide to Option Pricing Formulas}},
  publisher = {McGraw-Hill},
  year = {1997},
  author = {E. G. Haug},
  month = {October},
  note = {ISBN 0786312408},
}

@TECHREPORT{HawkinsFrieden,
  author = {R. Hawkins and R. Frieden},
  title = {{Financial Probabilities from Fisher Information}},
  institution = {Mulsanne Capital Management / Optical Sciences Center of the University
	of Arizona},
  year = {2003},
  type = {Working paper},
  month = {February},
  note = {\url{arxiv.org/pdf/cond-mat/0302579}},
}

@ARTICLE{HeathCoherentRiskMeasures,
  author = {F. Delbaen and J. M. Eber and D. Heath},
  title = {{Thinking Coherently}},
  journal = {Risk},
  year = {1997},
  volume = {10},
  number = {11},
  month = {November},
}

@ARTICLE{HeathJarrowMorton,
  author = {D. Heath and R. Jarrow and A. Morton},
  title = {{Bond pricing and the term structure of interest rates: A new methodology}},
  journal = {Econometrica},
  year = {1992},
  volume = {60},
  pages = {77--105},
  number = {1},
}

@BOOK{HellekalekLarcher,
  title = {{Random and Quasi-Random Point Sets}},
  publisher = {Springer},
  year = {1998},
  editor = {P. Hellekalek and G. Larcher},
  volume = {138},
  series = {Lecture Notes in Statistics},
  note = {ISBN 0387985549},
}

@INCOLLECTION{HestonRisk,
  author = {Steven L. Heston},
  title = {{A closed-form solution for options with stochastic volatility with
	applications to bond and currency options}},
  booktitle = {{Volatility}},
  publisher = {Risk publications},
  year = {1998},
  pages = {341--349},
  month = {June},
}

@ARTICLE{Hestona,
  author = {S. L. Heston},
  title = {{A closed-form solution for options with stochastic volatility with
	applications to bond and currency options}},
  journal = {The Review of Financial Studies},
  year = {1993},
  volume = {6},
  pages = {327--343},
}

@ARTICLE{Hestonb,
  author = {S. L. Heston},
  title = {{Invsible parameters in option prices}},
  journal = {Journal of Finance},
  year = {1993},
  volume = {48},
  pages = {933--947},
}

@TECHREPORT{Hestonc,
  author = {S. L. Heston},
  title = {{Yield curves and volatility}},
  institution = {Washington University},
  year = {1993},
  type = {Working paper},
  address = {St Louis, MO},
}

@ARTICLE{Higham,
  author = {N. J. Higham},
  title = {{Computing the Nearest Correlation Matrix - A Problem from Finance}},
  journal = {IMA Journal of Numerical Analysis},
  year = {2002},
  volume = {22},
  pages = {329--343},
  note = {\url{www.ma.man.ac.uk/~nareports/narep369.pdf}},
}

@ARTICLE{HoLee,
  author = {T. S. Y. Ho and S.-B. Lee},
  title = {{Term structure movements and pricing interest rate contingent claims}},
  journal = {Journal of finance},
  year = {1986},
  volume = {41},
  pages = {1011--1029},
  month = {December},
}

@TECHREPORT{HoganWeintraub,
  author = {M. Hogan and K. Weintraub},
  title = {{The Lognormal Interest Rate Model and Eurodollar Futures}},
  institution = {Citibank},
  year = {1993},
  type = {Discussion paper},
  address = {New York},
}

@BOOK{Hollingdale,
  title = {{High Speed Computing: Methods and Applications}},
  publisher = {The English Univerisity Press LTD},
  year = {1959},
  author = {S. H. Hollingdale},
  address = {102 Newgate Street, London EC1},
}

@BOOK{Householder,
  title = {{The Numerical Treatment of a Single Nonlinear Equation}},
  publisher = {McGraw-Hill New York},
  year = {1970},
  author = {A. S. Householder},
}

@BOOK{Hull,
  title = {{Options, Futures, and Other Derivatives}},
  publisher = {Prentice Hall},
  year = {1989,1993,1997},
  author = {John Hull},
}

@TECHREPORT{Hull00,
  author = {J. Hull and A. White},
  title = {{Valuing Credit Default Swaps II: Modeling Default Correlations}},
  institution = {University of Toronto},
  year = {2000},
  type = {Working paper},
  note = {\url{www.rotman.utoronto.ca/~hull/DownloadablePublications/CredDefSw2.pdf}},
}

@TECHREPORT{HullPredescuWhiteCorrelationUsingStructural,
  author = {J. Hull and M. Predescu and A. White},
  title = {{The valuation of correlation-dependent credit derivatives using
	a structural model}},
  institution = {University of Toronto},
  year = {2005},
  type = {Working paper},
  month = {March},
  note = {\url{www.rotman.utoronto.ca/~hull/DownloadablePublications/StructuralModel.pdf}},
}

@ARTICLE{HullWhite,
  author = {J. Hull and A. White},
  title = {{Pricing interest rate derivative securities}},
  journal = {Review of Financial Studies},
  year = {1990},
  volume = {3},
  pages = {573--592},
  number = {4},
}

@TECHREPORT{HullWhiteCorrelatedTimeOfDefault,
  author = {J. Hull and A. White},
  title = {{Valuation of a CDO and an n-th to Default CDS Without Monte Carlo
	Simulation}},
  institution = {University of Toronto},
  year = {2003},
  type = {Working paper},
  note = {\url{www.rotman.utoronto.ca/~hull/DownloadablePublications/HullWhiteCDOPaper.pdf}},
}

@TECHREPORT{HullWhiteCreditDefaultSwapsAndSwaptions,
  author = {J. Hull and A. White},
  title = {{The Valuation of Credit Default Swap Options}},
  institution = {Joseph L. Rotman School of Management, University of Toronto},
  year = {2002},
  type = {Working paper},
  month = {September},
  note = {\url{www.rotman.utoronto.ca/~hull/DownloadablePublications/HullWhiteCDSoptionspaper.pdf}},
}

@BOOK{HullWhiteOnDerivatives,
  title = {{Hull-White on Derivatives}},
  publisher = {Risk Publications},
  year = {1996},
  editor = {J. Hull and A. White},
  note = {ISBN 1 899332 45 6},
}

@ARTICLE{HullWhiteStochasticVolatility,
  author = {J. Hull and A. White},
  title = {{An Analysis of the Bias in Option Pricing Caused by a Stochastic
	Volatility}},
  journal = {Advances in Futures and Options Research},
  year = {1988},
  volume = {3},
  pages = {27--61},
}

@ARTICLE{HullWhiteStochasticVolatilityModel,
  author = {J. Hull and A. White},
  title = {{The Pricing of Options on Assets with Stochastic Volatilities}},
  journal = {Journal of Finance},
  year = {1987},
  volume = {42},
  pages = {281--300},
  number = {2},
  month = {June},
  note = {\url{faculty.baruch.cuny.edu/lwu/890/HullWhite87.pdf}},
}

@ARTICLE{HullWhiteSwaptionVolatility,
  author = {J. Hull and A. White},
  title = {{Forward rate volatilities, swap rate volatilities, and the implementation
	of the {{LIBOR}} market model}},
  journal = {Journal of Fixed Income},
  year = {2000},
  volume = {10},
  pages = {46--62},
  number = {2},
  month = {September},
}

@BOOK{HuntKennedy,
  title = {{Financial Derivatives in Theory and Practice}},
  publisher = {John Wiley and Sons},
  year = {2000},
  author = {P. J. Hunt and J. E. Kennedy},
}

@ARTICLE{HunterJaeckelJoshi,
  author = {C. Hunter and P. J{\"a}ckel and M. Joshi},
  title = {{Getting the Drift}},
  journal = {Risk},
  year = {2001},
  month = {July},
  note = {\url{www.quarchome.org/MarketModelPredictorCorrector.pdf}},
}


@ARTICLE{Hyman,
  author = {J. M. Hyman},
  title = {{Accurate Monotonicity Preserving Cubic Interpolation}},
  journal = {SIAM Journal on Scientific and Statistical Computing},
  year = {1983},
  volume = {4},
  pages = {645--653},
  number = {4},
}


@MISC{ISDA,
  author = {ISDA},
  title = {{International Swap Dealers Association master agreements}},
  note = {\url{www.isda.org/publications/isdamasteragrmnt.html}},
}

@MISC{ITL,
  author = {A. Lumsdaine and L. Lee and J. Siek},
  title = {{The iterative template library}},
  note = {\url{www.osl.iu.edu/research/itl}},
  key = {ITL},
}

@MISC{InflationHICPXTBreakEvenDataSet,
  title = {{Data Set of Daily Broker HICPXT Break Even Quotes 2002-2006}},
  note = {\url{file://nlas-00033.emea.abnamro-net.com/source/Product%20Development%20Group/Documentation/TeX/InflationDistributionFitting/HICPXTSwapsHistoricalData.xls}},
}

@ARTICLE{Ingersoll,
  author = {J. E. Ingersoll},
  title = {{Approximating American options and other financial contracts using
	barrier derivatives}},
  journal = {Journal of Computational Finance},
  year = {1998},
  volume = {2},
  pages = {85--112},
  number = {1},
}

@ARTICLE{InuiKijima,
  author = {K. Inui and M. Kijima},
  title = {{A Markovian framework in multi-factor Heath-Jarrow-Morton models}},
  journal = {Journal of Financial and Quantitative Analysis},
  year = {1998},
  volume = {33},
  pages = {423--440},
  number = {3},
}

@ARTICLE{JacksonSueliHowison,
  author = {N. Jackson and Endre S{\"uli} and S. Howison},
  title = {{Computation of deterministic volatility surfaces}},
  journal = {Journal of Computational Finance},
  year = {1998},
  volume = {2},
  pages = {5--32},
  number = {2},
}

@MISC{Jaeckel2002,
  author = {P. J{\"a}ckel},
  title = {{The handling of continuous barriers for derivatives on many underlyings}},
  month = {November 26},
  year = {2002},
  note = {\url{www.jaeckel.org/TheHandlingOfContinuousBarriersForDerivativesOnManyUnderlyings.pdf}},
  type = {Quantitative Finance London Conference},
}

@INPROCEEDINGS{Jaeckel2004,
  author = {P. J{\"a}ckel},
  title = {{Stochastic volatility models - past, present, and future}},
  year = {2004},
  pages = {355--377},
  note = {The original presentation given at the "Quantitative Finance Review"
	conference in November 2003 in London can be found at \url{www.jaeckel.org/StochasticVolatilityModels-PastPresentAndFuture.pdf}},
  crossref = {TheBestOfWilmottI},
}

@TECHREPORT{JaeckelAsianAndBasket,
  author = {P. J{\"a}ckel},
  title = {{Asian and basket options}},
  institution = {ABN AMRO},
  year = {2004},
  month = {December},
  note = {\url{file://nlas-00033.emea.abnamro-net.com/source/Product%20Development%20Group/Documentation/TeX/AsianAndBasketOptions/AsianAndBasketOptions.pdf}},
}

@TECHREPORT{JaeckelDiscontinuityAwareClosedIntervalQuadrature,
  author = {P. J{\"a}ckel},
  title = {{Discontinuity aware closed interval quadrature}},
  institution = {ABN AMRO},
  year = {2005},
  month = {April},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/$defaultview/F7393BEDE98459FBC1256FE20040D2BE/$File/DiscontinuityAwareClosedIntervalQuadrature.pdf}},
}

@INPROCEEDINGS{JaeckelHybrids2005,
  author = {P. J{\"a}ckel},
  title = {{A practical method for the valuation of a variety of hybrid products}},
  booktitle = {{ICBI Global Derivatives Conference Paris}},
  year = {2005},
}

@TECHREPORT{JaeckelInversePolynomialRootfinding,
  author = {P. J{\"a}ckel},
  title = {{Inverse polynomial root finding}},
  institution = {ABN AMRO},
  year = {2005},
  month = {April},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/$defaultview/3B0D9B112E11297CC1256FDB004AE7BA/$File/InversePolynomialRootfinding.pdf}},
}

@ARTICLE{JaeckelKawai,
  author = {P. J{\"a}ckel and A. Kawai},
  title = {{The Future is Convex}},
  journal = {Wilmott},
  year = {2005},
  pages = {2--13},
  month = {February},
  note = {\url{www.jaeckel.org/TheFutureIsConvex.pdf}},
}

@TECHREPORT{JaeckelMoreLikelyThanNot,
  author = {P. J{\"a}ckel},
  title = {{More likely than not}},
  institution = {ABN AMRO},
  year = {2004},
  month = {September},
  note = {\url{file:///nlas-00033.emea.abnamro-net.com/source/Product%20Development%20Group/Documentation/TeX/MoreLikelyThanNot/MoreLikelyThanNot.pdf}},
}

@MISC{JaeckelMultivariateGaussHermite,
  author = {P. J{\"a}ckel},
  title = {{A note on multivariate Gauss-Hermite quadrature}},
  howpublished = {\url{www.jaeckel.org/ANoteOnMultivariateGaussHermiteQuadrature.pdf}},
  month = {May},
  year = {2005},
}

@ARTICLE{JaeckelRebonato,
  author = {P. J{\"a}ckel and R. Rebonato},
  title = {{The link between caplet and swaption volatilities in a Brace-Gatarek-Musiela/Jamshidian
	framework: approximate solutions and empirical evidence}},
  journal = {Journal of Computational Finance},
  year = {2003 (submitted in 2000)},
  volume = {6},
  pages = {41--59},
  number = {4},
  note = {\url{www.jaeckel.org/LinkingCapletAndSwaptionVolatilities.pdf}},
}

@MISC{JaeckelRootsAndWeightsForRadialGaussHermiteQuadrature,
  author = {P. J{\"a}ckel},
  title = {{Roots and weights for radial Gauss-Hermite quadrature}},
  howpublished = {\url{www.jaeckel.org/RootsAndWeightsForRadialGaussHermiteQuadrature.cpp}},
  month = {May},
  year = {2005},
}

@MISC{JaeckelSplittingTheCore,
  author = {P. J{\"a}ckel},
  title = {{Splitting the core}},
  howpublished = {\url{www.jaeckel.org/SplittingTheCore.pdf}},
  year = {2004},
}

@MISC{JaeckelStabilisedMultidimensionalrootfinding,
  author = {P. J{\"a}ckel},
  title = {{Stabilised multidimensional root finding}},
  howpublished = {\url{www.jaeckel.org/StabilisedMultidimensionalRootFinding.pdf}},
  year = {2004},
}

@TECHREPORT{JaeckelTsouderosHybrid,
  author = {P. J{\"a}ckel and G. Tsouderos},
  title = {{Multivariate-multitemporal marginal density modelling of hybrid
	derivatives}},
  institution = {ABN AMRO},
  year = {2004},
  month = {November},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Index/30C3D45A255B7C55C1256F4A004B5B38/?OpenDocument\&Form=h_PageUI}},
}

@BOOK{JamesWebber,
  title = {{Interest rate modelling}},
  publisher = {John Wiley and Sons},
  year = {2000},
  author = {J. James and N. Webber},
  series = {Financial Engineering},
  month = {May},
}

@ARTICLE{Jamshidian,
  author = {F. Jamshidian},
  title = {{Libor and swap market models and measures}},
  journal = {Finance and Stochastics},
  year = {1997},
  volume = {1},
  pages = {293--330},
  number = {4},
}

@ARTICLE{JamshidianBondOptionFormula,
  author = {F. Jamshidian},
  title = {{An exact bond option pricing formula}},
  journal = {Journal of Finance},
  year = {1989},
  volume = {44},
  pages = {205--209},
  number = {9},
}

@TECHREPORT{JamshidianCreditDefaultSwapsAndSwaptions,
  author = {F. Jamshidian},
  title = {{Valuation of Credit Default Swaps and Swaptions}},
  institution = {NIB Capital Bank},
  year = {2002},
  type = {Working paper},
  month = {October},
  note = {\url{www.defaultrisk.com/pdf__files/Valuation_o_Cr_Default_Swap_n_Swptns.pdf}},
}

@INCOLLECTION{JamshidianInHullWhiteOnDerivatives,
  author = {F. Jamshidian},
  title = {{An exact bond option formula}},
  booktitle = {{Hull-White on Derivatives}},
  publisher = {Risk Publications},
  year = {1996},
  editor = {F. Jamshidian},
  crossref = {HullWhiteOnDerivatives},
}

@INCOLLECTION{JamshidianInVasicekAndBeyond,
  author = {F. Jamshidian},
  title = {{Pricing of Contingent Claims in the One-Factor Term Structure Model}},
  booktitle = {{Vasicek and beyond}},
  year = {1996},
  chapter = {7},
  pages = {111--127},
  crossref = {VasicekAndBeyond},
}

@ARTICLE{JarrowYildirim2003,
  author = {R. Jarrow and Y. Yildirim},
  title = {{Pricing Treasury Inflation Protected Securities and Related Derivatives
	using an HJM model}},
  journal = {Journal of Financial and Quantitative Analysis},
  year = {2003},
  volume = {38},
  pages = {409--430},
  number = {2},
  note = {\url{forum.johnson.cornell.edu/faculty/jarrow/papers.html}},
}

@ARTICLE{JarrowYildirimDefaultSwaps,
  author = {R. Jarrow and Y. Yildirim},
  title = {{Valuing Defualt Swaps under Market and Credit Risk Correlation.}},
  journal = {Journal of Fixed Income},
  year = {2000},
  volume = {11},
  pages = {7--19},
  number = {4},
  note = {\url{forum.johnson.cornell.edu/faculty/jarrow/papers.html}},
}

@BOOK{Joe,
  title = {{Multivariate Models and Dependence Concepts}},
  publisher = {CRC Press},
  year = {1997},
  author = {H. Joe},
  month = {May},
}

@BOOK{JohnnsonKotzBalakrishnan,
  title = {{Continuous Univariate Distributions}},
  publisher = {John Wiley and Sons},
  year = {1994},
  author = {N. L. Johnson and S. Kotz and N. Balakrishnan},
  volume = {I and II},
}

@ARTICLE{Johnson,
  author = {N. L. Johnson},
  title = {{Systems of frequency curves generated by methods of translation}},
  journal = {Biometrika},
  year = {1949},
  volume = {36},
  pages = {14--76},
  note = {A fitting algorithm for Johnson distributions can be found in: {ALGORITHM
	AS 99 APPL. STATIST. (1976) VOL.25, P.180}, \url{lib.stat.cmu.edu/apstat/99}},
}

@ARTICLE{JohnsonLee,
  author = {S. Johnson and H. Lee},
  title = {{Capturing the Smile}},
  journal = {Risk},
  year = {2003},
  volume = {16},
  number = {3},
  month = {March},
  note = {\url{www.numerix.com/news/announcements/0303_smile.pdf}},
}

@ARTICLE{JohnsonLee2003,
  author = {S.R. Johnson and H.H. Lee},
  title = {{Capturing the Smile}},
  journal = {Risk},
  year = {2003},
  pages = {89-93},
  month = {March},
}

@BOOK{JorionBook,
  title = {{Financial Risk Manager Handbook 2001--2001}},
  publisher = {John Wiley and Sons},
  year = {2001},
  author = {P. Jorion},
}

@BOOK{JoshiConcepts,
  title = {{The Concepts and Practice of Mathematical Finance}},
  publisher = {Cambridge University Press},
  year = {2003},
  author = {M. Joshi},
}

@ARTICLE{JoshiRebonato2003,
  author = {M. Joshi and R. Rebonato},
  title = {{A stochastic-volatility, displaced-diffusion extension of the LIBOR
	Market Model}},
  journal = {Quantitative Finance},
  year = {2003},
  volume = {3},
  pages = {458-469},
  number = {6},
  month = {December},
  note = {\url{www.quarchome.org/StochasticVolatilityBGMFin.pdf}},
}

@ARTICLE{JoshiTheis,
  author = {M. Joshi and J. Theis},
  title = {{Bounding Bermudan swaptions in a swap-rate market model}},
  journal = {Quantitative Finance},
  year = {2002},
  volume = {2},
  pages = {370--377},
  number = {5},
  month = {October},
  note = {\url{www.quarchome.org/BermBounds.pdf}},
}

@TECHREPORT{JouaninRapuchRibouletRoncalli,
  author = {J. Jouanin and G. Rapuch and G. Riboulet and T. Roncalli},
  title = {{Modelling dependence for credit derivatives with copulas}},
  institution = {Groupe de Recherche Op{\'e}rationnelle, Cr{\'e}dit Lyonnais, France},
  year = {2001},
  type = {Working paper},
  note = {\url{gro.creditlyonnais.fr/content/wp/copula-intensity.pdf}},
}

@ARTICLE{JuPearson99,
  author = {J. Xiongwei and N. Pearson},
  title = {{Using Value-at-Risk to Control Risk Taking: How wrong can you be?}},
  journal = {Journal of Risk},
  year = {1999},
  volume = {1},
  pages = {5--36},
  number = {2},
  month = {Winter},
}

@TECHREPORT{KSS,
  author = {O. Kurbanmuradov and K. Sabelfeld and J. Schoenmakers},
  title = {{Lognormal random field approximations to LIBOR market models}},
  institution = {Weierstrass Institute, Berlin},
  year = {1999},
  type = {Working paper},
  note = {\url{www.wias-berlin.de/publications/preprints/481/document.pdf}},
}

@INPROCEEDINGS{Kac,
  author = {M. Kac},
  title = {{On some connections between probability theory and differential
	and integral equations}},
  booktitle = {{Proc.\ 2nd Berkeley Symposium on Math. Stat. \& Probability}},
  year = {1951},
  pages = {189--215},
}

@MASTERSTHESIS{Kahl2004,
  author = {C. Kahl},
  title = {{Positive numerical integration of stochastic differential equations}},
  school = {Bergische Universit{\"a}t Wuppertal},
  year = {2004},
  note = {\url{www.math.uni-wuppertal.de/~kahl/publications/DT.pdf}},
}

@TECHREPORT{KahlGuentherRossberg,
  author = {C. Kahl and M. G{\"u}nther and T. Ro{\ss}berg},
  title = {{Structure preserving stochastic integration schemes in interest
	rate derivative modelling}},
  institution = {Bergische Universit{\"a}t Wuppertal},
  year = {2004},
  type = {Working paper},
  month = {September},
  note = {\url{www.math.uni-wuppertal.de/org/Num/Files/amna_04_10.pdf}},
}

@ARTICLE{KahlJaeckel1,
  author = {C. Kahl and P. J{\"a}ckel},
  title = {{Not-so-complex logarithms in the Heston model}},
  journal = {Wilmott},
  year = {2005},
  volume = {September},
  month = {September},
}

@ARTICLE{KahlJaeckel2,
  author = {C. Kahl and P. J{\"a}ckel},
  title = {{Fast strong approximations Monte Carlo schemes for stochastic volatility
	models}},
  journal = {In preparation},
  year = {2005},
}

@TECHREPORT{KahlSchurz2005,
  author = {C. Kahl and H. Schurz},
  title = {{Balanced Milstein Methods for Ordinary SDEs}},
  institution = {Department of Mathematics, Southern Illinois University},
  year = {2005},
  owner = {gbjaep},
}

@TECHREPORT{KakodkarGalinni,
  author = {A. Kakodkar and S. Galinni},
  title = {{Constant maturity CDS: bullish on credit, bearish on spreads}},
  institution = {Merrill Lynch},
  year = {2004},
  month = {April},
}

@TECHREPORT{Kamthan,
  author = {Pankaj Kamthan},
  title = {{XML Entities and their Applications}},
  institution = {Internet-Related Technologies},
  year = {2000},
  month = {May},
  note = {\url{www.tech.irt.org/articles/js212/index.htm}},
}

@TECHREPORT{Karasinski,
  author = {P. Karasinski},
  title = {{Do we need a new market volatility standard? Exploring rate-level
	dependence of volatility}},
  institution = {Fixed Income Research Citigroup Schroder Salomon Smith Barney},
  year = {2002},
  type = {presented at the Quantitative Finance London 2002 conference},
  month = {November 25},
}

@BOOK{KaratzasShreve,
  title = {{Brownian motion and Stochastic Calculus}},
  publisher = {Springer},
  year = {1991},
  author = {I. Karatzas and S. E. Shreve},
}

@BOOK{KaratzasShreve2,
  title = {{Methods of Mathematical Finance}},
  publisher = {Springer},
  year = {1998},
  author = {I. Karatzas and S. E. Shreve},
}

@BOOK{KarlinTaylorSecond,
  title = {{A Second Course in Stochastic Processes}},
  publisher = {Academic Press},
  year = {1981},
  author = {S. Karlin and M. Taylor},
}

@TECHREPORT{Kaufmann,
  author = {R. Kaufmann},
  title = {{Copulas as an Integrated Risk Management Tool}},
  institution = {RiskLab, Departement Mathematik, ETH Z{\"u}rich, Switzerland},
  year = {2001},
  type = {Risk 2001 Europe Conference, April 10-11, Paris},
  note = {\url{www.math.ethz.ch/~kaufmann/Copulas/Paris2001.pdf}},
}

@ARTICLE{Kawai02,
  author = {A. Kawai},
  title = {{Analytical and Monte Carlo swaption pricing under the forward swap
	measure}},
  journal = {Journal of Computational Finance},
  year = {2002},
  volume = {6},
  pages = {101--111},
  number = {1},
  note = {\url{www.maths.unsw.edu.au/statistics/preprints/2002/s02-12.pdf}},
}

@ARTICLE{Kawai03,
  author = {A. Kawai},
  title = {{A new approximate swaption formula in the LIBOR market model: an
	asymptotic expansion approach}},
  journal = {Applied Mathematical Finance},
  year = {2003},
  volume = {10},
  pages = {49--74},
  number = {1},
  month = {March},
  note = {\url{www.maths.unsw.edu.au/statistics/preprints/2002/s02-13.pdf}},
}

@ARTICLE{Kawai05,
  author = {A. Kawai},
  title = {{An asymptotic FX option formula in the Libor market model}},
  journal = {In Preparation},
  year = {2005},
}

@TECHREPORT{KieselPerraudinTaylor,
  author = {R. Kiesel and W. Perraudin and A. Taylor},
  title = {{The structure of credit risk}},
  institution = {Birkbeck College},
  year = {1999},
  note = {\url{wp.econ.bbk.ac.uk/respap/respap_frames.html}},
}

@ARTICLE{KirikosNovak,
  author = {G. Kirikos and D. Novak},
  title = {{Convexity Conundrums}},
  journal = {Risk},
  year = {1997},
  pages = {60--61},
  month = {March},
  note = {\url{www.powerfinance.com/convexity}},
}

@BOOK{KloedenPlaten,
  title = {{Numerical Solution of Stochastic Differential Equations}},
  publisher = {Springer},
  year = {1992, 1995, 1999},
  author = {P. E. Kloeden and E. Platen},
}

@OTHER{Kluge,
  author = {T. Kluge},
  month = {September},
  note = {\url{kluge.in-chemnitz.de/documents/diploma/diploma.pdf}},
  school = {Technische Universit{\"a}t Chemnitz},
  title = {{Pricing derivatives in stochastic volatility models using the finite
	difference method}},
  year = {2002},
}

@BOOK{Knopp,
  title = {{Theory and application of infinite series}},
  publisher = {General Publishing Company, Canada; Dover},
  year = {1921,1928,1947,1951,1990},
  author = {Konrad Knopp},
}

@TECHREPORT{Knudsen,
  author = {T. Knudsen},
  title = {{Calibration and Vega of Exotic Models}},
  institution = {Abbey National Financial Products},
  year = {2002},
  type = {Working paper, presented at King's College London},
  month = {March},
}

@BOOK{Knuth,
  title = {{The Art of Computer Programming: Seminumerical Algorithms}},
  publisher = {Addison-Wesley},
  year = {1969,1981},
  author = {D. Knuth},
  volume = {2},
}

@ARTICLE{KouWang,
  author = {S. G. Kou and H. Wang},
  title = {{First passage times of a jump diffusion process}},
  journal = {Advances in Applied Probability},
  year = {2003},
  volume = {35},
  pages = {504--531},
  number = {2},
  note = {\url{www.columbia.edu/\~sk75/KouWangAAP.pdf}},
}

@MISC{KouWang2,
  author = {S. G. Kou and H. Wang},
  title = {{Option pricing under a double exponential jump diffusion model}},
  howpublished = {\url{www.columbia.edu/\~sk75/option.pdf}},
  month = {September},
  year = {2001},
}

@MISC{KouWangWorkingPaper,
  author = {S. G. Kou and H. Wang},
  title = {{First passage times of a jump diffusion process}},
  howpublished = {\url{www.columbia.edu/\~sk75/KouWangAAP.pdf}},
  year = {2000},
}

@ARTICLE{KrekelKockKornMan,
  author = {M. Krekel and J. de Kock and R. Korn and T.-K. Man},
  title = {{An Analysis of Pricing Methods for Basket Option}},
  journal = {Wilmott},
  year = {2004},
  pages = {82--89},
}

@ARTICLE{KullbackLeibler,
  author = {S. Kullback and R. A. Leibler},
  title = {{On information and sufficiency}},
  journal = {Ann. Math. Stat.},
  year = {1951},
  volume = {22},
  pages = {79--86},
}

@ARTICLE{KunitomoIkeda,
  author = {N. Kunitomo and M. Ikeda},
  title = {{Pricing Options with Curved Boundaries}},
  journal = {Mathematical Finance},
  year = {1992},
  volume = {2},
  pages = {275--298},
  number = {4},
  month = {October},
}

@ARTICLE{Kupiec,
  author = {P. H. Kupiec},
  title = {{Stress Testing in a Value at Risk Framework}},
  journal = {Journal of Derivatives},
  year = {1998},
  pages = {7--24},
  month = {Fall},
}

@TECHREPORT{KurpielRoncalli,
  author = {A. Kurpiel and T. Roncalli},
  title = {{Option hedging with stochastic volatility}},
  institution = {Universit{\'e} Montesquieu-Bordeaux IV / City University Business
	School London},
  year = {1998},
  type = {Working paper},
  month = {December},
  note = {\url{users.wbs.ac.uk/cms_attachment_handler.cfm?f=3.pdf\&t=3.pdf}},
}

@BOOK{Kvasov,
  title = {{Methods of Shape-Preserving Spline Approximation}},
  publisher = {World Scientific Publishing},
  year = {2000},
  author = {B. Kvasov},
  note = {ISBN 9810240104},
}

@TechReport{LPRJ,
  author = 	 {Y. Liu and S. Phillips and E. Rogge and P. J{\"a}ckel},
  title = 	 {A Linear Swap Rate Model With A Risky Component},
  institution =  {ABN AMRO},
  year = 	 {2005},
  month = {May},
}

@BOOK{Lando,
  title = {{Credit Risk Modeling: Theory and Applications}},
  publisher = {Princeton University Press},
  year = {2004},
  author = {D. Lando},
  note = {ISBN 0691089299},
}

@article{Langevin1908,
		 author={Langevin, P.},
		 title={Sur la th{\'e}orie du mouvement brownien},
		 journal={{C. R. Acad. Sci. (Paris)}},
		 volume={146},
		 year={1908},
		 pages={530--533}
}

@ARTICLE{LaplaceTransformationOptionValuation,
  author = {M. C. Fu and D. B. Madan and T. Wang},
  title = {{Pricing continuous {{Asian}} options: a comparison of {{Monte Carlo}}
	and {{Laplace}} transform inversion methods}},
  journal = {Journal of Computational Finance},
  year = {1998},
  volume = {2},
  pages = {49--74},
  number = {2},
}

@BOOK{LargeScaleCpp,
  title = {{Large-Scale C++ Software Design}},
  publisher = {Addison Wesley},
  year = {1996},
  author = {John S. Lakos},
  note = {ISBN 0201633620},
}

@TECHREPORT{LaurentGregory,
  author = {J.P. Laurent and J. Gregory},
  title = {{Basket default swaps, CDO's and Factor Copulas}},
  institution = {BNP Paribas},
  year = {2002},
  type = {Working paper},
  note = {\url{www.maths.univ-evry.fr/mathfi/JPLaurent.pdf}},
}

@ARTICLE{Lecuyer,
  author = {P. L'Ecuyer},
  title = {{Efficient and Portable Combined Random Number Generators}},
  journal = {Communications of the ACM},
  year = {1988},
  volume = {31},
  pages = {742--749,774},
}

@INPROCEEDINGS{LecuyerGoodAndBad,
  author = {P. L'Ecuyer},
  title = {{Software for Uniform Random Number Generation: Distinguishing the
	Good and the Bad}},
  booktitle = {{Proceedings of the 2001 Winter Simulation Conference}},
  year = {2001},
  note = {\url{www.iro.umontreal.ca/~lecuyer/myftp/papers/wsc01rng.pdf}},
  crossref = {2001WinterSimulationConference},
}

@INBOOK{LecuyerRandomNumbers,
  chapter = {Random Numbers (P. L'Ecuyer)},
  pages = {12735--12738},
  title = {{International Encyclopedia of the Social and Behavioral Sciences}},
  publisher = {Pergamon},
  year = {2002},
  editor = {N. J. Smelser and P. B. Baltes},
  note = {\url{www.iro.umontreal.ca/~lecuyer/myftp/papers/ensbs.pdf}},
}

@ARTICLE{Lee2005,
  author = {R. Lee},
  title = {{Option Pricing by Transform Methods: Extensions, Unification, and
	Error Control}},
  journal = {Journal of Computational Finance},
  year = {2005},
  volume = {7},
  pages = {51--86},
  number = {3},
  owner = {gbjaep},
}

@ARTICLE{Leland,
  author = {H. E. Leland},
  title = {{Option Pricing and Replication with Transaction Costs}},
  journal = {Journal of Finance},
  year = {1985},
  volume = {40},
  pages = {1283--1301},
}

@TECHREPORT{LevinSingh,
  author = {R. Levin and K. Singh},
  title = {{What hides behind the smile?}},
  institution = {Derivatives Research, J. P. Morgan Securities Inc., New York},
  year = {1995},
  type = {Published Report},
  address = {Ron Levin: (97-2) 253-6017, Kuljot Singh: (1-212) 648-3104},
  month = {March},
}

@INPROCEEDINGS{Levy1951,
  author = {P. L{\'e}vy},
  title = {{Wiener's random function, and other Laplacian random functions}},
  booktitle = {{Proceedings of the Second Berkeley Symposium on Mathematical Statistics
	and Probability, 1950}},
  year = {1951},
  pages = {171--187},
  address = {Berkeley and Los Angeles},
  publisher = {University of California Press},
  mrclass = {60.0X},
  mrnumber = {13,476b},
  owner = {gbjaep},
}

@ARTICLE{LevyLognormalBaskets,
  author = {E. Levy},
  title = {{Pricing {{European}} average rate currency options}},
  journal = {Journal of International Money and Finance},
  year = {1992},
  volume = {11},
  pages = {474--491},
}

@MISC{LevyMantion,
  author = {E. Levy and F. Mantion},
  title = {{Approximate Valuation of Discrete Lookback and Barrier options}},
  year = {1998},
  note = {\url{sina.sharif.edu/~khoshnevisan/LEVY.PDF}},
  type = {Working paper},
}

@ARTICLE{LevyMantionRisk,
  author = {E. Levy and F. Mantion},
  title = {{Discrete by Nature}},
  journal = {Risk},
  year = {1997},
  volume = {10},
  pages = {74--75},
  month = {January},
}

@TECHREPORT{Lewis2001,
  author = {A. Lewis},
  title = {{A Simple Option Formula for General Jump-Diffusion and other Exponential Levy Processes}},
  institution = {Envision Financial Systems and OptionCity.net},
  year = {2001},
  note = {\url{optioncity.net/pubs/ExpLevy.pdf}},
  type = {Working paper},
  address = {983 Bayside Cove West, Newport Beach, Ca 92660 USA},
  month = {August},
}

@ARTICLE{LewisGoodmanMiller,
  author = {P. A. W. Lewis and A. S. Goodman and J. M. Miller},
  title = {{A pseudorandom number generator for the System/360}},
  journal = {IBM System Journal},
  year = {1969},
  volume = {8},
  pages = {136--146},
}

@ARTICLE{Li,
  author = {D. X. Li},
  title = {{On Default Correlation: A Copula Approach}},
  journal = {Journal of Fixed Income},
  year = {2000},
  volume = {9},
  pages = {43--54},
  month = {March},
}

@PHDTHESIS{Lindskog,
  author = {F. Lindskog},
  title = {{Modelling Dependence with Copulas and Applications to Risk Management}},
  school = {ETH},
  year = {2000},
  type = {Masters Thesis},
  address = {Z{\"u}rich},
  month = {Version 02-July},
}

@TECHREPORT{LindskogMcNeil,
  author = {F. Lindskog and A. McNeil},
  title = {{Common Poisson Shock Models: Application to Insurance and Credit
	Risk Modelling}},
  institution = {RiskLab, Departement Mathematik, ETH Z{\"u}rich, Switzerland},
  year = {2001},
  type = {Working paper},
  note = {\url{www.risklab.ch/ftp/papers/CommonPoissonShockModels.pdf}},
}

@TECHREPORT{LindskogMcNeilSchmock,
  author = {F. Lindskog and A. McNeil and U. Schmock},
  title = {{Kendall's Tau for Elliptical Distributions}},
  institution = {RiskLab, Departement Mathematik, ETH Z{\"u}rich, Switzerland},
  year = {2001},
  type = {Working paper},
  note = {\url{www.risklab.ch/ftp/papers/KendallsTau.pdf}},
}

@BOOK{LionsCiarlet,
  title = {{Handbook of Numerical Analysis, Volume I}},
  publisher = {Elsevier Science Publishers},
  year = {1989},
  editor = {J. Lions and P. Ciarlet},
}

@ARTICLE{LiuJaeckel,
  author = {Y. Liu and P. J{\"a}ckel},
  title = {{Options on Credit Default Index Swaps}},
  journal = {Wilmott},
  year = {2005},
  pages = {92--97},
  month = {July},
}


@TECHREPORT{LiuYCDSwaption,
  author = {Y. Liu},
  title = {{Credit Default Swaptions On Indices}},
  institution = {ABN AMRO},
  year = {2005},
  month = {January},
}

@ARTICLE{LoHuen1,
  author = {C. F. Lo and P. H. Yuen},
  title = {{Option Risk Measurement with Time-Dependent Parameters}},
  journal = {International Journal of Theoretical and Applied Finance},
  year = {2000},
  volume = {3},
  pages = {581--589},
  number = {3},
  note = {\url{www.phy.cuhk.edu.hk/people/teach/cflo/Finance/papers/optionrisk_IJTAF.pdf}},
}

@ARTICLE{LoHuen2,
  author = {C. F. Lo and P. H. Yuen},
  title = {{Constant Elasticity Of Variance Option Pricing Model with Time-Dependent
	Parameters}},
  journal = {International Journal of Theoretical and Applied Finance},
  year = {2000},
  volume = {3},
  pages = {661--674},
  number = {4},
  note = {\url{www.phy.cuhk.edu.hk/people/teach/cflo/Finance/papers/publications/CEV_IJTAF.pdf}},
}

@TECHREPORT{LongstaffSantaClaraSchwartz00,
  author = {F. A. Longstaff and P. Santa-Clara and E. S. Schwartz},
  title = {{The Relative Valuation of Caps and Swaptions: Theory and Empirical
	Evidence}},
  institution = {The Anderson school, UCLA},
  year = {2000},
  type = {Working paper},
}

@TECHREPORT{LongstaffSantaClaraSchwartz99,
  author = {F. A. Longstaff and P. Santa-Clara and E. S. Schwartz},
  title = {{Throwing away a billion dollars: the cost of sub-optimal exercise
	strategies in the swaptions market}},
  institution = {The Anderson school, UCLA},
  year = {1999},
  type = {Working paper},
}

@TECHREPORT{LongstaffSchwarz,
  author = {F. A. Longstaff and E. S. Schwartz},
  title = {{Valuing American options by simulation: A simple least squares approach}},
  institution = {The Anderson school, UCLA},
  year = {1998},
  type = {Working paper},
}

@ARTICLE{MAP1976,
  author = {G. Marsaglia and K. Anantharayanan and N.J. Paul},
  title = {{Improvements on fast methods for generating normal random variables}},
  journal = {Information Processing Letters},
  year = {1976},
  volume = {5},
  pages = {27--30},
  owner = {gbjaep},
}

@ARTICLE{MMB1964,
  author = {G. Marsaglia and M.D. MacLaren and T.A. Bray},
  title = {{A fast procedure for generating normal random variables}},
  journal = {Communications of the ACM},
  year = {1964},
  volume = {5},
  pages = {27--30},
  owner = {gbjaep},
}

@article{MPS:98,
   author={G. N. Milshtein and E. Platen and H. Schurz},
   title={Balanced implicit methods for stiff stochastic systems},
   journal={SIAM},
   volume= 38,
   year= 1998,
   pages={1010--1019},
   number= 3
}

@TECHREPORT{MacKay,
  author = {D. J. C. MacKay},
  title = {{Introduction to Monte Carlo Methods}},
  institution = {Department of Physics, Cambridge University},
  year = {1997},
  address = {CB3 0HE, England},
  note = {\url{ftp://wol.ra.phy.cam.ac.uk/pub/mackay/erice.ps.gz} or \url{l3www.cern.ch/homepages/susinnog/finance/Articles4/erice.ps.gz}},
}

@TECHREPORT{MadanCarrChang,
  author = {D. B. Madan and P. Carr and E. C. Chang},
  title = {{The {{Variance Gamma}} process and option pricing}},
  institution = {University of Maryland},
  year = {1998},
  type = {Working paper},
  address = {College park, MD 20742},
  month = {June},
}

@ARTICLE{MadanMilne,
  author = {D. B. Madan and F. Milne},
  title = {{Option pricing with {{Variance Gamma}} Martingale Components}},
  journal = {Mathematical Finance},
  year = {1991},
  volume = {1},
  pages = {39--55},
  number = {4},
}

@ARTICLE{MadanSeneta,
  author = {D. B. Madan and E. Seneta},
  title = {{The {{Variance Gamma}} Model for share market returns}},
  journal = {Journal of Business},
  year = {1990},
  volume = {63},
  pages = {511--524},
  number = {4},
}

@BOOK{Malliavin1978,
  title = {{Geometrie differentielle stochastique}},
  publisher = {Montreal: Presses de l' Universite de Montreal},
  year = {1978},
  author = {P. Malliavin},
  journal = {Montreal: Presses de l' Universite de Montreal},
  owner = {gbjaep},
}

@INPROCEEDINGS{Malliavin1978a,
  author = {P. Malliavin},
  title = {{Stochastic calculus of variation and hypoelliptic operators}},
  booktitle = {Proc. Int. Symp. S.D.E. Kyoto (1976)},
  year = {1978},
  pages = {195--263},
  publisher = {John Wiley and Sons},
  journal = {Proc. Int. Symp. S.D.E. Kyoto, (1976) 195 - 263, Wiley and Sons,
	New York 1978. MR 81f:600},
  owner = {gbjaep},
}

@BOOK{Malliavin2002,
  title = {{Stochastic Analysis}},
  publisher = {Springer},
  year = {2002},
  author = {P. Malliavin},
  owner = {gbjaep},
}

@BOOK{Marchuk,
  title = {{Numerical Methods and Applications}},
  publisher = {CRC Press},
  year = {1994},
  editor = {G. I. Marchuk},
  month = {March},
  note = {ISBN 084938947X},
}

@INCOLLECTION{MarchukSplitting,
  author = {G. I. Marchuk},
  title = {{Splitting and Alternating Direction Methods}},
  booktitle = {{Handbook of Numerical Analysis, Volume I}},
  publisher = {Elsevier Science Publishers},
  year = {1989},
  editor = {J. Lions and P. Ciarlet},
  volume = {I},
  pages = {197--462},
  optcrossref = {LionsCiarlet},
}

@ARTICLE{Margrabe,
  author = {W. Margrabe},
  title = {{The value of an option to exchange one asset for another}},
  journal = {Journal of Finance},
  year = {1978},
  volume = {33},
  pages = {177--186},
}

@ARTICLE{MarkovFunctionalModels,
  author = {J. Kennedy and P. Hunt and A. Pelsser},
  title = {{Markov-functional interest rate models}},
  journal = {Finance and Stochastics},
  year = {2000},
  volume = {4},
  pages = {391--408},
  number = {4},
}

@ARTICLE{MarsagliaZamanMarsaglia,
  author = {G. Marsaglia and A. Zaman and J. Marsaglia},
  title = {{Rapid Evaluation of the Inverse of the Normal Distribution Function}},
  journal = {Statistics and Probability Letters},
  year = {1994},
  pages = {259--266},
  number = {19},
}

@ARTICLE{Maruyama1955,
  author = {G. Maruyama},
  title = {{Continuous Markov processes and stochastic equations}},
  journal = {Rendiconti del Circolo Matematico di Palermo},
  year = {1955},
  volume = {4},
  pages = {48--90},
  owner = {gbjaep},
}

@ARTICLE{Matsumoto,
  author = {K. Matsumoto},
  title = {{Lognormal swap approximation in the Libor marekt model and its application}},
  journal = {Journal of Computational Finance},
  year = {2001},
  volume = {5},
  pages = {107--131},
  number = {1},
}

@ARTICLE{May,
  author = {R. M. May},
  title = {{Simple mathematical models with very complicated dynamics}},
  journal = {Nature},
  year = {1976},
  volume = {26},
  pages = {459--467},
}

@TECHREPORT{McCarthyWebber,
  author = {L. A. McCarthy and N. J. Webber},
  title = {{An Icosahedral Lattice Method for Three-Factor Models}},
  institution = {University of Warwick},
  year = {1999},
  type = {Working paper},
  note = {\url{www.warwick.ac.uk}},
  pages = {1--45},
}

@TECHREPORT{McGinty,
  author = {L. McGinty},
  title = {{Introducing Base Correlation}},
  institution = {JP Morgan},
  year = {2004},
  type = {Working paper},
  month = {March},
  note = {\url{www.wilmott.com/attachments/IntroducingBaseCorrelations.zip}},
}

@TECHREPORT{McGintyBeinsteinAhluwaliaWatts,
  author = {L. McGinty and E. Beinstein and R. Ahluwalia and M. Watts},
  title = {{Credit Correlation: A Guide}},
  institution = {JP Morgan},
  year = {2004},
  type = {Working paper},
  month = {March},
  note = {\url{www.wilmott.com/attachments/Base correlationJPM.zip}},
}

@TECHREPORT{McGintyWatts,
  author = {L. McGinty and M. Watts},
  title = {{Credit Volatility -- A Primer}},
  institution = {JPMorgan},
  year = {2003},
  month = {July},
}

@BOOK{McKean,
  title = {{Stochastic Integrals}},
  publisher = {New York Academic Press},
  year = {1969},
  author = {H. P. McKean},
}

@TECHREPORT{Mercurio2002,
  author = {F. Mercurio},
  title = {{Pricing the smile in a forward LIBOR market model}},
  institution = {Banca IMI},
  year = {2002},
  note = {\url{www.fabiomercurio.com/BGMsmile.pdf}},
}

@TECHREPORT{MercurioInflationTalk,
  author = {F. Mercurio},
  title = {{Pricing of Inflation-Indexed Derivatives}},
  institution = {Banca IMI},
  year = {2004},
  note = {\url{www.fabiomercurio.it/wbs2004.pdf}},
}

@ARTICLE{MersenneTwister,
  author = {M. Matsumoto and T. Nishimura},
  title = {{Mersenne Twister: A 623-dimensionally equidistributed uniform pseudorandom
	number generator}},
  journal = {ACM Trans. on Modeling and Computer Simulation},
  year = {1998},
  volume = {8},
  pages = {3--30},
  number = {1},
  month = {January},
}

@MISC{MersenneTwisterURL,
  author = {M. Matsumoto and T. Nishimura},
  title = {{Mersenne Twister: A 623-dimensionally equidistributed uniform pseudorandom
	number generator}},
  howpublished = {\url{www.math.keio.ac.jp/~matumoto/emt.html}},
  year = {1997},
}

@BOOK{Merton,
  title = {{Continuous-Time Finance}},
  publisher = {Blackwell Publishers Ltd.},
  year = {1990},
  author = {R. C. Merton},
}

@ARTICLE{Merton74,
  author = {R. Merton},
  title = {{On the Pricing of Corporate Debt: The Risk Structure of Interest
	Rates}},
  journal = {Journal of Finance},
  year = {1974},
  volume = {29},
  pages = {449--470},
}

@ARTICLE{MertonDiscontinuous,
  author = {R. C. Merton},
  title = {{Option Pricing When Underlying Stock Returns are Discontinuous}},
  journal = {Journal of Financial Economics},
  year = {1976},
  volume = {3},
  pages = {125--144},
}

@ARTICLE{MertonTheoryOfRationalOptionPricing,
  author = {R. C. Merton},
  title = {{Theory of Rational Option Pricing}},
  journal = {Bell Journal of Economics and Management Science},
  year = {1973},
  volume = {4},
  pages = {141--183},
  month = {Spring},
}

@ARTICLE{MetropolisUlam,
  author = {N. Metropolis and S. Ulam},
  title = {{The Monte Carlo method}},
  journal = {Journal of the American Statistical Association},
  year = {1949},
  volume = {44},
  pages = {335--341},
  number = {247},
  month = {September},
}

@BOOK{Meyer,
  title = {{Monte Carlo simulation with Java and C++}},
  publisher = {\url{download.berlios.de/martingale/MCBook-1.2.pdf.gz}},
  year = {2003},
  author = {M. Meyer},
  note = {\url{download.berlios.de/martingale/MCBook-1.2.pdf.gz}},
}

@MISC{MeyerBermudan,
  author = {M. Meyer},
  title = {{Monte Carlo Pricing of Bermudan Options}},
  howpublished = {\url{martingale.berlios.de/topics/Bermudan/Index.html}},
  year = {2003},
}

@ARTICLE{MikeCurranGeometricConditioning,
  author = {Mike Curran},
  title = {{Valuing Asian and portfolio options by conditioning on the geometric
	mean price}},
  journal = {Management science},
  year = {1994},
  volume = {40},
  pages = {1705--1711},
}

@INCOLLECTION{MikeCurranGreeksMC,
  author = {M. Curran},
  title = {{Greeks in Monte Carlo}},
  booktitle = {{Monte Carlo: Methodologies and Applications for Pricing and Risk
	Management}},
  publisher = {Risk Publications},
  year = {1998},
  crossref = {DupireMC},
}

@ARTICLE{MikeCurranStratification,
  author = {M. Curran},
  title = {{Strata Gems}},
  journal = {Risk},
  year = {1994},
  month = {March},
}

@ARTICLE{MikhailovNoegel2003,
  author = {S. Mikhailov and U. N{\"o}gel},
  title = {{Heston's Stochastic Volatilty Model: Implementation, Calibration,
	and some Extensions}},
  journal = {Wilmott},
  year = {2003},
  volume = {July},
  pages = {74--79},
  owner = {gbjaep},
}

@TECHREPORT{Mikkelsen,
  author = {P. Mikkelsen },
  title = {{Cross-Currency LIBOR Market Models}},
  institution = {Aarhus School of Business},
  year = {1999--2002},
  note = {\url{www.hha.dk/fin/finance/Research/D01_6.PDF}},
}

@ARTICLE{MilevskyPosnerAsian,
  author = {M. A. Milevsky and S. E. Posner},
  title = {{Asian Options, the sum of Lognormals and the Reciprocal Gamma Distribution}},
  journal = {Journal of Financial and Quantitative Analysis},
  year = {1998},
  volume = {33},
  number = {3},
  month = {September},
}

@ARTICLE{MilevskyPosnerBasket,
  author = {M. A. Milevsky and S. E. Posner},
  title = {{A Closed-Form Approximation for Valuing Basket Options}},
  journal = {Journal of Derivatives},
  year = {1998},
  volume = {5},
  pages = {54--62},
  number = {4},
}

@ARTICLE{MilevskyPosnerBasketErratum,
  author = {M. A. Milevsky and S. E. Posner},
  title = {{Erratum. A Closed-Form Approximation for Valuing Basket Options}},
  journal = {Journal of Derivatives},
  year = {1998},
  volume = {5},
  pages = {83},
}

@TECHREPORT{MilevskyPosnerReciprocalGamma,
  author = {M. A. Milevsky and S. E. Posner},
  title = {{Closed-Form Analytic Pricing and Hedging of Arithmetic Asian Options
	using a Reciprocal Gamma Distribution}},
  institution = {York University, Ontario, Canada},
  year = {1997},
  note = {\url{papers.ssrn.com/sol3/Delivery.cfm/9705303.pdf}},
}

@ARTICLE{Milshtein,
  author = {G. N. Milshtein},
  title = {{Approximate integration of stochastic differential equations}},
  journal = {Theory of Probability and Applications},
  year = {1974},
  volume = {19},
  pages = {557--562},
}

@ARTICLE{MiltersenSandmannSondermann,
  author = {K. R. Miltersen and K. Sandmann and D. Sondermann},
  title = {{Closed-form solutions for term structure derivatives with lognormal
	interest rates}},
  journal = {Journal of Finance},
  year = {1997},
  volume = {52},
  pages = {409--430},
  number = {1},
}

@TECHREPORT{MitchellTaylorWest,
  author = {K. Mitchell and D. R. Taylor and G. West},
  title = {{Discrete solutions for barrier options}},
  institution = {School of Computational and Applied Mathematics, University of the
	Witwatersrand, Johannesburg, South Africa},
  year = {2003},
  type = {Working paper},
  month = {December},
  note = {\url{www.cam.wits.ac.za/mfinance/graeme/barrier.pdf}},
}

@ARTICLE{Moro,
  author = {B. Moro},
  title = {{The Full Monte}},
  journal = {Risk},
  year = {1995},
  volume = {8},
  pages = {57--58},
  number = {2},
  month = {February},
}

@BOOK{MortonMayers,
  title = {{Numerical Solution of Partial Differential Equations}},
  publisher = {Cambridge University Press},
  year = {1994},
  author = {K. W. Morton and D. F. Mayers},
  note = {ISBN 0521429226},
}

@ARTICLE{MusielaRutkowski,
  author = {M. Musiela and M. Rutkowski},
  title = {{Continuous-time term structure models: Forward measure approach}},
  journal = {Finance and Stochastics},
  year = {1997},
  volume = {1},
  pages = {261--292},
  number = {4},
}

@BOOKLET{NBSMonteCarloMethod,
  title = {{Monte Carlo Method}},
  address = {U.S. Department of Commerce, National Bureau of Standards, Applied
	Mathematics Series 12},
  month = {June},
  year = {1951},
  note = {A 42-page booklet on number generation methods and applications of
	the Monte Carlo method},
  key = {Monte Carlo Method},
}

@ARTICLE{NL2SOL,
  author = {J. E. Dennis and D. M. Gay and R. E. Welsch},
  title = {{NL2SOL -- an adaptive nonlinear least-squares algorithm}},
  journal = {ACM Transactions on Mathematical Software},
  year = {1981},
  volume = {7},
  pages = {348--368},
  note = {\url{www.netlib.org/toms/573}},
}

@ARTICLE{NX1,
  author = {H. Niederretier and C. P. Xing},
  title = {{Low-discrepancy sequences obtained from algebraic function fields
	over finite fields}},
  journal = {Acta Arithmetica},
  year = {1995},
  volume = {72},
  pages = {281--298},
}

@ARTICLE{NX2,
  author = {H. Niederretier and C. P. Xing},
  title = {{Low-discrepancy sequences and global function fields with many rational
	places}},
  journal = {Finite Fields and Their Applications},
  year = {1996},
  volume = {2},
  pages = {241--273},
  note = {\url{www.dismat.oeaw.ac.at/pirs/niedxing.html}},
}

@BOOK{Natenberg,
  title = {{Option Volatility \& Pricing: Advanced Trading Strategies and Techniques}},
  publisher = {Probus Publishing Co.},
  year = {1994},
  author = {S. Natenberg},
  month = {July},
  note = {ISBN 155738486X},
}

@BOOK{Nayfeh,
  title = {{Introduction to Perturbation Techniques}},
  publisher = {John Wiley and Sons},
  year = {1981--1993},
  author = {A. H. Nayfeh},
}

@ARTICLE{Neave,
  author = {H. R. Neave},
  title = {{On using the Box-Muller transformation with multiplicative congruential
	pseudo-random number generators}},
  journal = {Applied Statistics},
  year = {1973},
  volume = {22},
  pages = {92--97},
}

@BOOK{Nelsen,
  title = {{An Introduction to Copulas}},
  publisher = {Springer},
  year = {1998},
  author = {R. B. Nelsen},
  number = {139},
  series = {Lecture Notes in Statistics},
  note = {ISBN 0-387-98623-5},
}

@BOOK{NelsenKrickeberg,
  title = {{An Introduction to Copulas}},
  publisher = {Springer},
  year = {1999},
  author = {R. B. Nelsen and K. Krickeberg},
  month = {June},
}

@ARTICLE{NengjiuJuAsian,
  author = {Nengjiu Ju},
  title = {{Pricing Asian and Basket Options via Taylor expansion of the underlying
	volatility}},
  journal = {Journal of Computational Finance},
  year = {2002},
  volume = {5},
  pages = {79--103},
  number = {3},
  month = {Spring},
  note = {\url{www.rhsmith.umd.edu/faculty/nju/JuJCF02.pdf}},
}

@PHDTHESIS{Neuhaus89,
  author = {H. Neuhaus},
  title = {{Option Valuation and Hedging under Transaction Costs}},
  school = {London Business School},
  year = {1989},
  address = {University of London},
  month = {December},
}

@INCOLLECTION{NeuhausKusuda,
  author = {H. Neuhaus and Y. Kusuda},
  title = {{Pricing and Hedging Equity Options: The Effect of Market Structure
	and Transaction Costs}},
  booktitle = {{Equity Derivatives}},
  publisher = {Risk Publications},
  year = {1997},
  month = {November},
}

@ARTICLE{Newton1991,
  author = {N. J. Newton},
  title = {{Asymptotically efficient Runge-Kutta methods for a class of Ito
	and Stratonovich equations}},
  journal = {SIAM Journal of Applied Mathematics},
  year = {1991},
  volume = {51},
  pages = {542--567},
  owner = {gbjaep},
}

@ARTICLE{Newton1994,
  author = {N. J. Newton},
  title = {{Variance reduction for simulated diffusions}},
  journal = {Siam Journal of Applied Mathematics},
  year = {1994},
  volume = {54},
  pages = {1780--1805},
  owner = {gbjaep},
}

@ARTICLE{NicolatoVenardos,
  author = {E. Nicolato and E. Venardos},
  title = {{Option Pricing in Stochastic Volatility Models of the Ornstein-Uhlenbeck
	type}},
  journal = {Mathematical Finance},
  year = {2003},
  volume = {13},
  pages = {445--466},
  number = {4},
  month = {October},
  note = {\url{www.cls.dk/caf/wp/wp-108.pdf}},
}

@BOOK{NiederreiterHellekalekLarcherZinterhof,
  title = {{Monte Carlo and Quasi-Monte Carlo Methods}},
  publisher = {Springer},
  year = {1997},
  editor = {H. Niederreiter and P. Hellekalek and G. Larcher and P. Zinterhof},
  volume = {127},
  series = {Lecture Notes in Statistics},
}

@ARTICLE{NonBlockingAlgorithms,
  author = {Maged M. Michael and Michael L. Scott},
  title = {{Non-Blocking Algorithms and Preemption-Safe Locking on Multiprogrammed
	Shared Memory Multiprocessors}},
  journal = {Journal of Parallel and Distributed Computing},
  year = {1998},
  volume = {51},
  pages = {1--26},
  number = {1},
  note = {\url{www.cs.rochester.edu/u/scott/papers/1998_JPDC_nonblocking.pdf}},
}

@TECHREPORT{NonRecombiningRadhakrishnan,
  author = {A. R. Radhakrishnan},
  title = {{An Empirical Study of the Convergence Properties of the Non-recombining
	HJM Forward Rate Tree in Pricing Interest Rate Derivatives}},
  institution = {Department of Finance, Stern School of Business, New York University},
  year = {1998},
  type = {Working paper},
  address = {9-190 P, 44 West 4th Street, New York, NY 10012-1126},
  note = {\url{www.stern.nyu.edu/~aradhakr}},
}

@BOOK{NumRec,
  title = {{Numerical Recipes in C}},
  publisher = {Cambridge University Press},
  year = {1992},
  author = {W. H. Press and S. A. Teukolsky and W. T. Vetterling and B. P. Flannery},
  note = {\url{http://www.nrbook.com/a/bookcpdf.php}},
}

@BOOK{OFKMNS,
  title = {{Equity Derivatives: Theory and Applications}},
  publisher = {John Wiley and Sons},
  year = {2002},
  author = {M. Overhaus and A. Ferraris and T. Knudsen and R. Milward and L.
	Nguyen-Ngoc and G. Schindlmayr},
  month = {February},
}

@BOOK{Oksendal,
  title = {{Stochastic Differential Equations}},
  publisher = {Springer},
  year = {1998},
  author = {B. {\O}ksendal},
  edition = {5th},
  note = {ISBN 3540637206},
}

@ARTICLE{OrnsteinUhlenbeck1930,
  author = {G.E. Uhlenbeck and L.S. Ornstein},
  title = {{On the theory of Brownian motion}},
  journal = {Physics Review},
  year = {1930},
  volume = {36},
  pages = {823--841},
  owner = {gbjaep},
}

@TECHREPORT{PJBushyTrees,
  author = {P. J{\"a}ckel},
  title = {{Non-recombining trees for the pricing of interest rate derivatives
	in the BGM/J framework}},
  institution = {NatWest Group / Royal Bank of Scotland},
  year = {2000},
  type = {Published report},
  address = {135 Bishopsgate, London EC2M 3UR},
  month = {July},
  note = {\url{www.quarchome.org/BushyTrees.pdf}},
}

@BOOK{PJMC,
  title = {{Monte Carlo methods in finance}},
  publisher = {John Wiley and Sons},
  year = {2002},
  author = {P. J{\"a}ckel},
  month = {February},
}

@ARTICLE{PJMindTheCap,
  author = {P. J{\"a}ckel},
  title = {{Mind the Cap}},
  journal = {Wilmott},
  year = {2003},
  pages = {54--68},
  month = {September},
  note = {\url{www.jaeckel.org/MindTheCap.pdf}},
}

@MISC{PJMonteCarloBermudan,
  author = {Peter J{\"a}ckel},
  title = {{Monte Carlo in the BGM/J framework: Using a non-recombining tree
	to design a new pricing method for Bermudan swaptions}},
  howpublished = {Maths Week (a RISK Conference), London},
  year = {2000},
  note = {\url{www.quarchome.org/MonteCarloBermudan.pdf}},
}

@MISC{PJPrimitivePolynomials,
  author = {P. J{\"a}ckel},
  title = {{Maple V routine for the calculation of a static table of primitive
	polynomials modulo~2}},
  howpublished = {\url{www.nr.com/contrib/}},
  year = {1997},
}

@article{PardouxTalay85,
   author={E. Pardoux and M. Talay},
   title={{Discretization and simulation of stochastic differential equations}},
   journal={{Acta Applicandae Mathematica}},
   volume={3},
   year= 1985,
   pages={23--47}
}

@ARTICLE{ParkMiller,
  author = {S. K. Park and K. W. Miller},
  title = {{Random Number Generators: Good Ones Are Hard to Find}},
  journal = {Communications of the ACM},
  year = {1988},
  volume = {31},
  pages = {1192--1201},
  number = {10},
  month = {October},
}

@ARTICLE{Parkinson,
  author = {M. Parkinson},
  title = {{Option Pricing: The American Put}},
  journal = {Journal of Business},
  year = {1977},
  volume = {50},
  pages = {21--36},
  month = {January},
}

@ARTICLE{PaskovTraub95,
  author = {S. H. Paskov and J. F. Traub},
  title = {{Faster Valuation of Financial Derivatives}},
  journal = {Journal of Portfolio Management},
  year = {1995},
  volume = {22},
  pages = {113--120},
  number = {1},
  note = {There are also several Columbia University technical reports on the
	subject},
  key = {FINDER software},
}

@ARTICLE{PatHagan,
  author = {P. Hagan and D. Kumar and A. S. Lesniewski},
  title = {{Managing Smile Risk}},
  journal = {Wilmott},
  year = {2002},
  pages = {84--108},
  month = {September},
}

@ARTICLE{PatHaganConvexity,
  author = {P. Hagan},
  title = {{Convexity Conundrums: Pricing CMS Swaps, Caps, and Floors}},
  journal = {Wilmott},
  year = {2003},
  pages = {38--44},
  month = {March},
}

@BOOK{PatelRead,
  title = {{Handbook of the Normal Distribution}},
  publisher = {Marcel Dekker Inc},
  year = {1982,1996},
  author = {J. K. Patel and C. B. Read},
  note = {ISBN 0824793420},
}

@ARTICLE{PeacemanRachford,
  author = {D. W. Peaceman and H. H. Rachford},
  title = {{The numerical solution of parabolic and elliptic differential equations}},
  journal = {Journal of the Society for Industrial and Applied Mathematics},
  year = {1955},
  volume = {3},
  pages = {28--41},
}

@TECHREPORT{Pedersen,
  author = {C.M. Pedersen},
  title = {{Valuation of Portfolio Credit Default Swaptions}},
  institution = {Fixed Income Quantitative Credit Research, Lehman Brothers},
  year = {2003},
  month = {November},
}

@TECHREPORT{PelsserBeenen,
  author = {A. Pelsser and J. Beenen},
  title = {{Convexity correction products}},
  institution = {ABN AMRO},
  year = {2000},
  month = {May},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@ARTICLE{PelsserConvexity,
  author = {A. Pelsser},
  title = {{Mathematical foundation of convexity correction}},
  journal = {Quantitative Finance},
  year = {2003},
  volume = {3},
  pages = {59--65},
  number = {1},
  note = {\url{www.iop.org/EJ/article/1469-7688/3/1/306/qf3106.pdf}},
}

@TECHREPORT{PelsserIrregularSwaptions,
  author = {A. Pelsser},
  title = {{Multi-Factor Pricing Model for Irregular Swaptions}},
  institution = {ABN AMRO},
  year = {2000},
  month = {February},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70030EC0C.nsf/h_Index/699B5E7BF0001556C1256F4900463708/?OpenDocument}},
}

@ARTICLE{PhilippeHuu,
  author = {Philippe Khuong-Huu},
  title = {{Swaptions with a smile}},
  journal = {Risk},
  year = {1999},
  pages = {107--111},
  month = {August},
}

@TECHREPORT{PhillipsLatinHyperCube,
  author = {S. Phillips},
  title = {{Latin hypercube variance reduction applied to credit derivative
	portfolio products}},
  institution = {ABN AMRO},
  year = {2004},
  month = {April},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@TECHREPORT{PhillipsRoggeCDORiskDates,
  author = {S. Phillips and E. Rogge},
  title = {{CDOs with a RiskEndDate and a RiskFreeEndDate}},
  institution = {ABN AMRO},
  year = {2005},
  month = {March},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@TECHREPORT{PhillipsRoggeJaeckelCMCDS,
  author = {S. Phillips and E. Rogge and P. J{\"a}ckel},
  title = {{Constant Maturity Credit Default Swaps}},
  institution = {ABN AMRO},
  year = {2004},
  month = {December},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@ARTICLE{Pickover,
  author = {C. A. Pickover},
  title = {{A note on chaos and Halley's method}},
  journal = {Communications of the ACM},
  year = {1988},
  volume = {31},
  pages = {1326--1329},
  number = {11},
  month = {November},
}

@TECHREPORT{PieterszPelsserRegenmortel,
  author = {R. Pietersz and A. Pelsser and M. van Regenmortel},
  title = {{Fast drift approximated pricing in the BGM model}},
  institution = {Erasmus University Rotterdam},
  year = {2002},
  type = {Working paper},
  note = {\url{www.few.eur.nl/few/people/pelsser/papers/Pietersz_Pelsser_vanRegenmortel-FastDriftApproxBGM-02.pdf}},
}

@TECHREPORT{PieterszRegenmortelGenericMarketModels,
  author = {R. Pietersz and M. van Regenmortel},
  title = {{Generic Market Models}},
  institution = {ABN AMRO},
  year = {2005},
  month = {January},
  note = {\url{ssrn.com/abstract=605301}},
}

@ARTICLE{PiterbargCallableLibor,
  author = {V. Piterbarg},
  title = {{Computing deltas of callable Libor exotics in forward Libor models}},
  journal = {Journal of Computational Finance},
  year = {2003},
  volume = {7},
  number = {3},
  note = {\url{ssrn.com/abstract=396180}},
}

@TECHREPORT{PiterbargMixtureOfModels,
  author = {V. Piterbarg},
  title = {{Mixture of Models: A Simple Recipe for a ... Hangover ?}},
  institution = {Bank of America},
  year = {2003},
  note = {\url{ssrn.com/abstract=393060}},
}

@TECHREPORT{PiterbargStochasticVolatilityLiborMarketModel,
  author = {V. Piterbarg},
  title = {{A Stochastic Volatility Forward Libor Model with a Term Structure
	of Volatility Smiles}},
  institution = {Bank of America},
  year = {2003},
  note = {\url{ssrn.com/abstract=472061}},
}

@TECHREPORT{Platen,
  author = {E. Platen},
  title = {{Consistent Pricing and Hedging for a Modified Constant Elasticity
	of Variance Model}},
  institution = {University of Technology Sydney},
  year = {2002},
  type = {presented at the Quantitative Finance London 2002 conference},
  month = {November 25},
}

@ARTICLE{Poincare,
  author = {H. Poincar{\'e}},
  title = {{Sur les int{\'e}grales irreguli{\`e}res des {\'e}quations line{\'e}aires}},
  journal = {Acta mathematica},
  year = {1886},
  volume = {8},
  pages = {295--344},
}

@ARTICLE{Press1967,
  author = {J. S. Press},
  title = {{A compound events model for security prices}},
  journal = {Journal of Business},
  year = {1967},
  volume = {40},
  pages = {317--335},
  month = {July},
}

@TECHREPORT{RANDCorporation,
  author = {B. Brown},
  title = {{Some Tests of the Randomness of a Million Digits}},
  institution = {The RAND corporation},
  year = {1948},
  number = {RAOP-44},
  address = {Santa Monica, California},
  month = {October 19},
}

@ARTICLE{RRJCF,
  author = {R. Rebonato},
  title = {{On the simultaneous calibration of multifactor lognormal interest
	rate models to Black volatilities and to the correlation matrix}},
  journal = {Journal of Computational Finance},
  year = {1999},
  volume = {2},
  pages = {5--27},
  number = {4},
  month = {Summer},
}

@ARTICLE{RRRisk,
  author = {R. Rebonato},
  title = {{Calibration of the {{BGM}} model}},
  journal = {Risk},
  year = {1999},
  volume = {March},
  pages = {74--79},
}

@TECHREPORT{Razak,
  author = {S. Razak},
  title = {{The Term Structure of Default in Copula Models}},
  institution = {Bear Stearns},
  year = {2003},
  type = {Working paper},
  note = {\url{www.geocities.com/shaloub_razak/TSDCM.pdf}},
}

@BOOK{Rebonato1,
  title = {{Interest Rate Option Models}},
  publisher = {John Wiley and Sons},
  year = {1998},
  author = {R. Rebonato},
}

@BOOK{Rebonato2,
  title = {{Volatility and Correlation}},
  publisher = {John Wiley and Sons},
  year = {1999},
  author = {R. Rebonato},
}

@BOOK{Rebonato3,
  title = {{Modern Pricing of Interest-Rate Derivatives}},
  publisher = {Princeton University Press},
  year = {2002},
  author = {R. Rebonato},
}

@ARTICLE{RebonatoJaeckelAmericanReplication,
  author = {P. J{\"a}ckel and R. Rebonato },
  title = {{Valuing American options in the presence of user-defined smiles
	and time-dependent volatility: scenario analysis, model stress and
	lower-bound pricing applications}},
  journal = {Journal of Risk},
  year = {2001},
  volume = {4},
  pages = {35--61},
  number = {1},
  month = {Fall},
  note = {\url{www.jaeckel.org/AmericanReplicationInThePresenceOfUserDefinedSmileDynamics.pdf}},
}

@ARTICLE{RebonatoJaeckelCorrelationMatrix,
  author = {R. Rebonato and P. J{\"a}ckel},
  title = {{The most general methodology to create a valid correlation matrix
	for risk management and option pricing purposes}},
  journal = {Journal of Risk},
  year = {1999/2000},
  volume = {2},
  number = {2},
  month = {Winter},
  note = {\url{www.quarchome.org/correlationmatrix.pdf}},
}

@MISC{Reese,
  author = {G. Reese},
  title = {{Buffon's Needle: An Analysis and Simulation}},
  howpublished = {\url{www.mste.uiuc.edu/reese/buffon/buffon.html}},
  year = {2001},
  note = {(a nice web application for demonstration)},
}

@TECHREPORT{RegenmortelGenericCorrelationApproach,
  author = {M. van Regenmortel},
  title = {{Generic Correlation Approach}},
  institution = {ABN AMRO},
  year = {2003},
  month = {May}
}

@TECHREPORT{RegenmortelValidationOfConvexity,
  author = {M. Regenmortel},
  title = {{Validation of the convexity framework for single index products}},
  institution = {ABN AMRO},
  year = {2000},
  month = {March},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@INPROCEEDINGS{Reiner,
  author = {E. Reiner},
  title = {{Understanding Skew and Smile Behaviour in the Context of Jump Processes
	and Applying These Results to the Pricing and Hedging of Exotic Options}},
  booktitle = {{Global Derivatives Conference 1998}},
  year = {1998},
  address = {Paris},
  month = {April},
}

@INPROCEEDINGS{ReinerDavidovKumanduri,
  author = {E. Reiner and D. Davidov and R. Kumanduri},
  title = {{A rapidly convergent expansion method for Asian and Basket options}},
  booktitle = {{Risk Europe}},
  year = {2001},
  address = {Paris},
  month = {April 11th},
  note = {\url{finmath.stanford.edu/seminars/docs/ASIANTLJ.pdf}},
}

@BOOK{Ripley,
  title = {{Stochastic Simulation}},
  publisher = {John Wiley and Sons},
  year = {1987},
  author = {B. D. Ripley},
}

@BOOK{RiskManagementAndAnalysisI,
  title = {{Risk Management and Analysis: Volume 1: Measuring and Modeling Financial
	Risk}},
  publisher = {John Wiley and Sons},
  year = {1998},
  author = {C. Alexander},
}

@BOOK{RiskManagementAndAnalysisII,
  title = {{Risk Management and Analysis: Volume 2: New Markets and Products}},
  publisher = {John Wiley and Sons},
  year = {1998},
  author = {C. Alexander},
}

@ARTICLE{RitchkenSankarasubramanianI,
  author = {P. Ritchken and L. Sankarasubramanian},
  title = {{Volatility Structures of Forward Rates and the Dynamics of the Term
	Structure}},
  journal = {Mathematical Finance},
  year = {1995},
  volume = {5},
  pages = {55--72},
  number = {1},
  note = {\url{weatherhead.cwru.edu/ritchken/Research_stuf/Sankar.pdf}},
}

@ARTICLE{RitchkenSankarasubramanianII,
  author = {P. Ritchken and L. Sankarasubramanian},
  title = {{The Importance of Forward-Rate Volatility Structures in Pricing
	Interest Rate-Sensitive Claims}},
  journal = {Journal of Derivatives},
  year = {1995},
  pages = {24--41},
  month = {Fall},
  note = {\url{weatherhead.cwru.edu/ritchken/Research_stuf/Sankar.pdf}},
}

@BOOK{RogersI,
  title = {{Diffusions, Markov Processes, and Martingales: Volume 1, Foundations}},
  publisher = {Cambridge University Press},
  year = {2000},
  author = {L. C. G. Rogers and D. Williams},
  month = {April},
  optnote = {ISBN 0521775949},
}

@BOOK{RogersII,
  title = {{Diffusions, Markov Processes and Martingales: Volume 2, Ito Calculus}},
  publisher = {Cambridge University Press},
  year = {2000},
  author = {L. C. G. Rogers and D. Williams},
  month = {September},
  optnote = {ISBN 0521775930},
}

@TECHREPORT{RoggeCDO2,
  author = {E. Rogge},
  title = {{CDO$^2$}},
  institution = {ABN AMRO},
  year = {2004},
  month = {March},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@TECHREPORT{RoggeCDO2Variation,
  author = {E. Rogge},
  title = {{CDO$^2$}},
  institution = {ABN AMRO},
  year = {2004},
  month = {September},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@TECHREPORT{RoggeCDOContingentIRS,
  author = {E. Rogge},
  title = {{Contingent interest rate swaps linked to basket \& portfolio credit
	risk}},
  institution = {ABN AMRO},
  year = {2004},
  month = {October},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Index/0FB18F19FA5CE042C125703D002D6B34/?OpenDocument}},
}

@TECHREPORT{RoggeCDOVariations,
  author = {E. Rogge},
  title = {{Tranche default swaps additional variations}},
  institution = {ABN AMRO},
  year = {2001},
  month = {December},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@TECHREPORT{RoggeCreditContingentIRS,
  author = {E. Rogge},
  title = {{Credit Contingent Interest Rate Swaps}},
  institution = {ABN AMRO},
  year = {2003},
}

@TECHREPORT{RoggeNDB,
  author = {E. Rogge},
  title = {{N$^{th}$ -to-Default Swaps on Corporates}},
  institution = {ABN AMRO},
  year = {2000},
  month = {July},
  note = {\url{http://nlas-00033/source/Product%20Development%20Group/Documentation/PDF/nth-to-default.doc}},
}

@TECHREPORT{RoggeSchoenbucherDynamicPortfolioCreditRisk,
  author = {E. Rogge and P. J. Sch{\"o}nbucher},
  title = {{Modelling dynamic portfolio credit risk}},
  institution = {ABN AMRO, London, and Department of Mathematics, ETH Z{\"u}rich,
	Switzerland},
  year = {2003},
  type = {Working paper},
  month = {February},
  note = {\url{math.ethz.ch/~schonbuc/papers/schonbucher_rogge_dynamiccreditrisk.pdf}},
}

@TECHREPORT{RoggeSemiAnalytical,
  author = {E. Rogge},
  title = {{Efficient pricing of multiname credit derivatives}},
  institution = {ABN AMRO},
  year = {2003},
  month = {September},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@TECHREPORT{RoggeTDBswaps,
  author = {E. Rogge},
  title = {{Tranche default swaps}},
  institution = {ABN AMRO},
  year = {2001},
  month = {May},
  note = {\url{http://nlas-00033/source/Product%20Development%20Group/Documentation/PDF/CDOs/tranche.pdf}},
}

@TECHREPORT{Roncalli,
  author = {T. Roncalli},
  title = {{Statistical Methods in Integrated Risk Management}},
  institution = {Groupe de Recherche Operationnelle Credit Lyonnais},
  year = {2001},
  month = {January},
  note = {\url{www.gloriamundi.org/picsresources/copula-paris-jan2001-part2.pdf}},
}

@BOOK{Rubinstein,
  title = {{Simulation and the Monte Carlo method}},
  publisher = {John Wiley and Sons},
  year = {1981},
  author = {R. Y. Rubinstein},
  series = {Wiley series in probability and mathematical statistics},
  note = {ISBN 0-471-08917-6},
}

@ARTICLE{RubinsteinCompoundOptions,
  author = {M. Rubinstein},
  title = {{Double Trouble}},
  journal = {Risk},
  year = {1991},
  volume = {4},
  month = {December},
}

@ARTICLE{RubinsteinReiner,
  author = {E. Reiner and M. Rubinstein},
  title = {{Breaking Down the Barriers}},
  journal = {Risk},
  year = {1991},
  volume = {4},
  pages = {30--35},
  number = {8},
  month = {September},
  note = {A useful web site with most simple barrier formul\ae is at \url{www.global-derivatives.com/options/barrier-options.php}},
}

@ARTICLE{RubinsteinSmile,
  author = {M. Rubinstein},
  title = {{Implied binomial trees}},
  journal = {Journal of Finance},
  year = {1994},
  volume = {49},
  pages = {771--818},
  number = {3},
}

@TECHREPORT{RytenSeasonalityAndShortTermInflationForecasting,
  author = {M. Ryten},
  title = {{Seasonality and Short Term Inflation Forecasting in CAL Inflation Curves}},
  institution = {ABN AMRO},
  year = {2005},
  month = {August},
  note = {\url{file://nlas-00033.emea.abnamro-net.com/source/Product%20Development%20Group/Documentation/TeX/SeasonalityAndShortTermInflationForecasting/SeasonalityAndShortTermInflationForecasting.pdf}},
}

@TECHREPORT{RytenInflationCapStripping,
  author = {M. Ryten},
  title = {{Inflation Cap Stripping Using the Year On Year Inflation Exponential Mean Reversion Model}},
  institution = {ABN AMRO},
  year = {2005},
  month = {October},
  note = {\url{file://nlas-00033.emea.abnamro-net.com/source/Product%20Development%20Group/Documentation/TeX/InflationCapStripping/InflationCapStripping.pdf}},
}

@TECHREPORT{RytenYearOnYearInflationMeanReversionModelNotes,
  author = {M. Ryten},
  title = {{The Year On Year Inflation Exponential Mean Reversion Model}},
  institution = {ABN AMRO},
  year = {2005},
  month = {June},
  note = {\url{file://nlas-00033.emea.abnamro-net.com/source/Product%20Development%20Group/Documentation/TeX/YearOnYearInflationMeanReversionModel/YearOnYearInflationMeanReversionModel.pdf}},
}

@ARTICLE{Samuelson65,
  author = {P. Samuelson},
  title = {{Rational Theory of Warrant Pricing}},
  journal = {Industrial Management Review},
  year = {1965},
  volume = {6},
  pages = {13--31},
  number = {2},
  month = {Spring},
}

@TECHREPORT{SandmannSondermann1994,
  author = {K. Sandmann and D. Sondermann},
  title = {{On the stability of log-normal interest rate models and the pricing
	of Eurodollar futures}},
  institution = {Dept. of Statistics, Faculty of Economics, SFB 303, Universit{\"a}t
	Bonn},
  year = {1994},
  type = {Discussion paper},
  month = {June},
  note = {\url{ftp://ftp.wipol.uni-bonn.de/pub/RePEc/bon/bonsfb/bonsfb263.pdf}},
  abstract = {The lognormal distribution assumption for the term structure of interest
	is the most natural way to exclude negative spot and forward rates.
	However, imposing this assumption on the continuously compounded
	interest rate has a serious drawback: expected rollover returns are
	infinite even if the rollover period is arbitrarily short. As a consequence
	such models cannot price one of the most widely used hedging instrument
	on the Euromoney market, namely the Eurofuture contract. The purpose
	of this paper is to show that the problem with lognormal models result
	from modelling the wrong rate, namely the continuously compounded
	rate. If instead one models the effective annual rate the problem
	disappears, i.e. the expected rollover returns are finite. The paper
	studies the resulting dynamics of the continuously compounded rate
	which is neither normal nor lognormal.},
  annote = {Document code B-263},
}

@ARTICLE{SandmannSondermann1997,
  author = {K. Sandmann and D. Sondermann},
  title = {{A Note on the Stability of Lognormal Interest Rate Models and the
	Pricing of Eurodollar Futures}},
  journal = {Mathematical Finance},
  year = {1997},
  volume = {7},
  pages = {119},
  number = {2},
  month = {April},
  abstract = {The lognormal distribution assumption for the term structure of interest
	is the most natural way to exclude negative spot and forward rates.
	However, imposing this assumption on the continuously compounded
	interest rate has a serious drawback: rates explode and expected
	rollover returns are infinite even if the rollover period is arbitrarily
	short. As a consequence, such models cannot price one of the most
	widely used hedging instruments on the Euromoney market, namely the
	Eurodollar futures contract. The purpose of this note is to show
	that the problems with lognormal models result from modeling the
	wrong rate, namely the continuously compounded rate. If instead one
	models the effective annual rate these problems disappear.},
  annote = {Document code B-263},
  doi = {10.1111/1467-9965.00027},
  institution = {Dept. of Statistics, Faculty of Economics, SFB 303, Universit{\"a}t
	Bonn},
  type = {Discussion paper},
}

@TECHREPORT{SandmannSondermann1997b,
  author = {K. Sandmann and D. Sondermann},
  title = {{Log-Normal Interest Rate Models: Stability and Methodology}},
  institution = {Dept. of Statistics, Faculty of Economics, SFB 303, Universit{\"a}t
	Bonn},
  year = {1997},
  type = {Discussion paper},
  month = {January},
  note = {\url{ftp://ftp.wipol.uni-bonn.de/pub/RePEc/bon/bonsfb/bonsfb398.pdf}},
  abstract = {The lognormal distribution assumption for the term structure of interest
	is the most natural way to exclude negative spot and forward rates.
	However, imposing this assumption on the continuously compounded
	interest rate has a serious drawback: rates explode and expected
	rollover returns are infinite even if the rollover period is arbitrarily
	short. As a consequence such models cannot price one of the most
	widely used hedging instrument on the Euromoney market, nameley the
	Eurodollar future contract. The purpose of this paper is twofold:
	First to show that the problems with lognormal models result from
	modelling the wrong rate, namely the continuously compounded rate.
	If instead one models the effective annual rate these problems disappear.
	Second to give a survey on recent work on lognormal term structure
	models for effective or nominal forward rates.},
  annote = {Document code B-263},
}

@BOOK{Sato,
  title = {{L{\'e}vy Processes and Infinitely Divisible Distributions}},
  publisher = {Cambridge University Press},
  year = {1999},
  author = {Ken-iti Sato},
  month = {November},
}

@ARTICLE{ScavoThoo,
  author = {T. R. Scavo and J. B. Thoo},
  title = {{On the Geometry of Halley's Method}},
  journal = {Amer. Math. Monthly},
  year = {1995},
  volume = {102},
  pages = {417--426},
}

@ARTICLE{Schloegl,
  author = {E. Schl{\"o}gl},
  title = {{A multicurrency extension of the lognormal interest rate market
	models}},
  journal = {Finance and Stochastics},
  year = {2002},
  volume = {6},
  pages = {173--196},
}

@ARTICLE{SchoebelZhu,
  author = {R. Sch{\"o}bel and J. Zhu},
  title = {{Stochastic Volatility With an Ornstein Uhlenbeck Process: An Extension}},
  journal = {European Finance Review},
  year = {1999},
  volume = {3},
  pages = {23--46},
  note = {\url{ssrn.com/abstract=100831}},
}

@TECHREPORT{Schoenbucher,
  author = {P. J. Sch{\"o}nbucher},
  title = {{A Market Model for Stochastic Implied Volatility}},
  institution = {Dept. of Statistics, Faculty of Economics, SFB 303, Universit{\"a}t
	Bonn},
  year = {1998},
  type = {Discussion paper},
  month = {June},
  note = {\url{ftp.wiwi.uni-bonn.de/papers/1999/b/bonnsfb453.pdf}},
  annote = {Document code B-453, JEL-Classification-Number: G 13},
}

@BOOK{SchoenbucherCredit,
  title = {{Credit Derivates Pricing Models}},
  publisher = {John Wiley and Sons},
  year = {2003},
  author = {P. J. Sch{\"o}nbucher},
}

@TECHREPORT{SchoenbucherCreditDefaultSwaptions,
  author = {P. J. Sch{\"o}nbucher},
  title = {{A Note on Survival Measures and the Pricing of Options on Credit
	Default Swaps}},
  institution = {Department of Mathematics, ETH Z{\"u}rich, Switzerland},
  year = {2003},
  type = {Working paper},
  month = {May},
  note = {\url{www.math.ethz.ch/~schonbuc/papers/cdsoptions.pdf}},
}

@TECHREPORT{SchoenbucherCreditLibor,
  author = {P. J. Sch{\"o}nbucher},
  title = {{A LIBOR market model with default risk}},
  institution = {Dept. of Statistics, Faculty of Economics, SFB 303, Universit{\"a}t
	Bonn},
  year = {2000},
  type = {Discussion paper},
  month = {December},
  note = {\url{www.hermes.ucy.ac.cy/publications/conference_may_2000/Schonbucher.pdf}},
}

@TECHREPORT{SchoenbucherSimpleLoanDistributions,
  author = {P. J. Sch{\"o}nbucher},
  title = {{Taken to the limit: simple and not-so-simple loan loss distributions}},
  institution = {Dept. of Statistics, Faculty of Economics, Universit{\"a}t Bonn},
  year = {2002},
  type = {Discussion paper},
  month = {August},
  note = {\url{defaultrisk.com/pdf__files/Taken_To_the_Limit-Smpl_n_Nt-s-smpl_Ln_Lss_Dstrbtns.pdf}},
  annote = {JEL-Classification-Number: G 13},
}

@TECHREPORT{Schoenmakers,
  author = {J. G. M. Schoenmakers},
  title = {{Calibration of LIBOR models to caps and swaptions: a way around
	intrinsic instabilities via parsimonious structures and a collateral
	market criterion}},
  institution = {Weierstrass Institute, Berlin},
  year = {2000},
  type = {Working paper},
  note = {\url{www.wias-berlin.de/publications/preprints/740}},
}

@TECHREPORT{SchoenmakersCoffey,
  author = {J. G. M. Schoenmakers and B. Coffey},
  title = {{Stable implied calibration of a multi-factor LIBOR model via a semi-parametric
	correlation structure}},
  institution = {Weierstrass Institute, Berlin},
  year = {2000},
  type = {Working paper},
  note = {\url{www.wias-berlin.de/publications/preprints/611}},
}

@ARTICLE{Schroder,
  author = {M. Schroder},
  title = {{Computing the Constant Elasticity of Variance Option Pricing Formula}},
  journal = {Journal of Finance},
  year = {1989},
  volume = {44},
  pages = {211--219},
  number = {1},
  month = {March},
  note = {\url{home.ust.hk/jinzhang/ust/Schroder_JF.pdf}},
  optkey = {CEV},
}

@ARTICLE{SchroederBuffon,
  author = {L. Schroeder},
  title = {{Buffon's needle problem: An exciting application of many mathematical
	concepts}},
  journal = {Mathematics Teacher},
  year = {1974},
  volume = {67},
  pages = {183--186},
  number = {2},
}

@ARTICLE{Schurz1996,
  author = {H. Schurz},
  title = {{Numerical Regularization for SDE's: Construction of nonnegative
	solutions}},
  journal = {Dynamical Systems and Applications},
  year = {1996},
  volume = {5},
  pages = {323--352},
  owner = {gbjaep},
}

@ARTICLE{Scott,
  author = {L. Scott},
  title = {{Option Pricing When the Variance Changes Randomly: Theory, Estimation
	and An Application}},
  journal = {Journal of Financial and Quantitative Analysis},
  year = {1987},
  volume = {22},
  pages = {419--438},
  month = {December},
}

@ARTICLE{Sepp2004,
  author = {A. Sepp},
  title = {{Pricing European-Style Options under Jump Diffusion Processes with
	Stochastic Volatility: Applications of Fourier Transform}},
  journal = {Acta et Commentationes Universitatis Tartuensis de Mathematica},
  year = {2004},
  volume = {8},
  pages = {123-133},
  note = {\url{math.ut.ee/~spartak/papers/stochjumpvols.pdf}},
  owner = {gbjaep},
}

@ARTICLE{Shannon,
  author = {C. E. Shannon},
  title = {{A mathematical theory of communication}},
  journal = {Bell System Technical Journal},
  year = {1948},
  volume = {27},
}

@ARTICLE{Shevchenko,
  author = {P. V. Shevchenko},
  title = {{Addressing the bias in Monte Carlo pricing of multi-asset options
	with multiple barriers through discrete sampling}},
  journal = {Journal of Computational Finance},
  year = {2003},
  volume = {6},
  pages = {1--20},
  number = {3},
}

@MISC{ShrevesLectureNotes,
  author = {S. E. Shreve},
  title = {{Stochastic Calculus Lecture Notes}},
  howpublished = {\url{www.math.cmu.edu/users/shreve}},
  year = {1998},
}

@TECHREPORT{SideniusPiterbargAndersenSPA,
  author = {J. Sidenius and V. Piterbarg and L. Andersen},
  title = {{A New Framework For Dynamic Credit Portfolio Loss Modelling}},
  institution = {},
  year = {2005},
  month = {November},
  note = {\url{http://www.happycool.com/papers/spa_vp_1.pdf}},
}

@BOOK{SmithNumericalPartialDifferentialEquations,
  title = {{Numerical Solution of Partial Differential Equations: Finite Difference
	Methods}},
  publisher = {Oxford University Press},
  year = {1986},
  author = {G. Smith},
  month = {January},
}

@ARTICLE{Sobol67,
  author = {I. M. Sobol'},
  title = {{On the Distribution of Points in a Cube and the Approximate Evaluation
	of Integrals}},
  journal = {USSR Computational Mathematics and Mathematical Physics},
  year = {1967},
  volume = {7},
  pages = {86--112},
}

@BOOK{Sobol69,
  title = {{Multidimensional Quadrature Formulas and Haar Functions (Mnogomernye
	Kvadraturnye Formuly i Funktsii Khaara)}},
  publisher = {Nauka},
  year = {1969},
  author = {I. M. Sobol'},
  address = {Moscow},
}

@ARTICLE{Sobol76,
  author = {I. M. Sobol'},
  title = {{Uniformly Distributed Sequences with an Additional Uniform Property}},
  journal = {USSR Computational Mathematics and Mathematical Physics},
  year = {1976},
  volume = {16},
  pages = {236--242},
  number = {5},
}

@ARTICLE{Sobol79,
  author = {I. M. Sobol'},
  title = {{On the Systematic Search in a Hypercube}},
  journal = {Siam J. Numer. Anal.},
  year = {1979},
  volume = {16},
  number = {5},
  month = {October},
}

@ARTICLE{Sobol98,
  author = {I. M. Sobol'},
  title = {{On quasi-Monte Carlo integrations}},
  journal = {Mathematics and Computers in Simulation},
  year = {1998},
  pages = {103--112},
  number = {47},
}

@BOOK{SobolsMonteCarloPrimer,
  title = {{A Primer for the Monte Carlo Method}},
  publisher = {CRC press},
  year = {1994},
  author = {I. M. Sobol'},
  note = {ISBN 084938673X128},
}

@ARTICLE{Sprenkle,
  author = {C. Sprenkle},
  title = {{Warrant Prices as Indicators of Expectations and Preferences}},
  journal = {Yale Economic Essays},
  year = {1961},
  volume = {1},
  pages = {178--231},
}

@INCOLLECTION{SprenkleInCootner,
  author = {C. Sprenkle},
  title = {{Warrant Prices as Indicators of Expectations and Preferences}},
  booktitle = {{The Random Character of Stock Market Prices}},
  publisher = {Cambridge, MIT Press},
  year = {1964},
  editor = {P. H. Cootner},
  pages = {412--474},
}

@ARTICLE{SteinAndStein,
  author = {E. M. Stein and J. C. Stein},
  title = {{Stock Price Distribution with Stochastic Volatility : An Analytic
	Approach}},
  journal = {Review of Financial Studies},
  year = {1991},
  volume = {4},
  pages = {727--752},
}

@ARTICLE{SteinerWallmeierHafner,
  author = {M. Steiner and M. Wallmeier and R. Hafner},
  title = {{Pricing near the barrier: the case of discrete knock-out options}},
  journal = {Journal of Computational Finance},
  year = {1999},
  volume = {3},
  pages = {69--90},
  number = {1},
}

@ARTICLE{Stieltjes,
  author = {Th. Stieltjes},
  title = {{Recherches sur quelques s{\'e}ries semi-convergentes}},
  journal = {Annales de l'Ec. Norm. Sup.},
  year = {1886},
  volume = {3},
  pages = {201--258},
  number = {3},
}

@MISC{StochasticVolatilityForLevyProcesses,
  author = {D. Madan},
  title = {{Stochastic volatility for L{\'e}vy processes}},
  howpublished = {\url{www.imub.ub.es/events/sssf/barcelona2001-2.pdf}},
  year = {2001},
}

@ARTICLE{Takahashi01,
  author = {A. Takahashi and T. Kobayashi and N. Nakagawan},
  title = {{Pricing convertible bonds with default risk}},
  journal = {Journal of Fixed Income},
  year = {2001},
  volume = {11},
  number = {20},
  month = {9},
}

@TECHREPORT{TanUserManualCorrelationEstimator,
  author = {C. Tan},
  title = {{User Manual Correlation Estimator and Mean Reversion Estimator}},
  institution = {ABNAMRO},
  year = {2004},
  type = {Working paper},
  month = {March},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256C69005198D5.nsf/h_Index/1634A69E61486868C1256C690054E101/?OpenDocument}},
}

@BOOK{TavellaRandall,
  title = {{Pricing Financial Instruments: The Finite Difference Method}},
  publisher = {John Wiley and Sons},
  year = {2000},
  author = {D. Tavella and C. Randall},
  month = {April},
  note = {ISBN 0471197602},
}

@BOOK{Tezuka,
  title = {{Uniform Random Numbers: Theory and Practice}},
  publisher = {Kluwer Academic Publishers},
  year = {1995},
  author = {S. Tezuka},
}

@BOOK{TheBestOfWilmottI,
  title = {{The Best of Wilmott 1: Including the latest research from Quantitative
	Finance Review 2003}},
  publisher = {John Wiley and Sons},
  year = {2004},
  editor = {P. Wilmott},
}

@BOOK{ThorpKassouf,
  title = {{Beat The Market: A Scientific Stock Market System}},
  publisher = {New York Random House},
  year = {1967},
  author = {E. O. Thorp and S. T. Kassouf},
}


@ARTICLE{ToftPrucyk,
  author = {K. B. Toft and B. Prucyk},
  title = {{Options on leveraged equity: Theory and empirical tests}},
  journal = {Journal of Finance},
  year = {1997},
  volume = {52},
  pages = {1151--1180},
  number = {3},
  month = {July},
}

@ARTICLE{Tsiveriotis98,
  author = {K. Tsiveriotis and C. Fernandes},
  title = {{Valuing convertible bonds with credit risk}},
  journal = {Journal of Fixed Income},
  year = {1998},
  volume = {8},
  pages = {95--102},
}

@TECHREPORT{TsouderosTwoAssetTriggerOption,
  author = {G. Tsouderos},
  title = {{Two-Asset Trigger Options}},
  institution = {ABN AMRO},
  year = {2005},
  month = {August},
}

@TECHREPORT{TsouderosVanishingSwaps,
  author = {G. Tsouderos},
  title = {{Vanishing Swaps Under Market And Credit Risk Correlation}},
  institution = {ABN AMRO},
  year = {2004},
  month = {August},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Index/C8839D3949B2099FC1256F8C005F53C8/?OpenDocument}},
}

@TECHREPORT{TsouderosWildHybridSwaption,
  author = {G. Tsouderos and L. Wild},
  title = {{Options on Hybrid Notional Irregular Swaps}},
  institution = {ABN AMRO},
  year = {2005},
  month = {April},
}

@ARTICLE{TurnbullWakeman,
  author = {S. Turnbull and L. Wakeman},
  title = {{A Quick Algorithm for Pricing European Average Options}},
  journal = {Journal of Financial and Quantitiative Analysis},
  year = {1991},
  volume = {26},
  pages = {377--390},
  number = {3},
}

@ARTICLE{UlamVonNeumann,
  author = {S. M. Ulam and J. von Neumann},
  title = {{On combinations of stochastic and deterministic processes}},
  journal = {Bulletin of the American Mathematical Society},
  year = {1947},
  volume = {53},
  pages = {1120},
  number = {11},
  month = {November},
  note = {Preliminary report from the summer meeting in New Haven},
}

@ARTICLE{Vasicek,
  author = {O. A. Vasicek},
  title = {{An equilibrium characterisation of the term structure}},
  journal = {Journal of Financial Economics},
  year = {1977},
  volume = {5},
  pages = {177--188},
}

@TECHREPORT{Vasicek1987,
  author = {O. A. Vasicek},
  title = {{Probability of loss on loan portfolio}},
  institution = {KMV},
  year = {1987},
  type = {Working paper},
  note = {\url{www.moodyskmv.com/research/whitepaper/Probability_of_Loss_on_Loan_Portfolio.pdf}},
}

@BOOK{VasicekAndBeyond,
  title = {{Vasicek and beyond}},
  publisher = {RISK publications},
  year = {1996},
  editor = {L. Hughston},
}

@INCOLLECTION{VonNeumannOnRandomDigits,
  author = {J. von Neumann},
  title = {{Various Techniques Used in Connection With Random Digits}},
  booktitle = {{Monte Carlo Method}},
  year = {1951},
  chapter = {13},
  pages = {36--38},
  month = {June},
  crossref = {NBSMonteCarloMethod},
}

@TECHREPORT{VoortCDOContingentIRSValidation,
  author = {M. van der Voort},
  title = {{Validation report on multi-name ccirs}},
  institution = {ABN AMRO},
  year = {2004},
  month = {November},
}

@TECHREPORT{VoortCMCDSValidation,
  author = {M. van der Voort},
  title = {{CMCDS\ Validation report}},
  institution = {ABN AMRO},
  year = {2004},
  month = {November},
}

@TECHREPORT{VoortCathayFDO,
  author = {M. van der Voort},
  title = {{One-Off Validation on Cathay Life FDO}},
  institution = {ABN AMRO},
  year = {2005},
  month = {June},
}

@TECHREPORT{VoortCathayFDONewCalibration,
  author = {M. van der Voort},
  title = {{DRAFT One-Off Validation on Cathay Life FDO New Calibration and Reserves}},
  institution = {ABN AMRO},
  year = {2005},
  month = {December},
}

@TECHREPORT{VoortWeddingNDBOneOff,
  author = {M. van der Voort},
  title = {{One Off Validation on N$^{th}$-to-Default Wedding Cake Structure}},
  institution = {ONE06-17 Product-Analysis},
  year = {2006},
  month = {February},
}

@ARTICLE{VorstBasketFormula,
  author = {T. Vorst},
  title = {{Prices and Hedge Ratios of Average Exchange Rate Options}},
  journal = {International Review of Financial Analysis},
  year = {1992},
  volume = {1},
  pages = {179--193},
  number = {3},
}

@TECHREPORT{VorstWiersingaNDBVAL,
  author = {T. Vorst and M. Wiersinga},
  title = {{Validation Report on N$^{th}$-to-Default Swaps}},
  institution = {VAL00-48 Product-Analysis},
  year = {2000},
  month = {December},
}

@TECHREPORT{VriesConvexity,
  author = {M. de Vries},
  title = {{Convexity corrections}},
  institution = {ABN AMRO},
  year = {2002},
  month = {November},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Toc/CE6A3D6B1F546C9405256708001671FF/?OpenDocument}},
}

@ARTICLE{Walsh,
  author = {J. B. Walsh},
  title = {{The rate of convergence of the binomial tree scheme}},
  journal = {Finance and Stochastics},
  year = {2003},
  volume = {7},
  pages = {337--361},
}

@MISC{WeissteinHalleysMethod,
  author = {E. Weisstein},
  title = {{Halley's Method}},
  note = {\url{mathworld.wolfram.com/HalleysMethod.html}},
}

@MISC{WeissteinHouseholdersMethod,
  author = {E. Weisstein},
  title = {{Householder's Method}},
  note = {\url{mathworld.wolfram.com/HouseholdersMethod.html}},
}

@ARTICLE{Wheeler,
  author = {R. E. Wheeler},
  title = {{Quantile estimators of Johnson curve parameters}},
  journal = {Biometrika},
  year = {1980},
  volume = {67},
  pages = {725--8},
}

@TECHREPORT{Whelan,
  author = {N. Whelan},
  title = {{Sampling from Archimedean Copulas}},
  institution = {Bank of Nova Scotia},
  year = {2003},
  type = {Working paper},
  note = {\url{home.golden.net/~annaw/Niall/papers/Archimedean.pdf}},
}

@article{Wiener1923,
		 author={Wiener, N.},
		 title={{Differential-space}},
		 journal={{Journal of Mathematics and Physics}},
		 volume={2},
		 year={1923},
		 pages={131--174}
}

@ARTICLE{Wiggins1987,
  author = {J. Wiggins},
  title = {{Option values under stochastic volatility: Theory and empirical
	estimates}},
  journal = {Journal of Financial Economics},
  year = {1987},
  volume = {19},
  pages = {351--372},
  owner = {gbjaep},
}

@TECHREPORT{WildL,
  author = {L. Wild},
  title = {{Valuation of Bermudan Swaptions in the Forward Risk Adjusted Measure}},
  institution = {The Royal Bank of Scotland Corporate Banking and Financial Markets},
  year = {2000},
  type = {Internal Report},
}

@TECHREPORT{WildTsouderosVanishingSwaps,
  author = {L. Wild and G. Tsouderos},
  title = {{Vanishing Swaps Under Market And Credit Risk Correlation - A Mean
	Reverting Intensity-Based Model}},
  institution = {ABN AMRO},
  year = {2005},
  month = {January},
  note = {\url{https://nlamsq001.inet.nl.abnamro.com/QuickPlace/qa-group/PageLibraryC1256BF70032A9A2.nsf/h_Index/C8839D3949B2099FC1256F8C005F53C8/?OpenDocument}},
}

@TECHREPORT{WillowTree,
  author = {M. Curran},
  title = {{Willow Power}},
  institution = {Quantin' Leap working paper},
  year = {1996},
  note = {\url{www.quantinleap.com}},
}

@BOOK{Wilmott,
  title = {{Derivatives}},
  publisher = {John Wiley and Sons},
  year = {1998},
  author = {P. Wilmott},
}

@BOOK{Wilmott2000,
  title = {{Quantitative Finance}},
  publisher = {John Wiley and Sons},
  year = {2000},
  author = {P. Wilmott},
}

@article{WongZakai65,
   author={E. Wong and M. Zakai},
   title={{On the convergence of ordinary integrals to stochastic integrals}},
   journal={{Ann. Math. Stat.}},
   volume={36},
   year= 1965,
   pages={1560--1564}
}

@ARTICLE{Wu,
  author = {L. Wu},
  title = {{Fast at-the-money calibration of the Libor market model using Lagrange
	multipliers}},
  journal = {Journal of Computational Finance},
  year = {2002/2003},
  volume = {6},
  pages = {39--72},
  number = {2},
  month = {Winter},
  nnote = {\url{www.math.ust.hk/~malwu/Publ/bgm.pdf}},
}

@MISC{XinSplittingMethods,
  author = {J. Xin},
  title = {{Time Splitting Methods}},
  note = {\url{www.ma.utexas.edu/~jxin/m383gfiles/m383glec14.pdf}},
}

@TECHREPORT{Zhou,
  author = {C. Zhou},
  title = {{A Jump-Diffusion Approach to Modeling Credit Risk and Valuing Defaultable
	Securities}},
  institution = {Federal Reserve Board},
  year = {1997},
  month = {March},
  note = {\url{www.federalreserve.gov/pubs/feds/1997/199715/199715pap.pdf}},
}

@ARTICLE{ZhuSun,
  author = {Y. I. Zhu and Y. Sun},
  title = {{The singularity-separating method for two-factor convertible bonds}},
  journal = {Journal of Computational Finance},
  year = {1999},
  volume = {3},
  pages = {91--110},
  number = {1},
  month = {Fall},
}

@TECHREPORT{Zuehlsdorffa,
  author = {C. Z{\"u}hlsdorff},
  title = {{The Pricing of Derivatives on Assets with Quadratic Volatility}},
  institution = {University of Bonn},
  year = {2002},
  type = {Working paper},
  note = {\url{ftp.wiwi.uni-bonn.de/papers/bgse/2002/bgse5_2002.pdf}},
}

@TECHREPORT{Zuehlsdorffb,
  author = {C. Z{\"u}hlsdorff},
  title = {{Extended Libor Market Models with Affine and Quadratic Volatility}},
  institution = {University of Bonn},
  year = {2002},
  type = {Working paper},
  note = {\url{ftp.wiwi.uni-bonn.de/papers/bgse/2002/bgse6_2002.pdf}},
}

@ARTICLE{ZvanForsythVetzal,
  author = {R. Zvan and P. A. Forsyth and K. R. Vetzal},
  title = {{Robust Numerical Methods for PDE Models of Asian Options}},
  journal = {Journal of Computational Finance},
  year = {1997/1998},
  volume = {1},
  pages = {39--78},
  number = {2},
  month = {Winter},
}

@MISC{carr-option,
  author = {P. Carr},
  title = {{Option Pricing using Integral Transforms}},
  year = {2003},
  note = {\url{www.math.nyu.edu/research/carrp/papers/pdf/integtransform.pdf}},
}


@ARTICLE{Rahman-BehrensFisher,
  author = {M. Rahman and A.K.Md. Ehsanes Saleh},
  title = {{Explicit Form Of The Distribution Of The Behrens Fisher $d$-Statistic}},
  journal = {Journal Of The Royal Statistical Society. Series B(Methodological)},
  year = {1974},
  volume = {36},
  pages = {54-60},
  number = {1},
}

@ARTICLE{Rahman-BehrensFisher-Corrigendum,
  author = {M. Rahman and A.K.Md. Ehsanes Saleh},
  title = {{Corrigendum:Explicit Form Of The Distribution Of The Behrens Fisher $d$-Statistic}},
  journal = {Journal Of The Royal Statistical Society. Series B(Methodological)},
  year = {1974},
  volume = {36},
  pages = {466},
  number = {3},
}


@BOOK{PeskinSchroeder,
  title = {{An Introduction to Quantum Field Theory}},
  publisher = {Perseus Books,U.S.},
  year = {2008},
  author = {M. E. Peskin, D. V. Schroeder},
}

@TECHREPORT{WolframAppellF1,
  author = {Wolfram Research, Inc. },
  title = {{Appell F1 hypergeometric Function}},
  note = {\url{http://functions.wolfram.com/HypergeometricFunctions/AppellF1/17/ShowAll.html}},
  year = {1998-2009},
}

@TECHREPORT{WolframErf,
  author = {Wolfram Research, Inc. },
  title = {{Erf Function: Integration Involving exp}},
  note = {\url{http://functions.wolfram.com/GammaBetaErf/Erf/21/ShowAll.html}},
  year = {1998-2009},
}


@BOOK{SiegelFields,
  title = {{FIELDS}},
  publisher = {\url{http://insti.physics.sunysb.edu/~siegel/Fields3.pdf}},
  note = {p443-444},
  author = {W. Siegel},
}

@ARTICLE{RubenBehrensFisher,
  author = {H. Ruben},
  title = {{On The Distribution Of The Weighted Difference Of Two Independent Student Variables}},
  journal = {Journal Of The Royal Statistical Society. Series B(Methodological)},
  year = {1960},
  volume = {22},
  pages = {188-194},
  number = {1},
}


@ARTICLE{VasicekPhi2,
  author = {O.A. Vasicek},
  title = {{A series expansion for the bivariate normal integral}},
  journal = {The Journal of Computational Finance},
  year = {1998},
  volume = {1},
  pages = {5-10},
  number = {4},
}

@ARTICLE{KouPetrellaWang,
  author = {S. Kou and G. Petrella and H. Wang},
  title = {{ Pricing Path-Dependent Options with Jump Risk via Laplace Transforms }},
  journal = {The Kyoto Economic Review},
  year = {June 2005},
  volume = {74},
  pages = {1-23},
  number = {1},

}


@article{hurd-142,
author = {T. R. Hurd and Zhuowei Zhou},
collaboration = {},
title = {A Fourier Transform Method for Spread Option Pricing},
publisher = {SIAM},
year = {2010},
journal = {SIAM Journal on Financial Mathematics},
volume = {1},
pages = {142-157},
keywords = {spread options; multivariate spread options; jump diffusions; fast Fourier transform; gamma function},
url = {http://link.aip.org/link/?SJF/1/142/1},
doi = {10.1137/090750421}
}




@MISC{hubalek-2007,
  author = {T. Hubalek},
  title = {On Fourier methods for simple, multi-asset,and path-dependent options: accuracy and efficiency},
  howpublished = {\url{http://www.economia.uniroma2.it/conference/Public/1/Paper/102.pdf}},
  year = {2007}
}

@MISC{wolfram-parabolic-cylinder-function-interger-argument,
  author = {},
  title = {},
  howpublished = {\url{http://functions.wolfram.com/HypergeometricFunctions/ParabolicCylinderD/03/01/02/02/}},
}


@MISC{dirichlet-distribution-wiki,
  author = {wikipedia},
  title = {Dirichlet Distribution},
  howpublished = {\url{http://en.wikipedia.org/wiki/Dirichlet_distribution}},
}


@article{vanHameren2011,
title = "OneLOop: For the evaluation of one-loop scalar functions ",
journal = "Computer Physics Communications ",
volume = "182",
number = "11",
pages = "2427 - 2438",
year = "2011",
note = "",
issn = "0010-4655",
doi = "http://dx.doi.org/10.1016/j.cpc.2011.06.011",
url = "http://www.sciencedirect.com/science/article/pii/S0010465511002219",
author = "A. van Hameren",
keywords = "\{NLO\} computations",
keywords = "One-loop scalar functions ",
abstract = "OneLOop is a program to evaluate the one-loop scalar 1-point, 2-point, 3-point and 4-point functions, for all kinematical configurations relevant for collider-physics, and for any non-positive imaginary parts of the internal squared masses. It deals with all \{UV\} and \{IR\} divergences within dimensional regularization. Furthermore, it provides routines to evaluate these functions using straightforward numerical integration. Program summary Program title: OneLOop Catalogue identifier: AEJO_v1_0 Program summary URL: http://cpc.cs.qub.ac.uk/summaries/AEJO_v1_0.html Program obtainable from: \{CPC\} Program Library, Queen's University, Belfast, N. Ireland Licensing provisions: Standard \{CPC\} licence, http://cpc.cs.qub.ac.uk/licence/licence.html No. of lines in distributed program, including test data, etc.: 12 061 No. of bytes in distributed program, including test data, etc.: 74 163 Distribution format: tar.gz Programming language: Fortran Computer: Workstations Operating system: Linux, Unix RAM: Negligible Classification: 4.4, 11.1 Nature of problem: In order to reach next-to-leading order precision in the calculation of cross sections of hard scattering processes, one-loop amplitudes have to be evaluated. This is done by expressing them as linear combination of one-loop scalar functions. In a concrete calculation, these functions eventually have to be evaluated. If the scattering process involves unstable particles, consistency requires the evaluation of these functions with complex internal masses. Solution method: Expressions for the one-loop scalar functions in terms of single-variable analytic functions existing in literature have been implemented. Restrictions: The applicability is restricted to the kinematics occurring in collider-physics. Running time: The evaluation of the most general 4-point function with 4 complex masses takes about 180 μs, and the evaluation of the 4-point function with 4 real masses takes about 18 μs on a 2.80 \{GHz\} Intel Xeon processor. "
}

@article{DavydychevDelbourgo1998,
      author         = "Davydychev, Andrei I. and Delbourgo, Robert",
      title          = "{A Geometrical angle on Feynman integrals}",
      journal        = "J. Math. Phys.",
      volume         = "39",
      year           = "1998",
      pages          = "4299-4334",
      doi            = "10.1063/1.532513",
      eprint         = "hep-th/9709216",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "UTAS-PHYS-97-12",
      SLACcitation   = "%%CITATION = HEP-TH/9709216;%%"
}
@article{Withers2000,
title = "A simple expression for the multivariate Hermite polynomials ",
journal = "Statistics \& Probability Letters ",
volume = "47",
number = "2",
pages = "165 - 169",
year = "2000",
note = "",
issn = "0167-7152",
doi = "http://dx.doi.org/10.1016/S0167-7152(99)00153-4",
url = "http://www.sciencedirect.com/science/article/pii/S0167715299001534",
author = "C.S. Withers",
keywords = "Multivariate",
keywords = "Hermite polynomials",
keywords = "Edgeworth expansions ",
abstract = "We give a simple method for obtaining the multivariate Hermite polynomials. Explicitly we give all of them up to order three: these are needed for the second-order Edgeworth expansions for the distribution and density of most standardised vector estimates. "
}

@article{Carlson1963,
title = "Lauricella's hypergeometric function \{FD\} ",
journal = "Journal of Mathematical Analysis and Applications ",
volume = "7",
number = "3",
pages = "452 - 470",
year = "1963",
note = "",
issn = "0022-247X",
doi = "http://dx.doi.org/10.1016/0022-247X(63)90067-2",
url = "http://www.sciencedirect.com/science/article/pii/0022247X63900672",
author = "B.C Carlson"
}

 @article{Childs1967,
     jstor_articletype = {research-article},
     title = {Reduction of the Multivariate Normal Integral to Characteristic Form},
     author = {Childs, Donald R.},
     journal = {Biometrika},
     jstor_issuetitle = {},
     volume = {54},
     number = {1/2},
     jstor_formatteddate = {Jun., 1967},
     pages = {pp. 293-300},
     url = {http://www.jstor.org/stable/2333872},
     ISSN = {00063444},
     abstract = {The $n$th order integral over a generalized quadrant of the multivariate normal distribution has first been transformed to a series of integrals over the entire hypervolume for all orders. The series has been derived for all $n$ and is exhibited explicitly for all orders up to $n = 6$. The fourth-order integral has further been reduced to three first-order integrals, thus making them amenable to machine solution. This method avoids the difficulty of trying to integrate a mixed distribution over an interval when the variables cannot be separated. Three very special cases of the sixth-order integral are exhibited. It can be shown that the sixth-order integral can be reduced to five second-order integrals.},
     language = {English},
     year = {1967},
     publisher = {Biometrika Trust},
     copyright = {Copyright © 1967 Biometrika Trust},
    }
	
@BOOK{DeSacyGrammarI,
title     = {Grammaire Arabe I},
publisher = {Imprimerie Royale},
year      = {1831},
author    = {B. Silvestre De Sacy},
note = {www.archive.org/details/altufahalsanyah01sacygoog}
}
 
 
@BOOK{DeSacyGrammarII,
title     = {Grammaire Arabe II},
publisher = {Imprimerie Royale},
year      = {1831},
author    = {B. Silvestre De Sacy},
note = {www.archive.org/details/altufahalsanyah00sacygoog}
}

@article{SuzukiSantosSchmidt2003,
  author={A T Suzuki and E S Santos and A G M Schmidt},
  title={One-loop n -point equivalence among negative-dimensional, Mellin–Barnes and Feynman parametrization approaches to Feynman integrals},
  journal={Journal of Physics A: Mathematical and General},
  volume={36},
  number={47},
  pages={11859},
  url={http://stacks.iop.org/0305-4470/36/i=47/a=012},
  year={2003},
  abstract={We show that at one-loop order, negative-dimensional, Mellin–Barnes' (MB) and Feynman parametrization (FP) approaches to Feynman loop integral calculations are equivalent. Starting with a generating functional, for two and then for n -point scalar integrals, we show how to reobtain MB results, using negative-dimensional and FP techniques. The n -point result is valid for different masses, arbitrary exponents of propagators and dimension.}
}



@article{Davydychev1992,
   author = "Davydychev, A. I.",
   title = "General results for massive N‐point Feynman diagrams with different masses",
   journal = "Journal of Mathematical Physics",
   year = "1992",
   volume = "33",
   number = "1", 
   pages = "358-369",
   url = "http://scitation.aip.org/content/aip/journal/jmp/33/1/10.1063/1.529914",
   doi = "http://dx.doi.org/10.1063/1.529914" 
}



@article{Fleischer2003,
title = "A new hypergeometric representation of one-loop scalar integrals in d dimensions ",
journal = "Nuclear Physics B ",
volume = "672",
number = "1–2",
pages = "303 - 328",
year = "2003",
note = "",
issn = "0550-3213",
doi = "http://dx.doi.org/10.1016/j.nuclphysb.2003.09.004",
url = "http://www.sciencedirect.com/science/article/pii/S0550321303007545",
author = "J. Fleischer and F. Jegerlehner and O.V. Tarasov"
}


@book{Sinai2012,
   title =     {Theory of Probability and Random Processes},
   author =    {Leonid Koralov and Yakov G. Sinai},
   publisher = {Springer},
   isbn =      {3540254846,9783540254843},
   year =      {2012},
   series =    {Universitext},
   edition =   {2},
   volume =    {}
}

@book{Venkatesh2012,
   title =     {The theory of probability: explorations and applications},
   author =    {Santosh S. Venkatesh},
   publisher = {Cambridge University Press},
   isbn =      {1107024471,9781107024472,9781139169325,9781139848220},
   year =      {2012},
   series =    {},
   edition =   {},
   volume =    {}
	}
	
	
	@inproceedings{Weinzierl2010,
      author         = "Weinzierl, Stefan",
      title          = "{Introduction to Feynman Integrals}",
      booktitle      = "{Geometric and Topological Methods for Quantum Field
                        Theory}",
      year           = "2013",
      url            = "https://inspirehep.net/record/854751/files/arXiv:1005.1855.pdf",
      pages          = "144-187",
      eprint         = "1005.1855",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MZ-TH-1012",
      SLACcitation   = "%%CITATION = ARXIV:1005.1855;%%"
}

@book{Smirnov2012,
   title =     {Analytic tools for Feynman integrals},
   author =    {Vladimir A Smirnov },
   publisher = {Springer},
   isbn =      {9783642348853,3642348858,9783642348860,3642348866},
   year =      {2012},
   series =    {Springer tracts in modern physics, 250},
   edition =   {},
   volume =    {}
}


@article{Ferreira2003,
title = "Asymptotic expansions of the Lauricella hypergeometric function \{FD\} ",
journal = "Journal of Computational and Applied Mathematics ",
volume = "151",
number = "2",
pages = "235 - 256",
year = "2003",
note = "",
issn = "0377-0427",
doi = "http://dx.doi.org/10.1016/S0377-0427(02)00814-2",
url = "http://www.sciencedirect.com/science/article/pii/S0377042702008142",
author = "C. Ferreira and J. L. Lopez",
keywords = "Lauricella hypergeometric function",
keywords = "Asymptotic expansions",
keywords = "Distributional approach",
keywords = "Generalized Stieltjes transforms ",
}


@article{Davydychev1991,
title = "A simple formula for reducing Feynman diagrams to scalar integrals",
journal = "Physics Letters B",
volume = "263",
number = "1",
pages = "107 - 111",
year = "1991",
note = "",
issn = "0370-2693",
doi = "http://dx.doi.org/10.1016/0370-2693(91)91715-8",
url = "http://www.sciencedirect.com/science/article/pii/0370269391917158",
author = "A.I. Davydychev",

}


@article{Tarasov1996,
  title = {Connection between Feynman integrals having different values of the space-time dimension},
  author = {Tarasov, O. V.},
  journal = {Phys. Rev. D},
  volume = {54},
  issue = {10},
  pages = {6479--6490},
  numpages = {0},
  year = {1996},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.54.6479},
  url = {http://link.aps.org/doi/10.1103/PhysRevD.54.6479}
}

	
@book{Tilman2015,
   title =     {Fourier Transformation for Pedestrians},
   author =    {Tilman Butz},
   publisher = {Springer International Publishing},
   isbn =      {978-3-319-16984-2,978-3-319-16985-9},
   year =      {2015},
   series =    {Undergraduate Lecture Notes in Physics},
   edition =   {2},
   volume =    {}
 }	

@book{Hansen2014,
   title =     {Fourier Transforms: Principles and Applications},
   author =    {Eric W. Hansen},
   publisher = {Wiley},
   isbn =      {1118479149,9781118479148},
   year =      {2014},
   series =    {},
   edition =   {1},
   volume =    {}
 } 

@article{Abrahamson1964,
 ISSN = {00034851},
 URL = {http://www.jstor.org/stable/2238303},
 author = {I. G. Abrahamson},
 journal = {The Annals of Mathematical Statistics},
 number = {4},
 pages = {1685-1703},
 publisher = {Institute of Mathematical Statistics},
 title = {Orthant Probabilities for the Quadrivariate Normal Distribution},
 volume = {35},
 year = {1964}
}

@article{DelDuca2011wh,
      author         = "Del Duca, Vittorio and Dixon, Lance J. and Drummond,
                        James M. and Duhr, Claude and Henn, Johannes M. and
                        Smirnov, Vladimir A.",
      title          = "{The one-loop six-dimensional hexagon integral with three
                        massive corners}",
      journal        = "Phys. Rev.",
      volume         = "D84",
      year           = "2011",
      pages          = "045017",
      doi            = "10.1103/PhysRevD.84.045017",
      eprint         = "1105.2011",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "HU-EP-11-22, CERN-PH-TH-2011-105, SLAC-PUB-14458,
                        LAPTH-016-11, IPPP-11-21, DCPT-11-42, NSF-KITP-11-072,
                        --IPPP-11-21",
      SLACcitation   = "%%CITATION = ARXIV:1105.2011;%%"
}

@article{DelDuca2011jm,
      author         = "Del Duca, Vittorio and Duhr, Claude and Smirnov, Vladimir
                        A.",
      title          = "{The One-Loop One-Mass Hexagon Integral in D=6
                        Dimensions}",
      journal        = "JHEP",
      volume         = "07",
      year           = "2011",
      pages          = "064",
      doi            = "10.1007/JHEP07(2011)064",
      eprint         = "1105.1333",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "IPPP-11-20, DCPT-11-40, NSF-KITP-11-070",
      SLACcitation   = "%%CITATION = ARXIV:1105.1333;%%"
}

@article{DelDuca2011ne,
      author         = "Del Duca, Vittorio and Duhr, Claude and Smirnov, Vladimir
                        A.",
      title          = "{The massless hexagon integral in D = 6 dimensions}",
      journal        = "Phys. Lett.",
      volume         = "B703",
      year           = "2011",
      pages          = "363-365",
      doi            = "10.1016/j.physletb.2011.07.079",
      eprint         = "1104.2781",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DCPT-11-34, IPPP-11-17"
}

@article{Dixon2011ng,
      author         = "Dixon, Lance J. and Drummond, James M. and Henn, Johannes
                        M.",
      title          = "{The one-loop six-dimensional hexagon integral and its
                        relation to MHV amplitudes in N=4 SYM}",
      journal        = "JHEP",
      volume         = "06",
      year           = "2011",
      pages          = "100",
      doi            = "10.1007/JHEP06(2011)100",
      eprint         = "1104.2787",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "HU-EP-11-17, CERN-PH-TH-2011-075, SLAC-PUB-14434,LAPTH-013-11, CERN--PH--TH-2011-075, SLAC--PUB--14434",
      SLACcitation   = "%%CITATION = ARXIV:1104.2787;%%"
}

@MISC{Acklam,
  author = {P. J. Acklam},
  title = {{An algorithm for computing the inverse normal cumulative distribution
	function}},
  url= {home.online.no/~pjacklam/notes/invnorm/index.html},
  month = {June},
  year = {2000},
  note = {University of Oslo, Statistics Division},
}

@MISC{Staron2006,
  author = {A. Staron},
  title = {{"Calculations of one-loop N-point scalar integrals for N≥5" }},
  url= {http://prac.us.edu.pl/~ztpce/images/stories/seminaria/staron.pdf},
  month = {Janvier},
  year = {2006},
  note = {},
}





@article{Davydychev1991_2,
author = {A. I. Davydychev},
title = {Some exact results for N-point massive Feynman integrals},
journal = {Journal of Mathematical Physics},
volume = {32},
number = {4},
pages = {1052-1060},
year = {1991},
doi = {10.1063/1.529383},
URL = {http://dx.doi.org/10.1063/1.529383},
eprint = { http://dx.doi.org/10.1063/1.529383}
}

@Article{Kreimer1992,
author="Kreimer, D.",
title="One loop integrals revisited",
journal="Zeitschrift f{\"u}r Physik C Particles and Fields",
year="1992",
volume="54",
number="4",
pages="667--671",
abstract="We present a new calculation of the well-known one-loop two-point scalar and tensor functions. We also present a systematic reduction to a certain class of functions which minimizes the effort for calculating tensor integrals drastically. We avoid standard techniques such as Feynman parametrization and Wick rotation.",
issn="1431-5858",
doi="10.1007/BF01559496",
url="http://dx.doi.org/10.1007/BF01559496"
}


@article{Kreimer1993,
author = {Kreimer, D.},
title = {ONE-LOOP INTEGRALS REVISITED - THE THREE-POINT FUNCTIONS},
journal = {International Journal of Modern Physics A},
volume = {08},
number = {10},
pages = {1797-1814},
year = {1993},
doi = {10.1142/S0217751X93000758},
URL = {http://www.worldscientific.com/doi/abs/10.1142/S0217751X93000758},
eprint = {http://www.worldscientific.com/doi/pdf/10.1142/S0217751X93000758}
}


@article{BrucherFranzkowskiKreimer1994,
author = {Brucher, L. and Franzkowski, J. and Kreimer, D.},
title = {LOOP INTEGRALS, R-FUNCTIONS AND THEIR ANALYTIC CONTINUATION},
journal = {Modern Physics Letters A},
volume = {09},
number = {25},
pages = {2335-2345},
year = {1994},
doi = {10.1142/S0217732394002203},
URL = {http://www.worldscientific.com/doi/abs/10.1142/S0217732394002203},
eprint = {http://www.worldscientific.com/doi/pdf/10.1142/S0217732394002203}
}


@article{Davydychev2006,
title = "Geometrical methods in loop calculations and the three-point function ",
journal = "Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment ",
volume = "559",
number = "1",
pages = "293 - 297",
year = "2006",
note = "Proceedings of the X International Workshop on Advanced Computing and Analysis Techniques in Physics ResearchACAT 05X International Workshop on Advanced Computing and Analysis Techniques ",
issn = "0168-9002",
doi = "http://dx.doi.org/10.1016/j.nima.2005.11.174",
url = "http://www.sciencedirect.com/science/article/pii/S0168900205023004",
author = "Andrei I. Davydychev",
keywords = "Feynman diagram",
keywords = "Three-point function",
keywords = "Dimensional regularization "
}



@article{THOOFT1979,
title = "Scalar one-loop integrals",
journal = "Nuclear Physics B",
volume = "153",
number = "",
pages = "365 - 401",
year = "1979",
note = "",
issn = "0550-3213",
doi = "http://dx.doi.org/10.1016/0550-3213(79)90605-9",
url = "http://www.sciencedirect.com/science/article/pii/0550321379906059",
author = "G. 't Hooft and M. Veltman",
}


@article{DENNER1991,
title = "A compact expression for the scalar one-loop four-point function",
journal = "Nuclear Physics B",
volume = "367",
number = "3",
pages = "637 - 656",
year = "1991",
note = "",
issn = "0550-3213",
doi = "http://dx.doi.org/10.1016/0550-3213(91)90011-L",
url = "http://www.sciencedirect.com/science/article/pii/055032139190011L",
author = "A. Denner and U. Nierste and R. Scharf",

}

@Article{vanOldenborgh1990,
author="van Oldenborgh, G. J.
and Vermaseren, J. A. M.",
title="New algorithms for one-loop integrals",
journal="Zeitschrift f{\"u}r Physik C Particles and Fields",
year="1990",
volume="46",
number="3",
pages="425--437",
abstract="New algorithms are presented for evaluating the scalar one loop integrals for three- and four-point functions for arbitrary masses and external momenta. These formulations are useful both for analytic integration and for numerical evaluation in a computer program. The expressions are very compact and provide for an easy isolation of asymptotic behaviour and potential numerical problems. The tensor integrals have also been rewritten according to new algorithms, making it very easy to express amplitudes in terms of scalar loop integrals.",
issn="1431-5858",
doi="10.1007/BF01621031",
url="http://dx.doi.org/10.1007/BF01621031"
}

@article{DennerDittmaier2011,
title = "Scalar one-loop 4-point integrals ",
journal = "Nuclear Physics B ",
volume = "844",
number = "2",
pages = "199 - 242",
year = "2011",
note = "",
issn = "0550-3213",
doi = "http://dx.doi.org/10.1016/j.nuclphysb.2010.11.002",
url = "http://www.sciencedirect.com/science/article/pii/S0550321310005651",
author = "A. Denner and S. Dittmaier"
}


@article{Halpern1963,
  title = {Reduction Formula for the Five-Point Function},
  author = {Halpern, Francis R.},
  journal = {Phys. Rev. Lett.},
  volume = {10},
  issue = {7},
  pages = {310--312},
  numpages = {0},
  year = {1963},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.10.310},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.10.310}
}

@Article{Melrose1965,
author="Melrose, D. B.",
title="Reduction of feynman diagrams",
journal="Il Nuovo Cimento A (1965-1970)",
year="1965",
volume="40",
number="1",
pages="181--213",
abstract="Formulae expressing the amplitude for a Feynman diagram consisting of a single internal loop withn sides andn external lines as a sum of its reduced diagrams are derived by applying restrictions imposed by the finite dimensionality of space-time on the unparametrized amplitude. In 4-dimensional space-time these formulae express the amplitude for then-sided diagram as i) a sum of all its 5-sided reduced diagrams; this can be further expressed as ii) a sum of all its 4-sided reduced diagrams. The coefficients in each sum depend only on the external invariants and internal masses.",
issn="1826-9869",
doi="10.1007/BF02832919",
url="http://dx.doi.org/10.1007/BF02832919"
}






@article{Petersson1965,
author = {Bengt Petersson},
title = {Reduction of a One Loop Feynman Diagram with n Vertices in m Dimensional Lorentz Space},
journal = {Journal of Mathematical Physics},
volume = {6},
number = {12},
pages = {1955-1959},
year = {1965},
doi = {10.1063/1.1704747},
URL = {http://dx.doi.org/10.1063/1.1704747},
eprint = {http://dx.doi.org/10.1063/1.1704747}
}


@article{VANOLDENBORGH1992,
title = "The complex four point function for arbitrary masses",
journal = "Physics Letters B",
volume = "282",
number = "1",
pages = "185 - 189",
year = "1992",
note = "",
issn = "0370-2693",
doi = "http://dx.doi.org/10.1016/0370-2693(92)90499-T",
url = "http://www.sciencedirect.com/science/article/pii/037026939290499T",
author = "G.J. van Oldenborgh",

}

@article{BERN1993,
title = "Dimensionally regulated one-loop integrals",
journal = "Physics Letters B",
volume = "302",
number = "2",
pages = "299 - 308",
year = "1993",
note = "",
issn = "0370-2693",
doi = "http://dx.doi.org/10.1016/0370-2693(93)90400-C",
url = "http://www.sciencedirect.com/science/article/pii/037026939390400C",
author = "Zvi Bern and Lance Dixon and David A. Kosower",
}

@article{VANNEERVEN1984,
title = "Large loop integrals",
journal = "Physics Letters B",
volume = "137",
number = "3",
pages = "241 - 244",
year = "1984",
note = "",
issn = "0370-2693",
doi = "http://dx.doi.org/10.1016/0370-2693(84)90237-5",
url = "http://www.sciencedirect.com/science/article/pii/0370269384902375",
author = "W.L. van Neerven and J.A.M. Vermaseren",
}

@article{Kniehl2010,
title = "Analytic result for the one-loop scalar pentagon integral with massless propagators ",
journal = "Nuclear Physics B ",
volume = "833",
number = "3",
pages = "298 - 319",
year = "2010",
note = "",
issn = "0550-3213",
doi = "http://dx.doi.org/10.1016/j.nuclphysb.2010.03.006",
url = "http://www.sciencedirect.com/science/article/pii/S0550321310001379",
author = "Bernd A. Kniehl and Oleg V. Tarasov",
keywords = "Feynman integrals",
keywords = "Appell hypergeometric functions",
keywords = "Multi-Regge kinematics "
}

@Article{Kozlov2016,
author="Kozlov, Mikhail G.
and Lee, Roman N.",
title="One-loop pentagon integral in d dimensions from differential equations in $\epsilon$-form",
journal="Journal of High Energy Physics",
year="2016",
volume="2016",
number="2",
pages="21",
abstract="We apply the differential equation technique to the calculation of the one-loop massless diagram with five onshell legs. Using the reduction to ϵ-form, we manage to obtain a simple one-fold integral representation exact in space-time dimensionality. The expansion of the obtained result in ϵ and the analytical continuation to physical regions are discussed.",
issn="1029-8479",
doi="10.1007/JHEP02(2016)021",
url="http://dx.doi.org/10.1007/JHEP02(2016)021"
}



@article{Tarasov2000,
title = "Application and explicit solution of recurrence relations with respect to space-time dimension ",
journal = "Nuclear Physics B - Proceedings Supplements ",
volume = "89",
number = "1–3",
pages = "237 - 245",
year = "2000",
note = "Loops and Legs in Quantum Field Theory ",
issn = "0920-5632",
doi = "http://dx.doi.org/10.1016/S0920-5632(00)00849-5",
url = "//www.sciencedirect.com/science/article/pii/S0920563200008495",
author = "O.V. Tarasov"
}


